Transparency and Control in Platforms for Networked Markets

In this paper, we analyze the worst case efficiency loss of online platform designs under a networked Cournot competition model. Inspired by some of the largest platforms in operation today, the platform designs that we consider examine the trade-off between transparency and control. Our results show that open access designs incentivize increased production towards perfectly competitive levels and limit efficiency loss, while controlled allocation designs lead to producer-platform incentive misalignment, resulting in low participation and unbounded efficiency loss. We also show that discriminatory access designs balance transparency and control, achieving the best of both worlds by maintaining high participation rates while limiting efficiency loss.

==> 2020_ OR_ Net Cournot and Platforms/DMAmacros.tex <==
% Theorem, Lemma, Propositions, etc

 %Classifies font styles of different math environments into 2 categories: definition and remark
\theoremstyle{plain} % plain, {definition}, remark (bold title, regular text)
%\newtheorem{theorem}{Theorem}[section]		% Option in [] specifies the name of the section level to use in numbering the theorem
\newtheorem{theore}{Theorem}
\newtheorem{corollar}{Corollary}
\newtheorem{lemm}[theore]{Lemma}
\newtheorem{definitio}{Definition}
\newtheorem{proble}{Problem}
\newtheorem{assumptio}{Assumption}
\newtheorem{propert}{Property}
\newtheorem{propositio}{Proposition}
\newtheorem{conjectur}{Conjecture}
\newtheorem{exampl}{Example}
\newtheorem{rul}{Rule}

%\theoremstyle{remark} % plain, definition, {remark} (title in italics, regular text)
\newtheorem{remar}{Remark}
\newtheorem{fac}{Fact}
\newtheorem{clai}{Claim}


\newcommand{\theorem}[1]{\begin{theore} {\rm #1} \hfill $\Box$ \end{theore}}
\newcommand{\corollary}[1]{\begin{corollar} {\rm #1} \end{corollar}}
\newcommand{\lemma}[1]{\begin{lemm} {\rm #1}  \hfill $\Box$ \end{lemm}}
%\newcommand{\definition}[1]{\begin{definitio} {\rm #1 } \hfill $\Box$ \end{definitio}}
\newcommand{\definition}[1]{\begin{definitio} {\rm #1 } \end{definitio}}
\newcommand{\problem}[1]{\begin{proble} {\rm #1 } \end{proble}}
\newcommand{\assumption}[1]{\begin{assumptio} {\rm #1 } \end{assumptio}}
\newcommand{\property}[1]{\begin{propert} {\rm #1 } \end{propert}}
%\newcommand{\proposition}[1]{\begin{propositio} {\rm #1} \hfill $\Box$ \end{propositio}}
\newcommand{\proposition}[1]{\begin{propositio} {\rm #1} \end{propositio}}
\newcommand{\conjecture}[1]{\begin{conjectur} #1 \end{conjectur}}
\newcommand{\example}[1]{\begin{exampl} {\rm #1} \end{exampl}}
%\newcommand{\proof}[1]{{\em Proof:} \, #1 \hfill $\Box$}
\newcommand{\remark}[1]{\begin{remar} {\rm #1} \hfill \hfill $\blacksquare$ \end{remar}}
\newcommand{\fact}[1]{\begin{fac} {\rm #1} \end{fac}}
\newcommand{\mrule}[1]{\begin{rul} {\rm #1}  \end{rul}}


%\newcommand{\assumption}[2]{\noindent {\bf A#1.} \, #2 \\}
%\newcommand{\assumption}[2]{\noindent {\bf A#1.}#2 \\}


% Beginnings and ends, equations
\def\nn{\nonumber}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqs{\begin{equation*}}
\def\eeqs{\end{equation*}}
\def\balign{\begin{align}}
\def\ealign{\end{align}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ba{\begin{array}}
\def\ea{\end{array}}
\def\bcenter{\begin{center}}
\def\ecenter{\end{center}}
\def\bitem{\begin{itemize}}
\def\eitem{\end{itemize}}
\def\benum{\begin{enumerate}}
\def\eenum{\end{enumerate}}
\def\bdoc{\begin{document}}
\def\edoc{\end{document}}
\def\defeq{{\stackrel{\Delta}{=}}}
\def\nn{\nonumber}


% Lattins
\def\eg{{e.g., \/}}
\def\etal{{\it et al. \/}}
\def\viz{{\iet viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\etc{{\it etc.,\ \/}}
\def\cf{{cf.,\ \/}}

% Colors:
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

%\def\red{\textcolor{red}}
%\def\blue{\textcolor{blue}}
\def\black{\textcolor{black}}
\def\yellow{\textcolor{yellow}}
\def\green{\textcolor{green}}
\def\tcbg{\textcolor{bgrd}}
\def\magenta{\textcolor{magenta}}
\def\white{\textcolor{white}}
\def\gray{\textcolor{gray}}

% User-specified command definitions/redefinitions
\newcommand\Quote[1]{\lq\textsl{#1}\rq}
\newcommand\fr[2]{{\textstyle\frac{#1}{#2}}}

%% Mathbb
\newcommand{\Ambb}{\mathbb{A}}
\newcommand{\Bmbb}{\mathbb{B}}
\newcommand{\Cmbb}{\mathbb{C}}
\newcommand{\Dmbb}{\mathbb{D}}
\newcommand{\Embb}{\mathbb{E}}
\newcommand{\Fmbb}{\mathbb{F}}
\newcommand{\Gmbb}{\mathbb{G}}
\newcommand{\Hmbb}{\mathbb{H}}
\newcommand{\Imbb}{\mathbb{I}}
\newcommand{\Jmbb}{\mathbb{J}}
\newcommand{\Kmbb}{\mathbb{K}}
\newcommand{\Lmbb}{\mathbb{L}}
\newcommand{\Mmbb}{\mathbb{M}}
\newcommand{\Nmbb}{\mathbb{N}}
\newcommand{\Ombb}{\mathbb{O}}
\newcommand{\Pmbb}{\mathbb{P}}
\newcommand{\Qmbb}{\mathbb{Q}}
\newcommand{\Rmbb}{\mathbb{R}}
\newcommand{\Smbb}{\mathbb{S}}
\newcommand{\Tmbb}{\mathbb{T}}
\newcommand{\Umbb}{\mathbb{U}}
\newcommand{\Vmbb}{\mathbb{V}}
\newcommand{\Wmbb}{\mathbb{W}}
\newcommand{\Xmbb}{\mathbb{X}}
\newcommand{\Ymbb}{\mathbb{Y}}
\newcommand{\Zmbb}{\mathbb{Z}}

%
%% MSC Letters
\newcommand{\Amsc}{\mathcal{A}}
\newcommand{\Bmsc}{\mathcal{B}}
\newcommand{\Cmsc}{\mathcal{C}}
\newcommand{\Dmsc}{\mathcal{D}}
\newcommand{\Emsc}{\mathcal{E}}
\newcommand{\Fmsc}{\mathcal{F}}
\newcommand{\Gmsc}{\mathcal{G}}
\newcommand{\Hmsc}{\mathcal{H}}
\newcommand{\Imsc}{\mathcal{I}}
\newcommand{\Jmsc}{\mathcal{J}}
\newcommand{\Kmsc}{\mathcal{K}}
\newcommand{\Lmsc}{\mathcal{L}}
\newcommand{\Mmsc}{\mathcal{M}}
\newcommand{\Nmsc}{\mathcal{N}}
\newcommand{\Omsc}{\mathcal{O}}
\newcommand{\Pmsc}{\mathcal{P}}
\newcommand{\Qmsc}{\mathcal{Q}}
\newcommand{\Rmsc}{\mathcal{R}}
\newcommand{\Smsc}{\mathcal{S}}
\newcommand{\Tmsc}{\mathcal{T}}
\newcommand{\Umsc}{\mathcal{U}}
\newcommand{\Vmsc}{\mathcal{V}}
\newcommand{\Wmsc}{\mathcal{W}}
\newcommand{\Xmsc}{\mathcal{X}}
\newcommand{\Ymsc}{\mathcal{Y}}
\newcommand{\Zmsc}{\mathcal{Z}}


%% Script Letters
\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}


% Tiny capital letters sub-super scripts
\def\Atiny{\mbox{\tiny{A}}}
\def\Btiny{\mbox{\tiny{B}}}
\def\Ctiny{\mbox{\tiny{C}}}
\def\Dtiny{\mbox{\tiny{D}}}
\def\Etiny{\mbox{\tiny{E}}}
\def\Ctiny{\mbox{\tiny{C}}}
\def\Ftiny{\mbox{\tiny{F}}}
\def\Gtiny{\mbox{\tiny{G}}}
\def\Htiny{\mbox{\tiny{H}}}
\def\Itiny{\mbox{\tiny{I}}}
\def\Jtiny{\mbox{\tiny{J}}}
\def\Ktiny{\mbox{\tiny{K}}}
\def\Ltiny{\mbox{\tiny{L}}}
\def\Mtiny{\mbox{\tiny{M}}}
\def\Ntiny{\mbox{\tiny{N}}}
\def\Otiny{\mbox{\tiny{O}}}
\def\Ptiny{\mbox{\tiny{P}}}
\def\Qtiny{\mbox{\tiny{Q}}}
\def\Rtiny{\mbox{\tiny{R}}}
\def\Stiny{\mbox{\tiny{S}}}
\def\Ttiny{\mbox{\tiny{T}}}
\def\Utiny{\mbox{\tiny{U}}}
\def\Vtiny{\mbox{\tiny{V}}}
\def\Wtiny{\mbox{\tiny{W}}}
\def\Xtiny{\mbox{\tiny{X}}}
\def\Ytiny{\mbox{\tiny{Y}}}
\def\Ztiny{\mbox{\tiny{Z}}}


%
%
%% Greeks Boldface
\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
%\def\Pibf{{\bf$\Pi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}

%
% BF letters
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\pbf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

\def\0bf{\mathbf{0}}
\def\1bf{\mathbf{1}}

\def\lambdabf{\boldsymbol{\lambda}}
\def\mubf{\boldsymbol{\mu}}
\def\gammabf{\boldsymbol{\gamma}}
\def\xibf{\boldsymbol{\xi}}
\def\sigmabf{\boldsymbol{\sigma}}
\def\zetabf{\boldsymbol{\zeta}}

\def\Lambdabf{\boldsymbol{\Lambda}}
\def\Mubf{\boldsymbol{\Mu}}
\def\Gammabf{\boldsymbol{\Gamma}}
\def\Xibf{\boldsymbol{\Xi}}
\def\Sigmabf{\boldsymbol{\Sigma}}
\def\Zetabf{\boldsymbol{\Zeta}}




==> 2020_ OR_ Net Cournot and Platforms/abstract.tex <==
% abstract 
\ABSTRACT{%
% 	This paper considers performance in terms of efficiency guarantees under different designs of online platform markets under a networked Cournot competition model. We consider three platform designs, (i) open access, which promises fair and transparent interactions to all participants, (ii) controlled allocation, which distributes aggregate production in a socially efficient manner, and (iii) discriminatory access, which carefully constrain interactions to ensure efficiency in the market. We show that open access retains $2/3$ of the optimal social welfare even under selfish behavior and demonstrate yet better bounds based on cost (a)symmetry. On the other hand, we show that a controlled allocation platform optimizing social welfare can lead to curtailment of production in anticipation of misaligned allocations, instead leading to socially inefficient markets. In the final platform, we show that carefully designing the network and restricting interactions can lead to an improved $3/4$ retention rate of optimal social welfare and introduce a greedy algorithm to find such a network when production costs are linear. We introduce a novel model including search cost, highlighting potential inefficiencies of open access and the robustness of discriminatory access when considering search costs.   % Enter your abstract
In this paper, we analyze the worst case efficiency loss of online platform designs under a networked Cournot competition model. Inspired by some of the largest platforms in operation today, the platform designs that we consider examine the trade-off between  transparency and control. Our results show that open access designs incentivize increased production towards perfectly competitive levels and limit efficiency loss, while controlled allocation designs lead to producer-platform incentive misalignment, resulting in low participation and unbounded efficiency loss. We also show that discriminatory access designs balance transparency and control, achieving the best of both worlds by maintaining high participation rates while limiting efficiency loss. %We also study a model of consumer search cost which further distinguishes between the three designs. 
}%

==> 2020_ OR_ Net Cournot and Platforms/conclusion.tex <==
%conclusion

% Online platforms have emerged for different marketplaces over the last two decades. Even for a similar industry, platforms have varied designs, e.g., Uber vs. Didi, Amazon vs. eBay. These different designs compel a better comprehension of platform designs, and an understanding of the situations in which certain platform designs work well, and the difficulty involved in some of the more intricate designs. 

% \sam{Sam: I removed the discussion on the background in the study of online platforms, as I think this would be a repetition for readers of the conclusions section.}

\sam{
In this paper, we study the trade-off between transparency and control that arises in the design of access and allocation control mechanisms in online platforms.
Specifically, we leverage on a networked Cournot model to study the efficiency loss under three different platform designs: open access, controlled allocation and discriminatory access platform designs. 
}
% 
% 
% In this work, we present an overview of platform designs related to access and allocation control, proving their respective performances with regards to preserving social welfare with respect to the efficient social welfare. The platform designs we consider aims to maximize social welfare obtained and operates at different levels of transparency and control under the networked Cournot model. Specifically, they include open access, controlled allocation and discriminatory access platform designs respectively. \rone{Our proposed model and results provide insights on the potential sources of efficiency loss in online platforms. Such insights might be helpful in guiding the monitoring of market power in online platforms. For example, a potential application of our insights lies in the monitoring of market power in Uber, as Uber drivers have been reported to form “surge clubs” that create artificial price surges via simultaneous driver log-offs. The specific insights on the potential sources of efficiency loss in online platforms that our model provides is summarized as follows.}

Open access platforms, exemplified by eBay, allow all firms to participate freely in all markets.
\sam{Under the networked Cournot model considered in this paper, we show that open access platforms are guaranteed to preserve at least $2/3$ of the efficient social welfare at Nash equilibrium. In spite of this, the allocation of aggregate production among producers and markets is, in general, suboptimal in open access platforms. Specifically, our results reveal an ``excess entry theorem" in open access platforms, in the sense that the entry of new producers might lead to both a reduction in social welfare at Nash equilibrium if producers’ cost functions are allowed to be highly asymmetric.}

% Under the setting considered in this work, these platforms designs preserves at least half of production and $2/3$ of the efficient social welfare in the worst case. We also sharpen this efficiency loss bound by considering how the efficiency loss in open access platforms is affected by the cost asymmetry among firms. \rone{Our result on the worst-case efficiency loss in open access platforms (Theorem \ref{thm:PoA_asym}) also reveals an ``excess entry theorem", in the sense that increasing the number of producers might lead to both a reduction in social welfare at Nash and an increase in worst-case efficiency loss if producers’ cost functions are allowed to be highly asymmetric. While this “excess entry” result is similar in nature to the prediction provided in the classical paper of \citet{suzumura1987entry}, the causes for the reduction in social welfare due to “excess entry” in our paper and their work are different. Namely, Suzumura's paper shows that excess entry might lead to a reduction in social welfare if each firm has a fixed cost for entering an industry. In our paper, we show that excess entry might lead to a reduction in social welfare if the production cost of the new entrant is much higher than its competitors. In such scenarios, the entrant of a costly producer increases the aggregate supply quantity, but also takes away the supply from its (low-cost) competitors. Our paper shows the possibility that the increase in production cost might exceed the increase in consumer utility, which leads to a reduction in social welfare. }

\sam{
In order to reduce the efficiency loss in open access control platforms that is associated with the potential ``misallocation" of supply between markets, we consider controlled allocation platforms, where the platform specifies the exact allocation of aggregate supply to each market. In spite of the good intentions behind the design of such platforms, the worst-case efficiency loss in controlled allocation platforms is unbounded due to the incentive for production withholding.
}
% Controlled allocation platforms assign production to maximize social welfare, potentially causing a reduction in production from firms, as empirically witnessed under ride-sharing platforms with similar designs such as Uber. We show under the setting considered in this work, that it leads to unbounded inefficiency in the worst case, i.e., the price of anarchy can grow linearly in the number of markets. %We show that the networked Stackelberg game introduced recently is equivalent to our controlled allocation platforms when there is no network constraints, and therefore our inefficiency results extends to that setting too. 
% We extend the construction to optimizing over a convex combination of revenue and consumer surplus, which leads to different worst case efficiency loss bounds.  The conclusion we draw from controlled allocation platforms hint at the potential danger of withheld production. \rone{Our results identify properties of the inverse demand function under which the withholding of supply indeed leads to a large efficiency loss. Specifically, the proof of Theorem \ref{thm:ineff} shows that the withholding of capacity would lead to a large efficiency loss if the inverse demand function has a “long tail” (i.e., settings in which the market consists of a large number of consumers whose willingness to pay is low). In contrast, our results on the bounded efficiency loss in open access platforms point out that the withholding of supply might not lead to a large efficiency loss if the inverse demand function does not exhibit such a “long-tail” property.}

\sam{Finally, with the objective of striking a balance between open access and controlled allocation platform designs, we consider discriminatory access platforms, where the platform chooses the network that specifies the set of markets that each firm has access to.
% Discriminatory access platform designs, exemplified by Amazon's Buybox, optimize network access, to restrict the interactions of certain firm-market pairs. 
We show that such a platform design improves upon open access platforms in terms of the worst-case efficiency loss.
Specifically, under the optimized network, discriminatory access platforms are guaranteed to preserve at least $3/4$ of the efficient social welfare. }
% Additionally, while network design may be difficult in general, we design a greedy algorithm that performs network design efficiently under linear cost constraints, which we show to be the worst case cost functions. 

% This work sheds light on the tradeoffs between transparency, control and worst case efficiency loss. Moreover, the main contributing factors for high and low efficiency loss, e.g., misaligned objectives that lead to production withholding for controlled allocation platform designs, are indeed witnessed too in real-life online platforms. For example, empirical studies on Uber have shown that drivers collaborate to synchronize their productions to cause demand spikes, resulting in better individual payoff but decreased system performance. 

\sam{We conclude this paper with a discussion on future work.} One aspect of platform design that we have ignored thus far is related to customer \emph{search costs}. 
% Search costs represent one form of consumer transaction or switching costs involved in searching for better alternatives. 
One of the initial goals of platforms is to lower search costs for consumers and lower entry costs for producers. Without careful understanding of the trade-offs between the aforementioned objectives and carefully balancing them, one can end up in a situation where search costs overwhelm consumers. For example, an open access platform design for a ride-sharing platform may not be a good idea, since the number of producers (in this case, drivers) in such platforms is large, resulting in large search costs for consumers. On the other hand, successful ride-sharing platforms, e.g., Uber, show only prices and do not offer alternative producers, eliminating any search cost involved in a transaction. Our preliminary results, included as Theorem 6 in the Appendix, confirm these observations when considering an additional search costs model. 
Additionally, certain unmodelled constraints can compel particular platform design over others. For example, electricity markets are an important platform that work under physical network constraints and therefore compelled to be under a controlled allocation design. As such, more work is needed to understand some of these issues, e.g., physical network constraints and the potential of demand management mechanisms such as demand response. 

% \textcolor{blue}{Taken from old intro, to merge with paragraph above. } To understand the impact of search costs on the efficiency of the three platform designs, we introduce a simple search cost model in Section \ref{sec:searchcosts} that yields important contrasts. In particular, under large consumer search cost, the worst case efficiency loss of open access platforms may no longer be bounded since welfare losses from search costs may outweigh the benefits of open access. On the other hand, the discriminatory access platform design remains efficient in the face of search costs and can be further optimized to balance search costs with efficiency of the matching. 

%Together with the prevalence of controlled allocation designs, e.g., in ride-sharing and electricity markets, the results that we have begs a better understanding of the design. Many such applications are networked constrained, e.g., electricity markets with transmission line constraints. What are the impact of network constraints on these networked Stackelberg games and more importantly, can the platform mitigate the unintended incentives for producers to curtail their production? 

%Lastly, we present a search cost model under this setting to study the impact of search cost on platform design. The search cost model is simple, and essentially penalizes too many choices from the consumers' point of view. We show that in the worst case, open access platforms with search costs may lead to an unbounded loss in efficiency while discriminatory access platforms continue to perform efficiently under linear cost settings. 

==> 2020_ OR_ Net Cournot and Platforms/controlledplatform.tex <==

\sam{While open access platforms are shown to exhibit bounded efficiency loss, the welfare loss stemming  from  the  ``misallocation"  of  supply  across  the  different  markets  can  be  large.
% Despite preserving large production rates, the open access platform design suffers from some efficiency loss through misaligned allocations. 
In this section, we investigate a class of  \emph{controlled allocation} platform designs, where the platform optimally allocates the aggregate production across the different markets to maximize  a convex combination of consumer surplus and producer revenue.
Despite their welfare-maximizing intentions, controlled allocation platforms may suffer large efficiency loss in practice, due to the firms' withholding their production relative to socially optimal levels. Such  withholding of capacity is has been observed to occur in ride-sharing platforms, for example \citep{chen2017thrown}.
% for example, the empirical study of the ride-sharing platform Uber in \citet{chen2017thrown}.
In this section, we show} \rone{that controlled allocation platforms may exhibit an unbounded price of anarchy. In particular, when the platform controls the allocation of supply to maximize social welfare, the corresponding price of anarchy is $\Omega(m)$,} \eb{which grows unbounded in the number of markets.  This is in stark contrast to open access and discriminatory access platforms, which are guaranteed to have a price of anarchy that is uniformly bounded from above in the number of markets $m$.}

% \sam{\textbf{Sam:} John, can you add a description of our contribution of this section here?} \johnp{John: Done...}

% to aggregate production and perfectly allocate to various markets %to maximize certain objectives, e.g., social welfare, 
% in hope that this control circumvents the misaligned allocations. %Some examples of platforms that have a similar platform design include Uber, which does not control the amount of hours drivers or drivers in a neighborhood put in, but makes allocation decisions for each driver-rider or driver area-pick-up area pair. 
% Unlike the open access platform described in Section \ref{sec:oap}, a controlled allocation platform allocates the production to different markets in a socially efficient way for any given aggregate production quantity. %Another similar platform is an independent system operator (ISO) in the electricity market which reallocates generation of power considering line capacity and physical constraints on the power network. 

% However, controlled allocation platforms are not as simple to optimize as they seem.  In particular, the control over allocations exerted by the platform may create unintended incentives incentives for firms to withhold production, as empirically shown in \citet{chen2017thrown} for the ride-sharing platform Uber. Though firms cannot strategically choose prices or matches, they retain control over their participation in the platform.  In the networked Stackelberg setting, this takes the form of strategic choices of production levels, with the platform only allocating on their behalf to maximize a certain quantity, e.g., social welfare.

%The first example of a controlled allocation platform is one that maximizes exactly what we hope to optimize for, namely social welfare. We show that in this controlled allocation platform, that the worst case efficiency loss grows linearly in the number of markets in the system.  

% Our main result in this section highlights that distorted incentives in controlled allocation platforms can lead to inefficient market outcomes that can be far worse than outcomes under open access designs. 

% \sam{\textbf{Sam:} it seems that the statement of Theorem \ref{thm:ineff} is tailored to the case where the platform maximizes social welfare. Can you point this out in the theorem statement (e.g., point out that maximizing social welfare corresponds to the case where $\lambda = 1/2$, and revise the corresponding discussions accordingly? } \johnp{John: Can you see if that's okay?}

\sam{We first consider a class of controlled allocation platform that maximize social welfare. This corresponds to a platform objective function ${\rm OBJ}(d;1/2)$ (i.e., $\lambda = 1/2$). In Theorem \ref{thm:ineff}, we show that the price of anarchy of controlled allocation platforms that maximize social welfare grows at least linearly in the number of markets.}
\begin{theorem}
	\label{thm:ineff}
% 	A controlled allocation platform that maximizes social welfare can have unbounded price of anarchy. 
	\sam{The price of anarchy of a controlled allocation platform that maximizes social welfare ${\rm OBJ}(d;1/2)$ grows at least linearly in the number of markets. That is, there exists a family of inverse demand functions and cost profiles such that}
% 	In particular, there exists a family of networks where the Stackelberg equilibrium is unique and the worst case efficiency loss is $\Omega(|M|)$, i.e., there exists $s^{\textrm{SE}}$ and cost functions $C$ such that: 
    $$
    \rho(1/2, M) \geq \frac{8m}{9}.
    $$
\end{theorem}

% \sam{Sam: one minor comment: I would suggest changing $|M|$ to $m$ throughout, as we have used $m$ as the number of markets previously.} \johnp{John: Good call!}

% \sam{Sam: I actually noticed that there are still some instances of the notation $\rho (\lambda, M)$ (e.g. after the definition of $\rho (\lambda)$ and in the statement of Theorem 3. Can you make sure that the notation is consistent throughout the paper?}

\sam{
%Theorem \ref{thm:ineff} shows that the worst-case efficiency loss in controlled allocation platforms can be substantially larger than open access platforms.
The primary driver behind this growth in efficiency loss  stems from the production withholding incentives  that emerge in controlled allocation platforms. In open access platforms, each firm is free to specify the exact quantity that it produces in each market. As a result, a firm can  increase its production in one market without affecting its revenue in other markets. 
In contrast, in controlled allocation platforms,  each firm is only allowed to specify its aggregate production, while the platform determines the allocation of supply across the different markets. 
Crucially, increasing a firm's aggregate production may result in a reduction in the uniform price that the firm is paid (in all markets), which may  ultimately give rise to stronger incentives for  production withholding than in open access markets.
In the proof of Theorem \ref{thm:ineff}, we construct an example that clearly illustrates this intuition. 
% In this example, the aggregate supply to each market is positive at the efficient production profile. At Nash equilibrium, however, only the market with the highest maximum willingness to pay has a nonzero aggregate supply due to the production withholding from producers. The efficiency loss at said Nash equilibrium grows linearly in the number of markets, as the inverse demand functions are constructed in such a way that the efficient social welfare grows linearly in the number of markets.
}

\eb{In Section \ref{sec:lb_cap}, we extend these analyses to address the entire gamut of controlled allocation  optimization objectives  ${\rm OBJ}(d;\lambda)$ ($0 \leq \lambda  \leq 1$) considered in this paper. Loosely speaking, our results reveal that platform objectives that ``favor'' firms over consumers  (by weighing the firms' aggregate revenue more heavily) weaken the incentive for production withholding.}

% \sam{One might argue that the large worst-case efficiency loss described in Theorem \ref{thm:ineff} is an artifact of a poorly chosen market clearing mechanism. Instead, one might consider a larger family of market clearing mechanisms, and select a different market clearing mechanism that has a smaller worst-case efficiency loss. 
% In Section \ref{sec:lb_cap}, 
% % we investigate a family of market clearing mechanisms where the objective function in the market clearing problem is given by a convex combination of consumer surplus and producer revenue.
% we show that the worst case efficiency loss can even be unbounded for a large family of market clearing mechanisms due to the potential production withholding from producers.} 



% \johnp{John: I feel like the statement 'increasing production in one market might lead to a reduction in the price that the producer is charged according to in all markets' may seem to suggest reallocations. I think one can only increase production and cannot choose where it goes to. To some extent the reduction in price across every market is true but perhaps part of the story also revolves around the alignment of objectives between the platform and the producers... }

% \sam{Sam: That's a good point. It should be that the producer couldn't increase its production solely in one market.} \johnp{John: Yup!}

% \sam{One might argue that the large worst-case efficiency loss described in Theorem \ref{thm:ineff} is an artifact of a poorly chosen market clearing mechanism. Instead, one might consider a larger family of market clearing mechanisms, and select a different market clearing mechanism that has a smaller worst-case efficiency loss. 
% In Section \ref{sec:lb_cap}, 
% % we investigate a family of market clearing mechanisms where the objective function in the market clearing problem is given by a convex combination of consumer surplus and producer revenue.
% we show that the worst case efficiency loss can even be unbounded for a large family of market clearing mechanisms due to the potential production withholding from producers.} 
% \rone{explore lower bounds for the price of anarchy over a family of market clearing mechanisms that are optimizing convex combinations of revenue and consumer surplus. We first show that a consumer surplus maximizing controlled allocation platform can suffer infinitely large price of anarchy even when the number of markets are small, and generalize that example to controlled allocation platforms with $\lambda \in [2/3,1]$, highlighting that they incur unbounded price of anarchy even in the presence of only two markets. On the other hand, we show that the example for the social welfare maximizing can be generalized over $\lambda \in [0,2/3)$, where price of anarchy grows in the number of markets $m$. }

% \rone{The contrast between Theorem \ref{thm:ineff} for controlled allocation platforms and Theorem \ref{thm:PoA_asym} for open access platforms in Section 3 is pronounced. While open access platforms preserve at least $2/3$ of the efficient social welfare regardless of market parameters, controlling allocations can lead to reactive producer behavior, which has instead an unbounded worst case efficiency loss. }
% We first define formally the networked Cournot game under the controlled allocation platform as a networked Stackelberg game, first introduced in \citet{xu2017efficiency}. We extend their results and show that the equivalent networked Stackelberg game can possibly have no equilibria, a unique equilibria or even multiple equilibria. 
% In this section, we first prove Theorem \ref{thm:ineff}. Additionally, we provide a generalization of Theorem \ref{thm:ineff} in Theorem \ref{thm:generalcap}, which shows that controlled allocation platforms remain inefficient even if the platform chooses different objective functions in clearing the market.


% \subsection{The networked Stackelberg game}
% A Stackelberg competition model is one that includes a leader, who moves first, and a follower, who moves sequentially after. The leader is assumed to know the best response of the follower (dependent on the move it makes), and solves by backward induction the optimal choice to make, i.e., in this scenario the quantity to produce. In our networked Stackelberg game, the firms act as leaders deciding their production, and the platform best responds by allocating the aggregate production to maximize an objective made known beforehand to the firms, e.g., social welfare. We adopt this model from the work of \citet{xu2017efficiency} where they also consider a networked Stackelberg model with constrained capacity.

% We first define the follower's or platform's action. Maximizing social welfare, the platform takes the aggregate production $Q$ (in which it has no control over), and performs the following optimization to find out the social welfare maximizing allocations to the different markets: 
% \begin{align*}
% \max_{d_1,d_2,\dots,d_m}~&~ \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)dz - \sum_{i=1}^n \cost_i(\supply_i)\\
% s.t. ~&~ \sum_{j=1}^m d_j\leq Q
% \end{align*}
% Having no control of the amount of production from the firms such that the supply is fixed, the optimization is equivalent to the maximizing just consumer welfare: 
% \begin{align*}
% \max_{d_1,d_2,\dots,d_m}~&~ \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)dz \\
% s.t. ~&~ \sum_{j=1}^m d_j\leq Q
% \end{align*}
% In general, the resulting allocation is equivalent for all objective functions that are equivalent modulo functions of the firms' productions, e.g., cost. One such example from above is that controlled allocation platforms maximizing social welfare and consumer welfare are essentially the same platform and make the same allocations. 

% By observing stationarity conditions of the platform's optimization problem, e.g., maximizing social welfare, the firms fully understand how firms' productions are going to be allocated across markets, and act together as joint leaders in the networked Stackelberg game. For example, for the social welfare maximizing controlled allocation platform, the platform allocates from the market with the largest willingness to pay, transitioning into markets with smaller willingness to pay, keeping prices across the markets participated in constant. An allocation function $A:\mathbf{R}^+ \rightarrow \mathbf{R}^m$ can then be defined that takes as input the aggregate production $Q = \sum_{i\in F} s_i$ and outputs the corresponding allocations to the markets $d=\{d_1,d_2, \dots, d_m\}$. We assume also that in optimizing other objective functions, the price offered to the firms is an weighted average price of the markets (irrelevant to the social welfare maximizing platform since prices are kept the same). 

% Having defined the allocation function $A$, we can now define a Stackelberg equilibrium based on the firms' productions $s_i$. The profit of a firm $i$ can be written under the platform as: 
% $$
% \pi(s_i, s_{-i}) = s_i p(A(\sum_i s_i)) - C_i(s_i),
% $$
% and a Stackelberg equilibrium $s^{SE}$ is such that: 
% $$
% \pi(s_i^{SE},s_{-i}^{SE}) \geq \pi(s_i,s_{-i}^{SE}), ~\forall s_i\geq 0
% $$

% \begin{remark}
% 	There exists systems with (i) no Stackelberg equilibrium, (ii) a unique Stackelberg equilibrium, and (iii) multiple Stackelberg equilibria.
% \end{remark}

% An example where an equilibrium does not exist can be found in \citet{xu2017efficiency}, while the single market case always leads to a unique equilibrium, and our result for unbounded price of anarchy for a social welfare maximizing controlled allocation platform will include an example for a system with multiple equilibria. For controlled allocation platforms maximizing objectives other than social welfare, the equilibrium under a networked setting is much harder to attain and the examples we have usually have only one firm, and often have zero production cost.  



%Despite the seemingly efficient open access platform result described in Section \ref{sec:oap}, a further optimized platform is always sought for. One intuitive first reaction to circumventing the remaining possible inefficiency of the open access model is for platforms to control and optimize allocation of firms' productions to markets directly.  It is typically possible for the platform to have considerable knowledge on the firm costs and market demands, which makes optimization of allocation appealing. This leads to the design of \emph{controlled allocation platforms}.

% However, controlled allocation platforms are not as simple to optimize as they seem.  In particular, 
% the control over allocations exerted by the platform may create unintended incentives for the firms, as empirically shown in \citet{chen2017thrown}.  Though firms cannot strategically choose prices or matches, they retain control over their participation in the platform.  In the networked Cournot setting, this takes the form of strategic choices of production levels, with the platform allocating on their behalf to maximize a certain quantity, e.g., social welfare.

% We show that for a variety of objectives between social welfare and consumer surplus, the resulting price of anarchy is arbitrarily large, either infinitely large or growing in the number of markets.  

% \subsection{Social Welfare Maximizing Controlled Allocation Platforms}

% \sam{Can you change Perfect allocation $\rightarrow$ efficient allocation? \johnp{John: done!}
% }

% Given the results from Section \ref{sec:oap}, one may intuitively think that efficient allocation can lead to improved efficiency loss bounds. In Theorem \ref{thm:ineff}, we show that such a platform, even with the best intentions, i.e., maximizing social welfare (equivalent to maximizing $\rm{OBJ}(d;1/2)$), can lead instead to an unbounded efficiency loss. On the other hand, allowing for an open access design and not controlling allocations lead to a bounded worst case efficiency loss as in Section \ref{sec:oap}. 

% Note that the networks constructed to prove Theorem \ref{thm:ineff} are simple. They use a single firm with costless production. \rone{Observe that when a firm has no production cost, the socially efficient production is always to produce until the price in every market is driven to~$0$. The efficient allocation is to allocate production in a way which keep prices constant. Consequently, as the profit-maximizing producer increase production, unit prices decrease monotonically. Therefore, the producer will not produce until the prices reach $0$.} 

% The construction begins with a single market and then, as markets are added one by one to the system, the parameters of each new market are such that the firm has no incentive to increase production as profit no longer increases due to the decreased unit prices, whereas the socially efficient (non-Nash) production level does increase, as does the efficient welfare. 

% \sam{I think the above paragraph can be re-organized as follows:
% \begin{itemize}
%     \item First talk about the structure of the efficient allocation (i.e., produce until price in every market is 0
%     \item Illustrate why producers don't want to increase production from the perspective of price change (as opposed to ``reallocation", which would be a vague concept
% \end{itemize}
% } \johnp{John: Edited! Can you see if that's okay? }


% Now, using \autoref{lem:agg-demand}, we can prove \autoref{thm:ineff}.



% Theorem \ref{thm:ineff} is proven using a construction which highlights that an efficient platform \rone{should incentivize} firms against withholding production by changing how quickly prices drop, which may be achieved by modifying the market clearing mechanism appropriately. 
% This begs the question: Can the platform do better by selecting a \rone{different market clearing mechanism}? We prove a lower bound of the worst case efficiency loss in controlled allocation platforms when the platform chooses over a family of alternative objective functions in clearing the market. In particular, such a family of objective functions can be \rone{parameterized by their weight of the} convex combinations of consumer surplus and revenue.

% \sam{A couple of comments:
% \begin{itemize}
%     \item I would actually be more direct in talking about the problem in controlled allocation platforms. Producers would withhold production due to unfavorable pricing policy (i.e. price might drop too fast as production quantity increases). As a result, we might modify the market clearing mechanism accordingly to deal with this problem
%     \item Instead of saying ``optimizing a different quantity", I would say ``choosing a different market clearing mechanism"
%     \item It would be more direct to describe how this family of market clearing mechanisms is parameterized. Specifically, they are parameterized by the weight of the convex combination.
% \end{itemize}
% }

% \johnp{John: Thanks for the comments. I've taken a shot at addressing them. }



% \subsection{Consumer Welfare Maximizing Controlled Allocation Platforms}

% Since the platform actually does not control the quantity produced into the system, but only allocates, then any objective function that is equivalent to social welfare modulo functions of cost all results in the same analysis and results. To illustrate this, consider consumer welfare, defined as follows: 

% \begin{definition}
% 	Specifically, the consumer welfare associated with a supply profile $\production$ defined according to
% 	\begin{align}
% 	\label{eq:cwelfare-def}
% 	\text{CW}(\production) := \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)dz,
% 	\end{align}
% 	where $\demand_j$ is defined in Eq. (2), respectively. 
% \end{definition}

% \begin{corollary}
% 	Since controlled allocation platforms do not consider production costs, the above result is true also if the platform maximizes consumer welfare. Any other objective functions of the form $\SW + g(C)$ would achieve the same result. 
% \end{corollary}

% \subsection{Consumer Surplus Maximizing Controlled Allocation Platforms}

%Instead of proving this result, we will prove a more general result in the proceeding subsection, showing exactly how supply will be distributed, and then give an example whereby price of anarchy is $\infty$.



% \subsection{A General result on Controlled Allocation Platforms. \ebc{Better title?}} 
\subsection{Lower Bounds on the Price of Anarchy in Controlled Allocation Platforms} \label{sec:lb_cap}
% \johnp{John: How about "Lower Bounds on Price of Anarchy for other Controlled Allocation Platforms/different Clearing Objectives"?} \ebc{(Eilyan: How abou ``Limits on the Performance of Controlled Allocation Platforms'' or ``Lower Bounds on the Price of Anarchy in Controlled Allocation Platforms''?)} \johnp{John: The latter looks good! }
% Before attending to the family of objectives, we first consider the corner case in consumer surplus, which helps give some intuition as to why the worst case efficiency loss can grow large. In fact, when platforms maximize ${\rm OBJ}(d;1)$ or equivalently, consumer surplus, the worst case efficiency loss is unbounded.

 \sam{We first consider the case in which the  platform controls the allocation of supply to maximize  consumer surplus ($\lambda = 1$).}
 
 %This particular setting sheds light the primary drivers of efficiency loss in controlled allocation platforms.
 
%We first consider the case in which the  platform controls the allocation of supply to maximize  consumer surplus ($\lambda = 1$). This particular setting sheds light on the The analysis of the worst case efficiency loss in such controlled allocation platforms provides intuition on the source of large efficiency loss in controlled allocation platforms.
% We have the following proposition.


% Given a fixed supply, the consumer surplus is defined as follows. 

% \begin{definition}
% 	\emph{Specifically, the consumer surplus associated with a demand profile $\demand$ is defined according to
% 	\begin{align}
% 	\label{eq:surplus-def}
% 	\text{CS}(d) := \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)dz - \demand_j\price_j(\demand_j),
% 	\end{align}
% 	where $\demand_j$ is defined in Eq. (2).} 
% \end{definition}


% \sam{The notation in Prop. 4 should be ${\rm OBJ}(d;1)$. Can you fix this notation throughout?} \johnp{John: I've changed that... }

\begin{proposition}\label{claim:cap-cs}
	Assume that there are at least $m \geq 2$ markets.
	Controlled allocation platforms that maximize  consumer surplus have an unbounded price of anarchy. \sam{That is, there exists a family of inverse demand functions and cost profile such that}
	\begin{align*}
	    \rho (1, M) = \infty.
	\end{align*}
\end{proposition}

\sam{%In the absence of explicit non-negativity constraint on the prices, 
It is not difficult to show that controlled allocation platforms, which maximize ${\rm OBJ}(d;1)$ (consumer surplus),  will allocate the entire aggregate supply to the market that has the largest demand price elasticity.
%(i.e. the largest slope in the inverse demand function). 
A supply allocation rule of this form will, in general, result in  production withholding relative to socially optimal levels. We illustrate these effects more concretely in a simple two-market platform.} In this example, each 
 firm is assumed to have a constant marginal cost of production $c > 0$, and the inverse demand functions associated with each of the two markets are defined as 
$$
p_1 = (c+\epsilon) - (\epsilon/2) d_1  \ \ \text{and} \ \ \ p_2 = (c-\epsilon) - \epsilon d_2, 
$$
where $\epsilon > 0$.
\sam{The supply allocation rule, which maximizes consumer surplus, will allocate the aggregate production quantity supplied by the firms to the second market. As the resulting market clearing price will in general be smaller than the per-unit production cost of each firm, the firms will collectively withhold their output, producing nothing at Nash equilibrium.} \eb{This is in contrast to  the socially efficient market outcome, where firms collectively produce two units in the first market and zero units in the second market. The price of anarchy is, therefore, unbounded in this simple example. }
% \sam{
% Finally, the aforementioned arguments can be generalized to show that the price of anarchy is large in controlled allocation platforms that maximize social welfare due to the production withholding behavior it induces.}

% The idea behind the two node construction which proves the proposition is simple: \rone{ A platform maximizing consumer surplus is agnostic} to the maximal willingness to pay, whereas rational producers do consider their maximal willingness to pay.

% \sam{A controlled allocation platform that maximizes ${\rm OBJ}(d;1)$ (consumer surplus) will allocate the aggregate production to the different markets in descending order of their price elasticity.}
% \rone{This means that the platform may allocate production to consumers whose willingness to pay is less than the marginal cost of production. As a result, producers might end up not producing anything.} 
% A simple example \sam{to illustrate this intuition} is a one firm, two market example, where the firm has \rone{fixed per-unit cost $c$}, and the markets have inverse demand functions
% $$
% p_1 = (c+\epsilon) - (\epsilon/2) d_1,~p_2 = (c-\epsilon) - \epsilon d_2.
% $$
% \sam{\textbf{Sam:} Should it be $\beta_2 > \beta_1$ instead?} \johnp{John: Somehow I got confused and change it the other day... }
% \sam{The platform will allocate all demand to the second market first, as the price elasticity of demand is higher in the second market. As a result, the firm produces nothing at Nash equilibrium.}
% \rone{Since the price elasticity is lower in the second market, the platform whose market clearing mechanism maximizes consumer surplus would allocate all demand to the second market first, }until price is zero before accessing the first market. It is trivial to show that being forced to produce first to satisfy the entire demand of the second market, the firm would rather not produce anything at all. 
% On the other hand, the efficient allocation has $2$ units in the first market and zero in the second. \sam{As a result, the efficient social welfare is strictly positive and the price of anarchy is unbounded.}

% \sam{A couple of comments:
% \begin{itemize}
%     \item Is this statement a typo? ``where the firm has linear production cost $cs$"
%     \item Instead of stating the parameters $\alpha_j$ and $\beta_j$ for $j = 1, 2$, I think it would be clearer to state the inverse demand functions directly. 
% \end{itemize}
% }

% \johnp{John: Fixed them! :) }

\sam{Proposition \ref{claim:cap-cs} reveals that a poorly chosen market clearing mechanism may result in a substantial loss of efficiency at Nash equilibrium.  In what follows, we inspect a family of market clearing mechanisms where the platform's  objective function ${\rm OBJ}(d;\lambda)$ ($0 \leq \lambda  \leq 1$) is specified according to a convex combination of aggregate consumer surplus and producer revenue (cf. Section \ref{sec:prelims} for detailed formulation).
% 
% The control over allocations is delicate, and explicitly not optimizing (as in the open access case) can be more efficient \rone{than controlling allocations with market clearing mechanisms of either social welfare or consumer surplus}. 
% To understand how the worst case efficiency loss is affected by different objective functions, we now extend the analysis of the social welfare case to consider an objective $\textrm{OBJ}(d;\lambda)$ to be a convex combination of consumer surplus and revenue, parameterized by $\lambda$, as defined in Section \ref{sec:prelims}. 
% $$
% \text{OBJ}(d; \lambda) = \sum_{j\in M} \left[\lambda\left(\int_{0}^{d_j} p_j(q)dq - d_jp_j(d_j) \right) + (1-\lambda)\left(d_jp_j(d_j)\right)\right].
% $$
% For example, when $\lambda=0.5$, the resulting objective is half of consumer welfare, which is equivalent to a social welfare objective since the platform have no control over supply profiles. In particular, 
In Theorem \ref{thm:generalcap}, we provide lower bounds on the price of anarchy in the controlled allocation platforms as a function of the objective function being optimized by the platform. }
% We present a generalized result over the. 
% \sam{Sam: I think the first sentence in the above paragraph would be too cavalier. }
\rone{\begin{theorem}\label{thm:generalcap}
    \sam{Assume that there are at least $m \geq 2$ markets.} The price of anarchy $\rho(\lambda,M)$  in  controlled allocation platforms satisfies: 
    %(characterized by $\sigma=\frac{2-3\lambda }{1 - \lambda}$) 
% \begin{equation*}
% \rho(\lambda,M) \geq 
% \begin{cases}
% \infty, ~ \text{if $\frac{2-3\lambda }{1 - \lambda} \leq 0$. }\\
% \frac{8|M|}{9},~\text{if $0 < \frac{2-3\lambda }{1 - \lambda} \leq 1$}\\
% \max\{\frac{2}{3\sqrt{\frac{1-\lambda}{2-3\lambda}\left(1-\frac{1-\lambda}{2-3\lambda}\right)}},\frac{3}{2}\}, ~\text{otherwise}.
% \end{cases}
% \end{equation*}
% \eb{\begin{equation*} 
% \rho(\lambda,M) \geq 
% \begin{cases}
% \max \left\{ \displaystyle\frac{3}{2}, \  \frac{2(2-3\lambda)}{3\sqrt{(1- \lambda)(1 - 2 \lambda)}} \right\},  &  \textrm{if} \ \  \lambda \in [0, \, 1/2)\\
% \displaystyle\frac{8|M|}{9}, & \textrm{if} \ \ \lambda \in [1/2, \, 2/3) \\
% \infty, & \textrm{if} \ \ \lambda \in [2/3, \, 1]\\
% \end{cases}
% \end{equation*}}
% \rone{\begin{equation*} 
% \rho(\lambda, M) \geq 
% \begin{cases}
% \max \left\{ \displaystyle\frac{3}{2}, \  \frac{2\lambda^2}{3((2\lambda - 1)(1-\lambda) + \sqrt{(1- \lambda)(1 - 2 \lambda)(1-3\lambda+3\lambda^2)})} \right\},  &  \textrm{if} \ \  \lambda \in [0, \, 1/2)\\
% \displaystyle\frac{8m}{9}, & \textrm{if} \ \ \lambda \in [1/2, \, 2/3) \\
% \infty, & \textrm{if} \ \ \lambda \in [2/3, \, 1]\\
% \end{cases}
% \end{equation*}}
\begin{equation*} 
\rho(\lambda, M) \geq 
\begin{cases}
\max \left\{ \displaystyle\frac{3}{2}, \  \frac{2}{3}\left(1+\sqrt{1+\frac{\lambda^2}{(2 \lambda -1)(\lambda -1)}}\right)  \right\},  &  \textrm{if} \ \  \lambda \in [0, \, 1/2)\\
\displaystyle\frac{8m}{9}, & \textrm{if} \ \ \lambda \in [1/2, \, 2/3) \\
\infty, & \textrm{if} \ \ \lambda \in [2/3, \, 1]\\
\end{cases}
\end{equation*}
\end{theorem}}

\sam{
If we let the number of markets $m \to \infty$, then the lower bound on the price of anarchy in controlled allocation in Theorem \ref{thm:generalcap} increases from $3/2$ to $+\infty$ as $\lambda$ increases from 0 to $1/2$, and remains $+ \infty$ for $\lambda \in [1/2, 1]$. Such a trend in the price of anarchy bound shows that the efficiency loss stemming from the incentive for production withholding potentially decreases as we increase the extent to which the platform's objective favors firms.
}

% \sam{The crux of the proof of Theorem \ref{thm:generalcap} relies on the construction of specific platform examples where production withholding results in a large loss of efficiency at Nash equilibrium. Specifically, for the case in which $\lambda \in [2/3, 1]$, one can construct a sequence of two-market examples where the ratio of the aggregate production quantity at Nash equilibrium to the efficient aggregate production quantity goes to zero asymptotically. For the case in which $\lambda \in [0, 2/3)$, one can construct examples where the aggregate supply is strictly positive in each market at the efficient production profile, but zero in all but one market at Nash equilibrium. We refer the readers to the Appendix for the details of the proof.}

% \sam{Theorem \ref{thm:generalcap} reveals that controlled allocation platforms can exhibit a large loss of efficiency at Nash equilibrium due to production withholding by firms. One possible approach to  production withholding behavior is to adopt market clearing mechanisms that favor the producers. Specifically,  under the restriction to the case where $\lambda \in [0, 1/2)$, the price of anarchy lower bound is strictly increasing in $\lambda$. This reveals the possibility that increasing the extent to which the platform favors consumers might lead to increasing efficiency loss. The formal investigation of such an intuition, however, is left as a direction for future work.}

The results contained in this section reveal that the  explicit control of the allocation of supply to each market by the platform can result in  production withholding by firms and large efficiency loss at Nash equilibrium. \eb{In the following section, we explore an alternative approach to platform control, where the platform employs a moderate approach to control by restricting the set of markets that different firms are given access to, while allowing firms to freely determine their individual production levels in each market. We refer to such platforms as \emph{discriminatory access platforms.}}







% \sam{Sam: I think we probably only need to include three paragraphs after Theorem 3:
% \begin{itemize}
%     \item A paragraph that illustrates the role of production withholding in increasing in efficiency loss in controlled allocation platforms
%     \item A paragraph on the proof intuition
%     \item A lead up into the next section
% \end{itemize}
% Also, can you provide the bound in a way that reveals the monotonicity of the bound in $\lambda$ more clearly? More specifically, is the bound monotonic in $\lambda$ for $\lambda \in [0, 1/2)$?
% }

% \johnp{John: Thanks for the simplification! The first of the next three paragraph revolves around how production withholding happens in these examples, and provides some further intuition to the proof for the social welfare case. The next paragraph aims to talk about how the proofs generalize, and what the differences are. The last paragraph summarizes the issues of controlled allocation platforms and introduces discriminatory access platforms... }

% \sam{Sam: I think you can actually show that
% $$\frac{\lambda^2}{(2\lambda - 1)(1-\lambda) + \sqrt{(1- \lambda)(1 - 2 \lambda)(1-3\lambda+3\lambda^2)}} = \sqrt{1 + \frac{1}{\eta}} + 1,$$
% where $\eta := 2 - \frac{3}{\lambda} + \frac{1}{\lambda^2}$. The method for deriving this is to express the LHS as a function of $(1 - \lambda)( 1- 2 \lambda)$ and $\lambda^2$. Can you help me verify that my claim is correct?}

% \sam{Sam: I think the PoA lower bound requires the assumption that the number of markets $m \geq 2$. Otherwise the Stackelberg game is equivalent to the Cournot game and has a PoA of 3/2.} \johnp{John: I think it's fine actually. Perhaps we can put $\max \left\{\frac{3}{2},\frac{8m}{9}\right\}$ for the second set of $\lambda$ values too to be consistent and add that the $3/2$ can be essentially inferred from the equivalence of Cournot and Stackelberg in the $m=1$ setting? Will that be ok? }

% \rone{Essentially, for all market clearing mechanisms defined by $\lambda \in [2/3,1]$, the price of anarchy of a Stackelberg game can be unboundedly large even in the case where $m=2$.} It turns out that the construction developed to prove Theorem \ref{thm:ineff} also can be used to show that any objective between consumer surplus and social welfare leads to similar results to the social welfare case in Theorem \ref{thm:ineff}. \rone{When $\lambda \in [1/2,2/3)$, the price of anarchy grows at least linearly in the number of markets $m$. Lastly, if $\lambda \in [0,1/2)$, the price of anarchy still increases in $m$ but in a sub-linear manner, and for clarity, we present the price of anarchy result as $m$ grows infinitely large. }

% \rone{The examples for $\lambda \in [0,2/3)$ are constructed with production withholding in mind. In each of them, the market parameters are set up such that a single zero cost producer is incentived to produce only enough for the platform to allocate to the market with the largest willingness to pay. Thereafter, production would be allocated in a way where profit does not increase. In particular, in proving Theorem \ref{thm:ineff}, or equivalently for $\lambda = 1/2$, the example has a firm with zero production cost, and it follows that the socially efficient production is always to produce until the price in every market is driven to~$0$. The construction of markets begins with a single market and then, as markets are added one by one to the system, the parameters of each new market are such that the firm has no incentive to increase production as profit do not increase due to the decreased unit prices, whereas the socially efficient welfare increases linearly in the number of markets.}

% \rone{We provide the following proof idea for the cases where $\lambda \in (1/2,2/3)$, while the entire proof can be found in the Appendix.  One can show that the unit price based on the corresponding allocation function for $\lambda \in (1/2,2/3)$ is no more than that of the $\lambda = 1/2$ case, thereby obtaining at least the same price of anarchy, which grows linearly with the number of markets $m$. Lastly, when $\lambda \in [0,1/2)$, the platform transitions to other markets sooner, which increases the unit price as compared to that of the $\lambda = 1/2$ case. However, by carefully adjusting the market parameters, the general structure of the example still hold. However, the addition of each market has a diminishing effect on the efficient social welfare, similar to a geometric progression where the common ratio is determined by, and decreasing, as $\lambda$ decreases. An intuition for why a $\lambda=0$ (i.e., revenue maximizing) controlled allocation platform is less inefficient is that the platform's allocations are more aligned with the producers, providing them less incentive to withhold production. For example, in the case of a single producer, such a platform will indeed allocate as the single producer would choose to if it were itself participating in an open access platform. For clarity of presentation, we present the price of anarchy result for the $\lambda \in [0,1/2)$ case when the number of markets $m$ approaches $\infty$. One can check that this term is indeed monotonically increasing in $\lambda$. Following the proof found in the Appendix, one can obtain similar bounds which are dependent on $m$ as in the $\lambda \in [1/2,2/3)$ case. On the other hand, the examples used in the $\lambda \in [2/3,1]$ cases are only slightly modified from that of the consumer surplus case. Essentially, by keeping the maximal willingness to pay equal between the two markets, the platform still allocates in decreasing price elasticity. }


% When considering linear inverse demand functions and assuming $d_j \leq \alpha_j/\beta_j$, $\rm{OBJ}(d;\lambda)$ can be simplified to the following 
% % $$
% % \text{OBJ}(\lambda) = \sum_{j\in M} \left[ \lambda(  \frac{1}{2}\beta_jd_j^2 ) + (1-\lambda)(\alpha_jd_j - \beta_jd_j^2) \right]
% % $$
% % or equivalently, by 
% after dividing by a constant $(1-\lambda)$ assuming $\lambda \neq 1$ (having dealt with the consumer surplus case in the previous subsection),
% $$
% \frac{1}{1-\lambda} \cdot \text{OBJ}(d;\lambda) = \sum_{j\in M} \alpha_jd_j - \frac{2-3\lambda}{2(1-\lambda)}\beta_jd_j^2
% $$

% Observing the stationarity conditions with respect to $d_j$, we find that the platform maximizing such an objective would keep the following quantity constant across markets: 
% $$
% \frac{1}{1-\lambda} \cdot\frac{\partial \text{OBJ}(d;\lambda)}{\partial d_j} 
% %= \frac{1}{1-\lambda}\left(\lambda(  \beta_jd_j ) + (1-\lambda)(\alpha_j - 2\beta_jd_j)\right) 
% = \alpha_j - \frac{2-3\lambda}{1-\lambda}\beta_jd_j,
% $$
% which confirms that as $\lambda$ approaches $1$, the emphasis on the maximal willingness to pay $\alpha_j$ decreases, and becomes potentially inefficient. Increasing past the point $\lambda=2/3$, the optimization function also changes from a concave maximization problem to a convex one, i.e., the problem ends up being a (nonconvex) Quadratic Program (QP). This also reveals that whenever a new market is accessed (regardless of $\lambda <1$), that the following relationship is preserved for any new additional supply $q_j,~q_k$, 
% $
%  \beta_jq_j = \beta_kq_k, 
% $
% with the parameter $\lambda$ basically dictating when the next market is accessed. For example, when $\lambda = 0.5$, prices are kept constant for each participated market. 

% \sam{The above discussion probably requires some major revisions
%     \begin{itemize}
%         \item As opposed to diving into the details of how the derivative of the objective function changes as a function of $\lambda$, I would instead prefer a discussion on the behavior of the ``bad case" you construct in the proof. For example, you can say that the platform will allocate to all of the supply to a market that has a larger price of elasticity and a lower price. This strongly incentivizes proceducers to withhold production, and will lead to an NE where the total production is zero.
%         \item The proof of Theorem 3 needs to be revised. It seems that the construction of the ``bad case" isn't clear for $\lambda \in [2/3, 1)$. We should spell out the cost function for the producers, the production profile at NE, and the efficient production profile.
%     \end{itemize}
% }
% \johnp{John: Can you check if that's fine? I've also tidied up the proof a little. }

%We can break our analysis into two cases, $\lambda \ge 2/3$ or $\lambda <2/3$, the cases where the coefficient of $\beta_jd_j$ is nonnegative or negative respectively. %One can observe for that any of the cases where $\lambda\ge 2/3$ (as the objective move towards consumer surplus), that the platform would first provide to the market with the smallest maximal willingness to pay.
% \begin{figure}
%     \centering
% 		\includegraphics[width=0.6\linewidth]{poavslambda.eps}
% 		\caption{Price of Anarchy plotted as a function of the objective function's closeness to consumer surplus (distance from revenue). Even the addition of one market for objective functions close to consumer surplus can lead to large inefficiencies (note the logarithmic scale), while objective functions closer to revenue are less affected.  }
% 		\label{fig:poavslambdagraph}
% 	\end{figure}


%While each of them in the $0 < \lambda<2/3$ regime can grow in the number of markets, the effect each objective has on the price of anarchy is different. %To reconcile the conflict towards the transition point $\lambda = 2/3$, we consider a two market scenario whereby adding a market has varied impact on the price of anarchy, illustrated by Figure \ref{fig:poavslambdagraph}, and exhibited in the following result.
	
% 	\begin{proposition}
% 		The worst case price of anarchy by adding a market to a costless firm, one market system is $\frac{4(1+1/\zeta)}{3}$, where $\zeta$ can be shown to be bounded via: 
% 		$$
% 		\zeta > \frac{k^2}{(k-2)^2},
% 		$$ 
% 		where $k = \frac{2-3\lambda}{1-\lambda}$ lies in $[0,2)$. This implies that as the objective approaches revenue maximizing, the effect that adding markets have on the price of anarchy become smaller, while the opposite is also true, that when $k$ is close to $0$, adding one market is sufficient to make the system inefficient.   
% 	\end{proposition}

% The issue with controlled allocation platforms is that the platform's market clearing mechanism is agnostic to underlying cost functions, \rone{which together with price formation being related across markets, can instead incentivize production withholding from the producer side}. While this action seemingly makes much sense under this setting, we show in this section that this can result in unbounded or infinitely large price of anarchy, preserving close to or none of the efficient social welfare. 
% \sam{Our results in this section shows that} a strategy of directly controlling the allocation of supply to each market potentially leads to \sam{undesirable producer behavior---namely, production withholding}. As such, an alternative market clearing mechanism is necessary. \rone{In the following section, we explore the discriminatory access platform which seeks control in a different manner. Specifically, the control in such platforms is performed by restricting the set of markets that each producer have access to. }
% \rone{An intuition for why revenue-maximizing allocations are less inefficient is that the platform's allocations are aligned with the producers, who then have less incentive to withhold production. For example, in the case of a single producer, a revenue-maximizing controlled allocation platform will indeed allocate as the single producer would choose to if it were in an open access platform. This is also the reason for the max operator in the result -- the price of anarchy in a controlled allocation platform cannot outperform that of open access platforms. } %\sam{\textbf{Sam:} can you explain what you meant by saying ``will indeed allocate as the single producer would"?} \johnp{John: Edited...}
	
% 	\sam{Sam: on second thought, I removed the discussion on the limitation of our model that is associated with the absence of capacity constraints. The reason for doing so is that production withholding is still a concrete source of efficiency loss even}
	
% 	\rone{Here, we also note that one of the biggest limitations of the networked Cournot model is that it does not consider capacity constraints. This may weaken the explanatory power of our model in analyzing the sources of efficiency loss in online platforms, as many online platforms arise in the context of “shared economy” and consist of a large number of producers, each of which has limited capacity. In the proof of Theorem \ref{thm:ineff}, we provide a problem instance including $1$ firm and $m$ markets, in which the efficiency loss scales at least linearly in $m$ due to the supply withholding from the one firm. However, this mechanism of exercising market power is not viable in platforms that consist of a large number of producers with small capacities, as the profit maximizing decision for a producer with a small capacity might, instead, be supplying all of its capacity. }


%We consider an objective being the convex combination of consumer surplus and consumer welfare, parametrized by $\lambda$: 
%$$
%\text{OBJ}(\lambda) = \sum_{j\in M} \left[\lambda\left(\int_{0}^{d_j} p_j(q)dq - d_jp_j(d_j) \right) + (1-\lambda)\left(\int_{0}^{d_j} p_j(q)dq\right)\right]
%$$
%For example, when $\lambda = 1$, the above objective is consumer surplus whereas $\lambda = 0$ gives consumer welfare. Similar to the consumer welfare argument, this is true modulo any production cost functions. 
%
%We hope to present a more general version of the results above, i.e. when $\lambda = 0$ (consumer surplus case) or when $\lambda = 1$ (social welfare case), where the price of anarchy is infinitely large and growing linearly in the number of markets. When considering linear inverse demand functions, the above can be simplified to the following: 
%$$
%\text{OBJ}(\lambda) = \sum_{j\in M} \left[ \lambda(  \frac{1}{2}\beta_jd_j^2 ) + (1-\lambda)(\alpha_j d_j - \frac{1}{2}\beta_jd_j^2) \right]
%$$
%
%Taking derivatives with respect to $d_j$, we find that: 
%$$
%\frac{\delta \text{OBJ}(\lambda)}{\delta d_j} = \lambda(  \beta_jd_j ) + (1-\lambda)(\alpha_j - \beta_jd_j)=(1-\lambda)(\alpha_j) - (1 -2\lambda)\beta_jd_j,
%$$
%
%which reveals that as $\lambda \rightarrow 1$, the emphasis on the maximal willingness to pay $\alpha_j$ decreases, and becomes potentially inefficient. This also reveals that whenever a new market is accessed (regardless of $\lambda <1$), that the following relationship is preserved for any new additional supply $q_j,~q_k$: 
%$$
%\forall \text{markets }j,k,~ \beta_jq_j = \beta_kq_k. 
%$$
%The parameter $\lambda$ basically dictates when the next market is accessed. For example, when $\lambda = 1$, prices are kept constant for each participated market. We can break our analysis into two cases, $\lambda \ge 1/2$ or $\lambda <1/2$, the cases where the coefficient of $\beta_jd_j$ is positive or negative. One can observe for that any of the cases where $\lambda\ge1/2$ (as the objective move towards consumer surplus), that the platform would insist on providing only to the market with the largest maximal willingness to pay and fails to take into consideration price elasticity with respect to demand. We prove the following claim informally: 
%
%\begin{theorem}
%	For all $\lambda\ge 1/2$, the price of anarchy of a controlled allocation platform maximizing OBJ$(\lambda)$ has infinitely large price of anarchy. On the other hand, for $0 < \lambda<1/2$, the price of anarchy grows with $M$, where $M$ is the number of markets. 
%\end{theorem} 
%
%In this regime, the coefficient of $\beta_jd_j$ is negative. This means that allocation is done in a counter-intuitive manner, and that the market with the lowest willingness to pay is allocated to first, which can certainly be manipulated to provide an infinitely large price of anarchy. For example, consider a quadratic cost function $cq$ such that $c>\alpha_M$, where $\alpha_M$ correspond to the lowest maximal willingness to pay among all markets. Consider further that the corresponding price elasticity in that market is $0$. In this case, the producer have no incentive to produce at all, since every quantity results in a loss, and will also never move on to another market since $\beta_M=0$. 
%
%On the other hand, when $\lambda<1/2$, we can design a series of markets for a costless firm with a resulting price of anarchy that grows in the number of markets accessed, similar to the social welfare maximizing platform ($\lambda=1$ case).
%
%We will prove the existence of such families of markets in the following series of lemmas, as follow: 
%
%\begin{lemma}\label{lem:allocationm}
%	Regardless of the parameter $ \lambda < 1/2 $ for one costless firm, optimal aggregate production for it maximizes social welfare, i.e. $q^* = \sum_{j\in M} \frac{\alpha_j}{2\beta_j}$.
%\end{lemma}
%
%Following the social welfare maximizing case, we want to design markets such that the maximal profits obtained at the introduction of each consecutive markets lead to the same profit, and so any of the equilibria have the same profit but results in different social welfare (since the firm has no cost), and where the optimal social welfare allocation satisfies all demand. 
%
%
%
%\begin{lemma} \label{existbeta}
%	If $1>\theta>k$, and $k>\frac{4+4\theta-8\theta^2}{2\theta^2+2}$, then there is at least one positive solution for $\beta_m$ such that there is a series of markets that result in the same profit with the inclusion of each market.
%\end{lemma}
%
%
%
%Controlling allocation assuming fixed supply quantities intuitively implies that the platform does not consider production costs and neglect considering the welfare of producers and accidentally put too much focus on consumers instead. While this action seemingly makes much sense under this setting, we show above that having the wrong objectives can yield (in the extreme) unbounded and infinite price of anarchy, preserving close to or none of the optimal social welfare. 
%
%It should be clear that such a strategy of controlling allocations potentially leads to undesirable producer behavior and that an alternative mode of optimizing the system is necessary. 


%\begin{lemma}
%	For any cubic function of the form $f(x) = x^3 + ax^2 + bx + c$, one can make a transformation $x=y-a/3$, recovering the normal form $g(y) = y^3 + py + q $, where $p,~q$ are defined as follows: 
%	\begin{enumerate}
%		\item $ p = \frac{1}{3}(3b - a^2)$
%		\item $q = \frac{1}{27}(2a^3 -9ab +27c)$
%	\end{enumerate}
%	and the normal form equation has the following three roots: 
%	\begin{enumerate}
%		\item $y_1 = A+B$, 
%		\item $y_2 = -\frac{1}{2} (A+B) + \frac{i\sqrt{3})}{2}(A-B)$
%		\item $y_3 = -\frac{1}{2} (A+B) - \frac{i\sqrt{3})}{2}(A-B)$
%	\end{enumerate}
%where $A = \sqrt[3]{-\frac{q}{2}+\sqrt{\frac{q^2}{4}+\frac{p^3}{27}}}$ and $B=\sqrt[3]{-\frac{q}{2}-\sqrt{\frac{q^2}{4}+\frac{p^3}{27}}}$. 
%
%\end{lemma}
%%\begin{enumerate}
%%	\item if $c<0$, then the function have at least one positive solution. Equivalently, we require $\frac{d_{\text{new}}}{a_{\text{new}}}>0$.
%%	\item if $f$ has real roots, and the signs are alternatively positive and negative, i.e., $a<0$, $b>0$ and $c<0$, then all three roots are positive. 
%%\end{enumerate} 
%These are basic identities in algebra, which we assume are familiar to the reader. 
%
%Expanding on the coefficients from before and normalizing by $a_{\text{new}}$, we get: 
%$$
%a_{\text{new}} = \frac{1}{L} \left[ \sum_{j=1}^m \frac{(1+\theta - 2\theta^2)\alpha_{m+1}^2 +(\theta- k)\alpha_j\alpha_{m+1} }{k\beta_j} \right],
%$$
%$$
%b_{\text{new}} = 4 + \frac{  \left[\sum_{j=1}^m -\frac{\theta\alpha_{m+1}(\alpha_{m+1} + \alpha_j) }{L\beta_j} \right] - \alpha_{m+1}^2 \left[ 1-\theta +\frac{2\theta^2 -1-\theta}{k}  \right]}{\frac{1}{L} \left[ \sum_{j=1}^m \frac{(1+\theta - 2\theta^2)\alpha_{m+1}^2 +(\theta- k)\alpha_j\alpha_{m+1} }{k\beta_j} \right]},
%$$
%$$
%c_{\text{new}} = (12a+4b+c),
%$$
%$$
%d_{\text{new}} = 8a + 4b + 2c + d,
%$$

==> 2020_ OR_ Net Cournot and Platforms/discplatform.tex <==

\eb{In this section, we investigate a class of  \emph{discriminatory access platforms} that aim to strike a balance between open access and controlled allocation platform designs, in order to improve upon on the worst case efficiency loss of both. As a compromise between these two extremes, discriminatory access platforms exercise a form of limited control in the marketplace by restricting the set of markets that different firms are given access to, while allowing firms to freely determine their individual production levels in each market.  Platforms designs of this kind are reminiscent of Amazon's \emph{Buybox} and Airbnb's \emph{Superhost} mechanisms, which selectively display particular suppliers to customers, while hiding others.}



%  Open access designs preserve large productions but suffer from misaligned allocations, while controlled allocation designs lead to undesirable and unintended incentives for the producers to curtail production. Recently, some platforms have started shifting from open access platform designs towards more delicate designs which aim to both retain the incentive to produce in open access platforms and exert some control over allocations. Results from this section show the promise of some of these changes. We design such a platform to be similar to mechanisms such as Amazon's Buybox and Airbnb's Superhost, which highlights particular sellers or renters while hiding others.  

%While many early platforms relied on an open access model, besides controlling allocations, recent platforms have also begun to exercise control over the set of markets to which each firm has access, restricting access and not controlling allocation as in the previous platform. 

In the context of our model, this form of access control  corresponds to the specification  of the edge set $\Ecal \subseteq F \times M$ in the bipartite graph that determines connections between firms and markets, with the goal of maximizing social welfare at the unique Nash equilibrium of the resulting networked Cournot game (cf. problem \eqref{opt:network}). 
% This platform is referred to as a \emph{discriminatory access platform} in this paper. 
Importantly, unlike the controlled allocation platforms, the efficiency loss of discriminatory access platforms is guaranteed to be no worse than that of open access platforms, since open access designs represent a particular approach to access control.
%In doing this, the platform seeks to block access of each firm to markets where its participation might decrease market efficiency, i.e., decrease social welfare.

\eb{Utilizing an assumption of \emph{linearity} of the firms' cost functions, in Theorem \ref{thm:discriminatory_PoA}, we provide  an explicit bound on the price of anarchy  in discriminatory access platforms} under the optimal network design.
%  Our work on discriminatory access design culminates in the following result, 
 We build on this result in Theorem \ref{thm:greedy-alg}, showing that the optimal network design can be  computed using an intuitive greedy algorithm that we specify later in the section. 

\begin{theorem} \label{thm:discriminatory_PoA}
    % Assume that each firm's cost function is linear over $(0, \infty)$, and assume that $\Ecal^*$ is the optimal network design for the discriminatory access platform.
% 	Assume that each firm's cost function is linear over $(0, \infty)$. If $\Ecal^*$ is the edge set generated by the greedy algorithm, then $\left( \Ecal^*, q^{\rm NE} (\Ecal^*) \right)$ is an optimal solution to $(9)$, that is, the greedy algorithm achieves the optimal network design. 
	Let $C \in \Lcal^n (c_{\min}, c_{\max})$  and assume that $c_{\min} < \max_{j\in M} \alpha_j$.  Additionally, let $\Ecal^* \subseteq F \times M$ denote the network structure that maximizes the  social welfare derived  under discriminatory access platforms at Nash equilibrium according to problem \eqref{opt:network}. The efficient social welfare associated with the edge set $\Ecal^*$ satisfies
	$$\SW^* (\Ecal^*, C) = \SW^* (F \times M, C).$$
% 	The efficient social welfare can be attained at the edge set $\mathcal{E}^*$. 
	Moreover, the price of anarchy of the corresponding networked Cournot game $(F, \mathcal{Q}(\Ecal^*), \pi)$ is upper bounded by
	\begin{align*}
	\rho (\Ecal^*, C) 
	\leq \dfrac{\displaystyle\sum_{j=1}^m  \frac{\left( (\alpha_j - c_{\min} )^+ \right)^2}{\beta_j}}{\displaystyle\sum_{j=1}^m \underset{k \in \{1, .., n\}}{\max}\left\{ \frac{2k+4}{3k+5}  + \delta (\gamma_j, k) \right\} \frac{ \left( (\alpha_j - c_{\min} )^+ \right)^2}{\beta_j}}.
	\end{align*}
	Recall that the function $\delta(\cdot,\cdot)$ (originally defined in Proposition \ref{prop:PoA_cmin_cmax})  measures the degree of asymmetry in the firms' cost profile. Finally, the above bound on the price of anarchy is tight if $\alpha_1 = \alpha_2 = \cdots = \alpha_m$.
\end{theorem} 
\eb{It is important to note that, while we have restricted ourselves to linear cost profiles in Theorem \ref{thm:discriminatory_PoA}, the upper bound on the price of anarchy that we have derived also holds in the more general setting where firms' have convex cost functions. This follows from Lemma \ref{Lem:WorstCaseLinear}, which shows that, among all convex cost profiles,  linear cost profiles result in the greatest loss of efficiency at equilibrium.}
% The functions that maximize worst case efficiency loss in networked Cournot games are linear cost functions. Therefore, by optimizing based on the linear cost functions, we are sure the bound in Theorem \ref{thm:discriminatory_PoA} also applies to cases where firms have general convex costs. 
\eb{Additionally, the upper bound on the price of anarchy that we provide is maximized at $n=1$, resulting in 
a price of anarchy bound} of $4/3$ that holds for \emph{optimized} discriminatory access platforms with any number of firms and markets. This improves substantially upon the $3/2$ upper bound on the  price of anarchy in open access platforms (cf. Corollary \ref{cor:poabound}). The result is formally stated as follows. 
\begin{corollary}%[Corollary to Theorem \ref{thm:discriminatory_PoA}]
	\label{cor:nine}
	%Assume that each firm's cost function is linear over $(0, \infty)$.
	%Let $C \in \Lcal^n (c_{\min}, c_{\max})$  and assume that $c_{\min} < \max_{j\in M} \alpha_j$. 
	The price of anarchy of optimized discriminatory access platforms is at most $4/3$. 
	%That is, if the discriminatory access platform chooses the edge set according to an optimal solution of problem \eqref{opt:network}, then the social welfare at the unique Nash equilibrium of the discriminatory access networked Cournot game is at least $3/4$ of the efficient social welfare.
\end{corollary}

% \ebc{(Eilyan says: Sam, do we need the assumption of linearity in light of Lemma 2?)}

% In general, we show that choosing an optimal edge set that maximizes social welfare at Nash equilibrium amounts to a mathematical program with equilibrium constraints (MPEC), and is, in general, computationally intractable. %However, under the simplifying assumption that each firm's cost function is linear on $(0, \infty)$ (which corresponds to the worse case scenario as a result of Lemma \ref{Lem:WorstCaseLinear}), we present a greedy algorithm that is guaranteed to generate an optimal solution to the MPEC. We then present a tight price of anarchy bound for the networked Cournot game that results under the optimal network design with the bound revealing the reduction in efficiency loss achievable through discriminatory access platforms over an open access one.


\eb{In contrast to controlled allocation platforms, which suffer from an unbounded price of anarchy, the price of anarchy of optimized discriminatory access platforms is not only guaranteed to be bounded, but also improves upon the  worst case efficiency loss  of open access platforms.}


% \rone{In comparison to controlling allocations, which leads to unbounded worst case loss, by controlling access we achieve a bounded worst case efficiency loss result. In addition, the worst case efficiency loss bound is improved from $3/2$ under open access to $4/3$ under discriminatory access. }

\subsection{The Optimal Network Design Problem}

The optimal network design problem amounts to the selection of an 
edge set $\Ecal$ that maximizes social welfare at the unique Nash equilibrium of the resulting networked Cournot game. Formally, Lemma \ref{lem:NE} provides a characterization of the supply profile at the unique Nash equilibrium of the game $(F, \Qcal (\Ecal), \pi)$ as the unique optimal solution to a convex program. Therefore, the \emph{optimal network design problem} can be formulated  as the  following mathematical program with equilibrium constraints (MPEC):
\begin{equation} \label{opt:network}
\begin{alignedat}{8}
& \text{maximize} \quad && \SW (q, C) \\
& \text{subject to} \quad && \Ecal \subseteq F\times M \\
&&& q \in \underset{x \in \Qcal (\Ecal) }{\argmax} \left\{ \SW (x, C) - \sum_{j=1}^m  \sum_{i=1}^n \frac{\beta_j x_{ij}^2}{2}  \right\}
\end{alignedat}
\end{equation}
Here, the decision variables are the edge set $\Ecal$ and the supply profile $q$. 
The challenge in solving the above problem the presence of the discrete decision variables $\Ecal$, and the equilibrium constraint on $q$. An equilibrium constraint requires that a decision variable be an optimal solution to a optimization problem. In general, this can result in o a nonconvex and disconnected feasible region. See \citet{luo1996mathematical} for a more detailed discussion.
%The MPEC \eqref{opt:network} is, in general, a nonconvex optimization problem with disconnected feasible region. It is therefore computationally intractable, in general. We refer the readers to \citet{luo1996mathematical} for a discussion on the difficulty in solving MPECs.
In what follows, we show that, when considering linear cost profiles, the proposed MPEC \eqref{opt:network}  can be efficiently solved using a greedy algorithm.   


%\john{due to the disconnectedness of its feasible region \citet{luo1996mathematical}}

%Given a cost function profile $C$ that consists of arbitrary convex cost functions, the calculation of the optimal solution for problem \eqref{opt:network} is, in general, computationally intractable. 

%Nonetheless, one may still procure reasonable approximations of problem \eqref{opt:network}, or solve problem \eqref{opt:network} to its full optimality, under simplifying assumptions on the underlying cost function profile. 
%In what follows, we show that given the simplifying assumption that firms have cost functions that are linear on $(0, \infty)$, the optimal network design problem \eqref{opt:network} can be solved by a simple greedy algorithm. 

%\sam{Add a transition to linear cost function results here. Mention problems of finding approximately optimal solutions in the footnote and the conclusion section.}

%Finding the optimal network design problem as in \cref{opt:network} is hindered both by the equilibrium constraint on $q$, and the presence of a combinatorial variable set $\Ecal$.

% This sheds light on the difficulty of the problem from two fronts: (i) The feasible region of the problem is a combinatorial set; which usually results in NP-hard problems; and (ii) an inner problem needs to be solved to obtain the corresponding outer feasible solution. 

\subsection{Greedy Algorithm for Optimal Worst-case Network Design}
In this section, we restrict ourselves to cost functions that are linear over $(0, \infty)$.
%i.e., the ones maximizing worst case efficiency loss. 
Specifically, we assume that the cost function of each firm $i \in F$ satisfies
$C_i (s_i) = (c_i s_i)^+$,  where $c_i \geq 0$. 
Leveraging on the assumption of linearity, we propose a greedy algorithm  that is shown to solve the optimal network design problem \eqref{opt:network}. At a high level, the proposed greedy algorithm functions as follows.
For each market $j \in M$, the greedy algorithm visits firms in ascending order of marginal cost, and provides each firm that it visits access to market $j$ if its inclusion in that market increases social welfare at equilibrium. 




\begin{algorithm}
	\caption{The Greedy Algorithm}\label{alg:linearDis}
	\begin{algorithmic}[1]
		%\Procedure{GLD}{$\demlim,\demrate,\cost$}\Comment{Returns optimal set of Firms}
		\Require $c_1 \leq \cdots \leq c_n$.      
		\State Initialize edge set $\Ecal \gets \emptyset$.
		%      \State Initialize $q \gets 0$.
		
		\For{$j=1$ to $m$}
		\State Initialize firm index $i \gets 1$.
		\State Initialize edge set $\widetilde{\Ecal} \gets \Ecal$.
		%      	\State Initialize $\widetilde{q} \gets q$.
		\Repeat
		\State Update edge set $\Ecal \gets \widetilde{\Ecal}$.
		%      		\State Update supply profile $q \gets \widetilde{q}$.
		\If{$i \leq n$}
		\State Set edge set $\widetilde{\Ecal} \gets \Ecal \cup (i, j)$.
		%      			\State Set $\widetilde{q} \gets q_{\rm NE} (\widetilde{\Ecal})$.
		\State Set firm index $i \gets i + 1$.
		\EndIf
		\Until{$\SW (q^{\rm NE} (\widetilde{\Ecal} ), C) \leq \SW (q^{\rm NE} (\Ecal), C)$}.
		\EndFor
		
		\State 
		\Return $\Ecal$.
		%\EndProcedure
	\end{algorithmic}
\end{algorithm}

%\red{\cref{alg:linearDis} is guaranteed to terminate within $mn$ iterations, where each iteration takes time that is polynomial in $mn$.}
% The following result establishes optimality of the greedy algorithm when firms' cost functions are linear over $(0, \infty)$.
%Its proof is provided in the Appendix.
%can be found in the extended version of this paper \citet{linpangbitarwierman2017}. 

% \begin{theorem} \label{thm:greedy_opt}
% 	Assume that each firm's cost function is linear over $(0, \infty)$. If $\Ecal^*$ is the edge set generated by the greedy algorithm, then $\left( \Ecal^*, q^{\rm NE} (\Ecal^*) \right)$ is an optimal solution to $(9)$.
% \end{theorem}


%\red{The key idea in the proof of \cref{thm:greedy_opt} is that for any edge set $\Ecal \subseteq F \times M$, one can construct a sequence of modifications to this edge set that recovers the edge set $\Ecal^*$. Moreover, the social welfare at Nash equilibrium is non-decreasing after each modification in this sequence.}

%The key idea in the proof of \cref{thm:greedy_opt} is that for any edge set $\Ecal \subseteq F \times M$, one can construct another edge set, whose social welfare at Nash equilibrium is no smaller than that of $\Ecal$, and no larger than that of $\Ecal^*$. 
%The proof of \cref{thm:greedy_opt} can be found in the extended version of this paper \citet{linpangbitarwierman2017}.  


It is not difficult to see that Algorithm \ref{alg:linearDis} yields an edge set $\Ecal^* \subseteq F \times M$ that induces a  Nash equilibrium whose social welfare  is no smaller than that of the open access platform. %Its proof is deferred to the Appendix.

\begin{theorem}\label{thm:greedy-alg}
Let $\Ecal^*$ be an edge set obtained from Algorithm \ref{alg:linearDis}. It follows that   $(\Ecal^*,q^{\textrm NE}(\Ecal^*))$ is an optimal solution to the MPEC $(\ref{opt:network})$.
% that is, the greedy algorithm achieves the optimal network design.  
\end{theorem}



%then both of the following statements are true
%\begin{enumerate}[(i)]
%\item The efficient social welfare associated with the edge set $\Ecal^*$ and the cost function profile $C$ satisfies 
%$$\SW^* (\Ecal^*, C) = \SW^* (\Kcal_{F, M}, C).$$
%\item The price of anarchy associated with the discriminatory access networked Cournot game $(F, \mathcal{Q}(\Ecal^*), \pi)$ and the cost function profile $C$ is upper bounded by
%\begin{align*}
%\hspace*{-0.8cm}\rho (\Ecal^*, C) 
%\leq \dfrac{\sum_{j=1}^m  \frac{\left( (\alpha_j - c_{\min} )^+ \right)^2}{\beta_j}}{\sum_{j=1}^m \underset{k \in \{1, .., n\}}{\max}\left\{ \frac{2k+4}{3k+5}  + \delta (\gamma_j, k) \right\} \frac{ \left( (\alpha_j - c_{\min} )^+ \right)^2}{\beta_j}}.
%\end{align*}
%The above bound is tight if $\alpha_1 = \cdots = \alpha_m$.
%\end{enumerate}


While Theorem \ref{thm:discriminatory_PoA} reveals a key advantage that optimized discriminatory access platforms have over open access platforms in terms of limiting efficiency loss at equilibrium, Theorem \ref{thm:greedy-alg} provides an algorithmic approach to efficiently  to  compute the optimal network structure in discriminatory access platforms. 

% Namely, when the edge set is chosen to be an optimal solution of the network design problem $(9)$, the discriminatory access platform is guaranteed to have a tight bound on the price of anarchy that is no larger than that of the open access platform.
% Moreover, this price of anarchy bound is guaranteed to be non-increasing in the number of firms $n$.



% Additionally, as the degree of asymmetry between firms' cost functions decreases, the price of anarchy bound for discriminatory access platforms gets close to that of open access platforms. More specifically, we consider the choice of $k^* \in \{1, .., n\}$ that maximizes $\frac{2k+4}{3k+5}  + \delta (\gamma, k)$, as a function of $\gamma$. 
% If $\gamma \leq 17/22$, the above maximum is attained by $k^* = 1$; whereas if $17/22< \gamma < 1$, $k^*$ satisfies
% $$k^* \in \left\{ \min \left\{ \left\lfloor  \frac{3\gamma - 2}{1 - \gamma} \right\rfloor, n \right\},  \  \min \left\{ \left\lfloor  \frac{3\gamma - 2}{1 - \gamma} \right\rfloor + 1, n \right\} \right\}.$$
% Clearly, as $\gamma $ increases, $k^*$ increases. In particular, for a fixed number of firms $n$, if $\gamma_j \geq 1 - 1/ (n+3)$ for each market $j \in M$, the price of anarchy bounds for open access and discriminatory access platforms become identical.

%Additionally, under the assumption of a linear cost function profile,  a straightforward calculation involving the price of anarchy bound in \cref{thm:discriminatory_PoA} 



%\sam{Suggestion on corollary statement: might get rid of everything after ``that is''}
% \begin{corollary}
% 	\label{cor:nine}
% 	Assume that each firm's cost function is linear over $(0, \infty)$. Discriminatory access platforms have a price of anarchy of at most $4/3$. %That is, if the discriminatory access platform chooses the edge set according to an optimal solution of problem \eqref{opt:network}, then the social welfare at the unique Nash equilibrium of the discriminatory access networked Cournot game is at least $3/4$ of the efficient social welfare.
% \end{corollary}

% We observe under our model that sacrificing transparency and discriminating choices of firms for different markets allow for a slight improvement in the worst case social welfare preserved, or a slight improvement in efficiency. 

%In what follows, we present a simple search cost model to study the impacts of consumer search cost on platform design, and further demonstrate the flexibility of the discriminatory access platform design to consider search costs.   


==> 2020_ OR_ Net Cournot and Platforms/intro.tex <==
%intro 
% Organizations like eBay, Uber and Amazon are undoubtedly one of today's largest and fastest growing companies, and every other start-up today attempts to be the next Uber for a different service sector, e.g., Snappr for photography, Care for babysitting, Airbnb for peer-to-peer short-stay home rentals, Kickstarter for start-up financing, and many more. In today's increasingly connected world, people are willing to exchange limited amounts of information, privacy and control to allow these organizations or entities to make decisions collectively for us. The estimated market value of some of these organizations alone is $\$ 4$ billion US dollars, a huge proportion of the $\$ 24$ billion US dollar market value on the top $500$ companies in the US listed on NASDAQ or NYSE.  These companies are also among the fastest growing ones out there today, and will only continue to accelerate in expansion in the future, as the next wave of digital revolution take place. These organizations have similarities - all of them seek to lower entry costs for ``producers", allow for small businesses to compete with larger organizations, utilize technology and information to improve matches between consumers and producers, and essentially, all of them are platforms and seek to bring together multi-sided markets. 

% Platforms are intermediaries that facilitate interactions between two or more groups where decisions made by one group have effects on the other group either directly or indirectly. An important characteristic of platforms is that they \emph{usually do not themselves produce nor consume}, but play the role of an intermediary and arrange matches between sides informatively, facilitating a safe and simple trading process, providing value for all sides (not necessarily equally), decreasing search cost for consumers, entry cost for producers, and often optimizing a global objective such as social welfare (for long-term, continued growth and expansion) or revenue (for short-term profits). Platforms are not new and have been around for a long time, but have recently rode on the internet technology wave towards an unprecedented success - the success of online platforms and marketplaces. 

% In the past, platforms include television networks that bring together advertisers and program viewers. As more viewers come on board, the network has more leverage on advertisers while if there is more revenue from advertising, the network can produce or air better shows to bring in more viewers. Online platforms today rely on this same theory to profit from what appears to be complimentary services provided to participants, e.g., Facebook's social media network relies on revenue from ads. Another platform that have been around for centuries are auctioneers that help offload valuable goods, oftentimes providing perks for interested and potential buyers. Today, eBay and Amazon have taken over this realm and are expanding in scale every day. Facebook, eBay and Amazon are but some examples in the world of online platforms today, that include also ridesharing platforms like Uber, Lyft, Grab, Didi and Blablacar. From an economist's point of view, the variety of market or platform design in each of these platforms (serving a common use case) provide an excellent set of examples to study. The emphasis in our work is on the effect of access and allocation control on the performance of these platforms. 



% %Each of these platforms belong to a certain type as defined in \citet{evans2016matchmakers}, namely \textit{exchanges} (e.g., eBay, Amazon), \textit{advertiser-supported media} (e.g., Facebook and Google AdWords), \textit{transaction systems} (e.g., Venmo, Paypal) and \textit{hardware/software platforms} (e.g., Apple App Store or Google Play Store). Our work focuses on the exchanges platform and look further into different platform designs with correspondingly different interactions between the two sides of each platform, and its resulting efficiency. %At a high level, one may also interpret our work for the other types but with different objectives.

% The design and operation of online platforms are extremely diverse. Having our focus on access and allocation control, platforms today differentiate themselves by either controlling for interactions at a fine-grained level, e.g., Uber, or allow for interactions to move very freely, e.g., eBay. In between, there are platforms like Amazon with its Buybox design (or respectively Airbnb with its Superhost program) that selectively withhold (present) information from (to) buyers in expectation of improving their overall shopping (staying) experience \citet{chen2016empirical,liang2017superhost}, restricting the interactions between buyers and sellers. In this work, we focus on the \emph{efficiency loss from various platform designs on access and allocation control}, referring to platforms like eBay as \emph{open access platforms}, where the platform provides information and allow all possible matches. We also introduce \emph{discriminatory access platforms}, which are exemplified by platforms that restrict information and matches, such as Amazon. Lastly, we include a platform like Uber, which we term \emph{controlled allocation platforms}, which allows firms to make decisions on their production, but decide on where each firm produces to, maximizing a certain measure of performance, e.g., for ride-sharing platforms like Uber and Lyft, drivers choose how much to drive, but the platform decides who they fetch on each particular ride. 

% Although both the open and discriminatory access platform designs optimize based on access control, they are very different approaches with opposing benefits. Open access platforms thrive on transparency, are easy to maintain and is naturally perceived to be fair. On the other hand, discriminatory access platforms block out some information or disallow some trades in order to further improve social welfare, potentially causing unfairness between firms, i.e., some firms may be totally not allowed to sell and some markets unprovided for. Generally, these platforms assume some form of search cost or search friction from their customers and restrict their choices in a sensible manner to improve overall welfare. For example, Amazon's \emph{Buybox} \citet{chen2016empirical} is usually held by a seller with competitive pricing, ready and available stock, punctual and free shipping, and excellent customer service, while superhosts in Airbnb are hosts which consistently receive good reviews, are responsive, active, and reliable. Lastly, controlled allocation platforms take this level of control to the extreme and directly allocate and control each trade to maximize some measure of performance, e.g., social welfare. For example, ride-sharing platforms take a cut from revenue in the system and may optimize based on it, but they may also do so based on social welfare to improve their long term market share among platforms. 

%\adam{tradeoff or trade-off} \rone{JP:American English I think its trade-off, while British English its tradeoff.} 
The recent emergence of online platforms has driven tremendous innovation in the design and operation of two-sided marketplaces. Platforms, unlike traditional retailers,  do not typically produce or store physical goods, but instead match producers to consumers and set prices algorithmically. For example, the majority of ride-sharing platforms (today) do not employ their drivers, but instead match available drivers to riders using mobile apps. %until recently when it was required by law in some US states, \rone{e.g., AB-5 in California as reported in \citet{sherman_2019}})}
Apart from ride-sharing, there are many other platforms that connect producers to consumers in innovative ways to improve both the provisioning of supply and the fulfillment of demand, which has led  to enormous efficiency gains and explosive platform growth across diverse marketplaces. \citet{evans2016rise} estimate the market value of platform companies to be over 4.3 trillion USD, representing a significant fraction of the  56.8 trillion USD aggregate  market value the largest $2000$ companies globally  \citep{forbesreport}.

\eb{There is a growing literature on the subject of platform design that seeks to understand how matching, access control, and pricing impact the efficiency of platform markets.}
%There are multiple factors to consider in designing a successful platform, including matching, access control, and pricing. An increasingly large literature on the design and analysis of platform and two-sided markets is driven by the desire to understand what makes them successful.
In a seminal paper on two-sided markets, \citet{rochet2003platform} compare market outcomes stemming from different governance structures, e.g., profit-maximizing versus not-for-profit organizations. Using a  similar two-sided market model, \citet{armstrong2006competition} compares platforms with  three different access control designs: monopolistic platforms, competing platforms where each user %\eb{(Eilyan says: Each what?)} 
can only choose one platform, and bottleneck platforms where \rone{only one side of the market (e.g., the consumer side)} can engage with multiple platforms.
% \sam{\textbf{Sam:} What is meant exactly by one side here?} 
More recently, \citet{akbarpour2017thickness} have shown under a model of dynamic matching that planners can improve overall utility with information on when agents depart as waiting patiently for a thicker market on both sides often allow for better matching, whenever it is feasible. 
% \eb{(Eilyan says: This reference needs clarification. What do you mean by `improve control'?  It's also not clear from the context what is meant by 'dynamic matching'. As opposed to static matching? It's also not clear what `agent's departure'  is meant to represent here.)} \rone{John: This was a paper on one of the kidney-matching sort of problems. One of the main results is that patiently allowing for the market to thicken can allow for a lower worst case loss as compared to greedily matching ASAP. I will continue to touch up the wordings in the main text.} 
The impact of algorithmic pricing on  real-world markets has also been  studied in recent years  \citep{chawla2007algorithmic, chawla2010multi,li2012automated}. Lately, \citet{dinerstein2018consumer} have focused on balancing trade-offs around search friction between conflicting designs, e.g., how much to guide consumers and reduce search friction while incentivizing price competition between sellers. 
% \eb{(Eilyan says: What do you mean by 'balancing trade-offs between conflicting designs'?)}

\emph{In this paper, we investigate the trade-off between  transparency and control that arises in the design of access and allocation control mechanisms in platforms.}
Present-day platforms exhibit a diverse array of access and allocation control designs.
For example, eBay adopts an \emph{open access} design that displays the offers from all producers to the customers. This design is intended for lowering producer entry cost and boosting competition, but may end up suffering from high consumer search cost. Uber, on the other hand, adopts a \emph{controlled allocation} design, in the sense that it only allows drivers to accept or decline the ride that is assigned from the platform. Lastly, Amazon employs a \emph{discriminatory access} design by directing its customers to its pre-selected ``Buybox" producers. While such an approach  serves to limit consumer search costs,  it may  lack transparency due to the ambiguity in the criterion for ``Buybox eligibility" (cf. \citet{chen2016empirical}).
% For example, within ride-sharing platforms, Didi requires a confirmation of pick-up and drop-off locations before allowing drivers to pick rides in an \emph{open access} design while Uber assigns or \emph{allocates} each ride to the nearest driver.
%

% \sam{For example, within ride-sharing platforms, Didi employs an \emph{open access} design for bidding during surge pricing, in the sense that it
% allows drivers to bid lower prices for riders through an \emph{open access} competition, as reported in \citet{muoio_2016}.  \eb{(Eilyan says: This description of `open access' could be interpreted as being inconsistent with our more formal definition of open access later in the paper. Can you clarify if Didi allows all drivers within a common geographic region to comepte (bid) against one another? If so, we should clarify this in the description.)}
% Uber, on the other hand, adopts a \emph{controlled allocation} design, in the sense that it only allows drivers to accept or decline the ride that is assigned from the platform.}
% \sam{In e-commerce, eBay adopts an \emph{open access} design that displays the offers from all producers to the customers.
% %
% This design is intended for lowering producer entry cost and boosting competition,} but may end up suffering from high consumer search cost. \eb
% %Uber, which minimizes search cost and friction in the platform, seeks to help decide \emph{allocations} between producer-consumer pairs and set clearing prices such that demand is served. 
% \sam{On the other hand, Amazon employs a \emph{discriminatory access} design by directing its customers to its pre-selected ``Buybox" producers. While such an approach  serves to limit consumer search costs,  it may  lack transparency due to the ambiguity in the criterion for ``Buybox eligibility" (cf. \citet{chen2016empirical}).}



% combines the scale of a populated marketplace with carefully differentiated access through their Buybox designs in a selective or \emph{discriminatory access} design. 

% \sam{\textbf{Sam:} Although the Didi and Uber examples are still here, I think we should remove them. Didi now operates as a controlled allocation platform that assigns riders to drivers. And I believe that their initial open access design has a lot to do with their growth strategy. Namely, they needed to attract a large number of taxi drivers in China in their incumbent stage. An open access design would make it much easier to attract taxi drivers. }

% \rone{JP: My thoughts are that we should either (i) include a short message around the necessity of open access then and the reason for transition to a controlled allocaiton, or (ii) to drop off the "ridesharing platforms with different designs" here as Sam suggests.  }

% \eb{(Eilyan says: I think that option (ii) makes the most sense. The current discussion surrounding ride-sharing feels like it meanders somewhat. And I'm not entirely convinced by Sam's explanation of open access as a key growth strategy in ride sharing, as this ignores the (more important?) role played by  ride subsidization in  driving growth. I suggest streamlining the discussion to very briefly describe the different platform types using well-known examples: (1) open access [ebay, airbnb], (2) discriminatory access [amazon buy box], and (3) controlled allocation platforms [ride-sharing or something else]. )}

% \rone{JP: Seems we are converging to option (ii). Eilyan's suggestion on streamlining the above two paragraphs is good. Adam? }
% \begin{itemize}
%     \item \sam{Do you mean that Didi does not entail any allocation of drivers to customers? This claim will require some references. }
%     \item \rone{JP: I read somewhere and heard from friends that drivers are allowed to bid on rides, somewhat in an open access fashion. Here's a potential article (\citet{muoio_2016}) describing this. I changed the description a little and added the article. }
%     \item \sam{It would be helpful if you could provide references on the way in which eBay and Amazon Buy box operates (e.g., articles on ``how to win the Buy box").}
%     \item \rone{JP: We provided references under related work:two-sided platform, e.g., \citet{chen2016empirical}. Do you think it will be good to list some of them here too? I have added a sentence adding this reference. }
% \end{itemize}


There are a variety of important open questions related to the design of access and allocation control mechanisms for platforms. First, what is the worst case efficiency loss of platforms under these designs? Second, what is the impact of allocation control on worst case efficiency loss
% \eb{(Eilyan says: impact on what?)}
, and are there any unintended incentives for strategic behavior that might decrease market efficiency? Lastly, is there a sweet spot between open access and controlled allocation mechanisms that balances transparency and control, while limiting efficiency loss? 

\subsection{Our Contributions}

In this paper, we model and analyze three different platform designs: (i) open access, (ii) controlled allocation and (iii) discriminatory access designs. \eb{Using a networked Cournot competition model as the basis for our analysis,  we provide worst case efficiency loss bounds for each design.}
%We study these designs using the model of networked Cournot competition. 
%\sam{This model considers a setting where firms compete to sell heterogeneous products to multiple markets.}
\eb{At the heart of the proposed model is a network (represented as a bipartite graph) that  specifies connections between firms and markets, where each firm competes \'{a} la Cournot in each of the markets that is has access to. In open access platform designs, all firms have access to all markets, resulting a complete bipartite graph. In discriminatory access designs, the platform determines the structure of network, i.e., the collection of markets that each firm is given access to.} \sam{In contrast, in controlled allocation platform designs, firms choose their individual supply levels, and the platform determines the allocation of the aggregate supply generated by the firms to the different
markets.} \eb{In this paper, we aim to shed light on the various trade-offs that emerge between efficiency loss, transparency, and control across these different platform designs.}
%Our analysis provides new results on the trade-offs between transparency and control in the design of platforms. 


%\sam{In open and discriminatory access designs, the firms and markets are connected by an undirected bipartite graph, and each firm is assumed to have access to those markets it is connected to in the bipartite graph.Specifically, open access designs correspond to the setting where the aforementioned bipartite graph is the complete bipartitte graph, and discriminatory access designs correspond to the setting where the aforementioned bipartite graph is specified by the platform.On the other hand, in controlled allocation platforms, the firms and markets are both connected to the platform that allocates the aggregate supply from the firms to all markets.}

% The open and discriminatory access designs correspond to the complete and optimal bipartite graph respectively, while the controlled allocation platform assumes a middleman performs allocations on behalf of the firms to markets to optimize certain objectives, such as social welfare. 
%Our analysis provides new results on efficiency loss and illustrates the trade-offs between transparency and control in the design of platforms.  %For the open and discriminatory access designs, we analyze the equilibrium of the networked Cournot game. On the other hand, we show that the controlled allocation design can be analyzed as a Stackelberg equilibrium instead. Under these network economic models, the consumers at each node are aggregated to a single inverse demand function. %We show that open access designs have bounded worst case efficiency losses while controlled allocation designs potentially and unintentionally create incentives for producers to curtail their productions, leading to unbounded worst case efficiency losses. Lastly, we show that a discriminatory access platform design maintains large production rates and leaves some room of control over allocations. 

%In the rest of this work, we introduce a networked Cournot competition model from \citet{bimpikis2014cournot} for networked competition between a group or producers and a group of consumers. We introduce the open access, controlled allocation and discriminatory access platform designs, and aim to determine the most robust platform design with respect to different market participants and environment. We introduce the considered market and producer model, and for each network, we define a corresponding networked Cournot or Stackelberg game and then define efficiency through social welfare and define our metric of performance, which is roughly speaking, a worst case guarantee on the minimal social welfare obtained as compared to the optimal social welfare.

The first platform design we consider is the open access design (Section \ref{sec:oap}), exemplified by online marketplaces like eBay and Etsy. The advantages of an open access platform design are its fairness, transparency, low producer entry cost, and the increased  market competitiveness driven by such attributes. %This design also increases competition among producers, which usually leads to large sales volume and lower prices for consumers. 
% We show that % under the networked Cournot competition model, 
% a large proportion of the optimal demand fulfilled in each market is preserved under open access designs, 
\sam{We prove that  open access  platform designs ensure  that at least half of the socially efficient demand level in each market is fulfilled at Nash equilibrium.}
%
% which plays a significant role in limiting efficiency loss at Nash equilibrium. 
 We also show that the social welfare levels achieved  under open access platform designs at equilibrium are no less than  $2/3$ of the efficient social welfare in the worst case. (Theorem \ref{thm:PoA_asym}). 
%Equivalently, we say that the \emph{price of anarchy (PoA)} for open access platforms under the networked Cournot competition model is $3/2$. 
\eb{In proving this result, we employ an intermediary argument---originally proposed by  \citet{johari2005efficiency} in the context single-market Cournot models---which shows that, among all convex producer cost functions,  \emph{linear} cost functions result in the greatest loss of efficiency at equilibrium. Building on this argument, we are also able to establish bounds that reflect the impact of asymmetry in  producer cost functions on  worst-case efficiency loss at equilibrium.}
%An integral piece of that result is a novel argument that \textit{the convex cost functions that maximize efficiency loss are linear cost functions}, a generalization of the results from \citet{johari2005efficiency} for single market Cournot competition. This fact also allows for us to obtain worst case efficiency loss bounds as a function of the degree of asymmetry in producers' cost functions. 
\sam{Together, these results show that open access platform designs promote sales volume across the different markets,} \eb{while limiting efficiency loss at equilibrium.}
% , has a small efficiency loss when firms have symmetric cost, 
%and retains a large proportion of the system's optimal social welfare.}


\eb{While open access platforms are shown to exhibit bounded efficiency loss, the welfare loss stemming from the ``misallocation'' of supply across the different markets can be substantial.
% With the purpose of alleviating the efficiency loss in open access platforms that results from the suboptimal allocation of supply to consumers. The allocation of supply to consumers is, in general, suboptimal in open access platforms.
As an alternative to open access platforms, we investigate a  controlled allocation platform design (Section \ref{sec:cap}), where the platform determines the allocation of supply across the different markets given quantity offers from the different producers.} 
%
%receives the supply quantity offers from producers and specifies the allocation of supply to the consumers.
%the possibility of alleviating such allocative efficiency loss through the adoption of a controlled allocation platform design.
%
% Given the efficiency loss in open access designs, one may intuitively posit that the efficiency loss in open access platforms is due to the poor allocation of supply to consumers. This is one of the many motivating factors towards considering a controlled allocation platform (Section \ref{sec:cap}). 
% These platforms control the allocation over each individual transaction, in order to carefully allocate supply from producers to consumers. Many modern platforms use designs of these forms. 
%\sam{Under the controlled allocation design, the platform receives the supply quantity offers from producers and specifies the allocation of supply to the consumers.}
For example, in ride-sharing platforms, drivers typically  decide when to drive, \eb{while the platform decides who they pick up.} 
\sam{As one of our main results, we show that the worst-case efficiency loss incurred by controlled allocation platforms grows at least linearly in the number of markets for a large family of supply allocation mechanisms (Theorem \ref{thm:generalcap}).} Perhaps surprisingly, this lower bound on the worst-case efficiency loss is shown to hold even in settings where the platform allocates supply across the different markets to maximize social welfare (Theorem \ref{thm:ineff}). The efficiency loss incurred by controlled allocation platform designs suggests that explicit allocation control may incentivize a reduction in production levels to such an extent that the efficient allocation of supply across the different markets cannot offset the efficiency loss associated with reduced production. 
%
%Such a result highlights that controlled allocation platforms may end up being inefficient in spite of its good intention.
% Given the prominence of these designs, one might expect that such platform designs are efficient. 
%Specifically, we show that \textit{the worst case efficiency loss \sam{at least grows} linearly in the number of markets even if the platform allocates supply to consumers in a way that maximizes social welfare} (Theorem \ref{thm:ineff}).  This highlights that controlled allocation platforms may end up being inefficient in spite of its good intention.
% Additionally, we show that the controlled allocation platform under the networked Cournot competition model results in a networked Stackelberg game, where neither the existence nor uniqueness of  Nash equilibrium can be guaranteed. 
%\sam{Additionally, such a result on the worst-case efficiency loss in controlled allocation platforms holds for a large family of market clearing mechanisms.} Specifically, we consider the setting in which the platform is allowed to choose its market clearing mechanism via the choice of its objective function used in market clearing. We show that any objective function that is a convex combination of consumer surplus and social welfare \sam{yields the same lower bound on the worst case efficiency loss (Theorem \ref{thm:generalcap}).}


% We conclude Section \ref{sec:cap} with \textit{a general result (Theorem \ref{thm:generalcap}) on the worst case efficiency loss under different choices of the market clearing mechanism.} Specifically, we consider the setting in which the platform is allowed to choose its market clearing mechanism via the choice of its objective function used in market clearing. We show that any objective function that is a convex combination of consumer surplus and social welfare has the same unbounded worst case efficiency loss result.
% while allocations that are more aligned to individual producers (such as revenue maximizing allocations) result in a smaller worst case efficiency loss. 

% \sam{\textbf{Sam:} I removed the statement ``while allocations that are more aligned to individual producers (such as revenue maximizing allocations) result in a smaller worst case efficiency loss". The reason for removing this is that this statement could be misleading, in the sense that Theorem \ref{thm:generalcap} only shows that the lower bound on worst case efficiency loss is low. This does not indicate that the worst case efficiency loss is small.}


\sam{As an alternative to controlled allocation platforms, we study a discriminatory access platform design where the platform indirectly controls the allocation of supply to consumers by restricting the set of markets that each seller has access to.}
% On the other hand, the result on incentivizing production in open access platforms motivates us to carefully restrict producer-consumer pairs in a way that strikes a balance between transparency and control to improve the allocation while maintaining large proportions of demand fulfilled. 
% Such a design is similar to the access control performed in Amazon's Buybox, which presents Amazon's preferred seller in the Buybox and other sellers lower in the page.
% which first presents a seller determined by Amazon based on various performance measures, and then presenting the selected list of alternative sellers lower on the page. 
% \rone{By limiting which potential sellers are exposed to the customer, the platform trades transparency for partial control.}
%
%
%
%
\eb{In this context, the set of markets that each firm has access to is determined by the platform in order to maximize  social welfare  at  the Nash equilibrium induced by the resulting  networked Cournot game.}
%
%We propose another platform design called discriminatory access in which the platform specifies the set of markets that each firm has access to in a way that maximizes the social welfare at the Nash equilibrium of the resulting networked Cournot competition. 
%
\eb{In Theorem \ref{thm:discriminatory_PoA}, we show that discriminatory access platforms improve upon the worst-case efficiency loss of open access and controlled allocation platforms, resulting in Nash equilibria whose  social welfare  is no less than 3/4 of the efficient social welfare in the worst case.}
% the improved allocations as a result of controlling the network allows for 
%\sam{the restriction on each firm's accessible markets leads to}
%\textit{an improved $3/4$ worst case guarantee on social welfare retention for discriminatory access platforms}. %Equivalently, we say that the worst case efficiency loss for discriminatory access platforms under the networked Cournot competition model is $4/3$. 
\sam{Given a simplifying assumption on the linearity of producers' cost functions, we  provide a greedy algorithm that is guaranteed to generate the optimal network (access control) structure, which  maximizes social welfare at Nash equilibrium (Theorem \ref{thm:greedy-alg}).}
\eb{Our analysis also sheds light on the role of producer cost asymmetry in determining  the optimal network structure. If producers have identical cost functions, then the optimal network structure is open access.  
If, however, there is significant asymmetry between producers' cost functions, then the optimal network structure may bar certain firms from participating in certain markets in order to preserve the ``competitiveness'' of those markets.}

%Similar to the open access platform results, we further explore the impact of cost asymmetry on the worst case efficiency loss. Specifically, when the production cost functions of firms are close to identical, it would be desirable to choose an open access design which maximizes the extent of competition between firms; on the other hand, if firms have substantially different cost functions, it would be desirable to choose a discriminatory access design, in which the platform picks out those firms with low production costs. 
%A careful design over the connections in the discriminatory access platform is also often not trivial, and w
% \sam{The resulting optimal network design problem is a mathematical program with equilibrium constraints (MPEC) that is, in general, difficult to solve both analytically and computationally. 
% However, under the simplifying assumption of linear cost functions,} we propose a greedy algorithm that is guaranteed to yield the network structure that maximizes the social welfare at the resulting Nash equilibrium (Theorem \ref{thm:greedy-alg}).

%In this work, we aim to answer the following questions to understand trends in platform design. 
%\begin{enumerate}
%	\item How well do platforms such as eBay that promise fairness, transparency and open access compare with a socially optimal solution? i.e., when there is one agent that makes production and allocation decisions for every agent? 
%	\item By allowing the platform control over allocation decisions, can we achieve further improvement in social welfare under controlled allocation platforms?  %(Note that allocation decisions are part of what the offline optimal setting require. Certainly if we allow for the platform to both decide allocations and productions, the system would be under benevolent dictatorship and absolutely efficient.)
%	\item How much can we gain in efficiency by sacrificing transparency and fairness in the system by careful design over allowed matches through discriminatory access platforms? 
%	\item How do search costs help shed light on a more realistic solution from the above questions? If we also consider search costs in our model, how much of a shift towards open/discriminatory access will we find depending on user search costs? %How can platforms learn if there are participants in their markets with contrasting search costs and how can they enable increased profits in light of knowledge of customers with different search costs? 
%\end{enumerate}

% \subsection{Our Contributions}
% Motivated by various successful online platforms, we first propose three different platform designs under the networked Cournot competition model, and look at efficiency losses due to selfish behavior under each design. In the literature, the objective we consider is usually known as \textit{Price of Anarchy (PoA)}, and we will formally define it in the following section. An informal definition of PoA is the worst-case (multiplicative factor) loss in social welfare due to behavior from selfish agents. For example, having a constant PoA bound implies that regardless of the parameters describing the particular market, said platform retains at least a constant fraction of the optimal social welfare. %On the other hand, having a bound that is non-constant implies that there are settings or parameters where performance of the platform can grow in inefficiency and be potentially unbounded in inefficiency. 
% Our main results are summarized here in the following points. 
% \begin{enumerate}
% 	\item Platform Market Models under Networked Cournot competition: Under the networked Cournot competition model introduced by \citet{bimpikis2014cournot} we introduce three different platforms, (i) an open access platform, e.g., eBay, (ii) a controlled allocation platform, e.g., Uber, and (iii) a discriminatory access platform, e.g., Amazon Buybox, designed to function in a similar fashion to some of today's popular online platforms. Under each platform design, we further show conditions under which a (possibly unique) equilibrium exists.  %We also state settings and conditions under which a (possibly unique) Nash equilibrium exists for each of the following platforms below. 
% 	\item Open Access Platforms: We show that platforms that offer open access %(corresponding to a full bipartite graph dictating firm-market pairings)
% 	preserve \textbf{at least $2/3$ (a provable tight bound) of the optimal social welfare obtainable in the worst case}. This general bound can be further tightened under certain settings, e.g., firms having symmetric cost or based on the number of firms with asymmetric costs. We also provide bounds based on the level of asymmetry in the cost functions of the firms. These results rely on an important argument that \textbf{the  ``worst-case" convex cost functions for efficiency loss are linear.}   
% 	\item Controlled Allocation Platforms: In the controlled allocation platform, we show an example whereby \textbf{efficiency loss grows linearly in the number of markets} even when platforms optimize for social welfare. The example helps shed light on why such platforms may end up being inefficient in spite of its good intentions. In particular, we find that firms' allocation decisions are not fully aligned with allocation with a social welfare maximizing platform, and that \textbf{firms may produce less in anticipation} to what seems as poor allocation decisions. Moreover, the controlled allocation platform may have multiple equilibria, or even none, which increases the complexity of computing worst case bounds of efficiency loss. We also consider a variety of other objectives, and present price of anarchy bounds for each objective.
% 	\item Discriminatory Access Platforms: Intuitively, optimizing over the set of bipartite graphs can only improve the PoA, and we explicitly show the possible improvement of discriminatory access over open access via \textbf{an improved PoA bound of $4/3$, as opposed to $3/2$ previously for open access platforms}. Similar to results from the open access platforms, we also provide tighter price of anarchy results under a number of different settings, such as when firms have symmetric costs. A \textbf{greedy algorithm for access control design} under the ``worst-case" setting where costs are linear is also designed, and help give some intuition on why the problem in the general cost setting is hard to solve. 
% 	\item Modeling Search Costs: To further motivate the shift in today's platform designs towards discriminatory access, we further include a search cost model where the platform is informed of the market's search cost or search friction. We show that considering search costs, the price of anarchy of open access platforms can be unboundedly large too, while discriminatory access platforms can always retain its bounded price of anarchy in spite of search costs. %We illustrate an example on how a platform can differentiate between low and high search cost participants and the benefits of this differentiation. %We show that when a market segment is equally split into a high and low search cost segment, the optimal set of actions differ between them and further, also between the case whereby the platform considers the two segments as one.% We show through an example that wrongly combining two market segments with different search costs can lead to loss of efficiency with a multiplicative factor of $\frac{13}{40}$.
% \end{enumerate}

%As a summary, the paper as a whole, under a simple and stylized model, sheds light on the dynamics of multi-sided platform markets, and the effect of platform design through access and allocation control on fairness, access, transparency, search costs, and most importantly, efficiency.    

\subsection{Related Literature}
% The proliferation of platforms and networked competition has led to a large and growing literature that covers many aspects of platform design, i.e., how to design successful platforms and why some platforms are more successful than others. 
% Additionally, with more platforms collecting data, much of the recent work uses data to learn particular features in the successful design of platforms. 

%\sam{The proliferation of platforms has led to a large and growing literature on the common features of successful online platforms.
% In this paper, we focus on the access and allocation control in online platforms, and examine its effect on the worst efficiency loss in online platforms.
\eb{In this paper, we examine the role  of access and allocation control on the worst-case efficiency loss in online platforms where producers compete \`{a} la Cournot.}
% Specifically, we study the worst case efficiency loss in online platforms associated with different access and allocation control methods using a networked Cournot model.
% In this paper, we present a study of the worst case efficiency loss of different designs with regards to access and allocation control for platforms using a networked Cournot model. 
% \sam{\sout{Our work is related to and builds upon two major streams of literature: two-sided platform markets and networked competition.}}
\sam{Our work contributes to two major streams of literature relate to (i) the design and operation of two-sided platforms, and (ii) the  analysis of competition in networked markets.}


% \eb{(Eilyan says: John, Sam: The lit. review, as it's currently organized, lacks a clear thread connecting the different bodies of literature being discussed. It's also not immediately clear how to interpret the  distinction between ``two-sided platform markets'' and ``networked competition'', given that a number of  papers discussed under the heading of ``platform markets'' are also concerned with networked markets. The first half of the lit. review might read more clearly if the  thread discussing the different facets/approaches to platform design and operation  (e.g., open access, controlled allocation, and discriminatory access) was emphasized more strongly. Thoughts?)}

% \rone{JP: That sounds like a great suggestion IMO - It will certainly read more clearly. I think the first part should touch on a quick overview into two-sided or multi-sided platforms and then shift gears onto well-defined headings on the different facts of platform design/operation. }

% \sam{Sam + John: TODO - Update skeleton for literature review and add more recent and related references, if possible. }


\subsection*{Platform Design and Operation}
% \sam{There is a large stream of literature that studies how different facets of platform design and different methods of operation affects the efficiency of online platforms. 
% The study on 
% }

% \sam{The focus of this paper is }

% \subsubsection*{Two-sided Platform Markets.}
The recent growth of online platforms has led researchers to focus on identifying design features common to successful platforms. Earlier works in this area started by introducing different models of two-sided platform markets. \rone{The renowned work of \citet{rochet2003platform} considered a model of platform competition in two-sided markets with network externalities, e.g., markets where the buyer surplus depends on the number of sellers.}
\sam{In that work, the authors leverage the platform competition model to quantify how the consumer and producer surplus is affected by the market clearing mechanism in the platform.}
% In that work, they studied how price allocations between the buyer and seller sides of the market depend on the platform type or design, but also other properties, such as how platforms differentiate themselves, and whether buyers are penalized for multi-homing. 
% \sam{\textbf{Sam:} what is meant exactly by ``pricing structure" here?}  
%They posit that the main determinants are (i) transaction costs existing between different sides, and (ii) constraints on types of transaction costs imposed by the platform. 
\sam{In \citet{evans2005industrial}, the authors provide additional applications of Rochet and Torile's model on the antitrust regulation of two-sided markets.}
% Based on the model in \citet{rochet2003platform}, \citet{evans2005industrial} provided additional application areas and empirical evidence around the structure of two-sided platforms in industry.
% \sam{\textbf{TODO:} revise the discussions on \citet{rochet2003platform} and \citet{evans2005industrial}.}
Using a different model, \citet{armstrong2006competition} considers the presence of important cross-group or indirect network effects between the customer groups participating on the platform. Other definitions and models are found in many other work, such as \citet{hagiu2015multi}, which compared the choice for a firm between operating within a multi-sided platform setting and operating independently via vertical integration. 
% Based on the focus of their work, models of two-sided or multi-sided platforms in the literature can differ slightly. 
A good summary of these earlier works can be found in \citet{rysman2009economics}. 
% \sam{\textbf{Sam:} can you provide a more detailed description of what is done in this paper?}
Our focus is on access and allocation control designs for these platforms.  

\subsubsection*{Open Access Platforms.}
Open access is touted in \citet{boudreau2010open} as a way to increase competition among participants \rone{in mobile device platforms}. In \citet{parker2017innovation}, the open access design of \sam{online platforms for developers} is shown to promote fairness and \sam{innovation}.
% openness, where they describe a platform as more ``open'' if it places less restrictions on participation. 
% \sam{\textbf{Sam:} what is meant by openness here?}
The classical example studied for open access \rone{for retail markets} is the online marketplace eBay.
% which had once the largest market capitalization among platforms, as found by \citet{chircu2001digital}. 
\sam{The study of eBay in \citet{gross2003balances,hui2016reputation} reveals that the success of open access platforms will, in general, depend heavily on the reputation of sellers and the platform regulation policies (e.g., seller ratings and buyer protections).}

% Lastly, \citet{heylighen2006open} shows that open access thrives on information symmetry, openness and transparency. 

% \sam{\textbf{Sam:} I removed the paper by \citet{heylighen2006open}. This paper is about open access development (e.g., open source communities) and seems to be unrelated to this paper.}

% By contrast, an intuitive way to exert control in the platform is to assume that producers make socially inefficient decisions and instead decide allocations on their behalf, e.g., Uber as studied in \citet{hall2015effects}. 
\subsubsection*{Controlled Allocation Platforms.} 
In contrast to the open access approach, some platforms (e.g., Uber) may choose to directly determine the allocation of supply to the consumers. 
% A concrete example of such platforms is Uber, as is studied in \citet{hall2015effects}.
% \citet{rosenblat2016algorithmic} showed that how well these producers understand allocation decisions affect their satisfaction on the app. For example, although hiding the destination can potentially prevent destination-based discrimination, one of their interviewees believed that they should have the right to know the destination and the right to refuse without penalization. It is also common to see drivers on ride-sharing platforms rejecting rides that are requested far from them. 
% \citet{malin2017free} showed that platforms like Uber prioritize riders from the drivers' perspective.  %\sam{\textbf{Sam:} can you elaborate on what the outcomes are exactly?}
\sam{These platforms, however, might be susceptible to the manipulation from the suppliers.}
For example, it is also well known and reported in \citet{chen2017thrown} that drivers on ride-sharing platforms collaborate and reduce their supply to cause price surge and demand spikes in the system. 
% \sam{Several papers have investigated pricing and allocation policies that the platform might adopt to limit the price manipulation from the suppliers.}
% 
\sam{Several papers have investigated pricing and allocation policies that might limit the price manipulation from suppliers. Examples of such work include the study on a spatio-temporal pricing mechanism in \citet{ma2018spatio} and the study on admission control policies in \citet{afeche2018ride}.
Apart from the potential market manipulation from suppliers, 
other major challenges in managing controlled allocation platforms include the difficulty in solving the supply allocation problem, and the potential insufficiency of supply that results from the competition with rival platforms. We refer the readers to \citet{alijani2017two, DBLP:journals/corr/Banerjee0L16, scheiber2017uber,lu2018surge,fang2018loyalty,banerjee2015pricing} for recent advances.
}

% Under various settings, \citet{alijani2017two} and \citet{DBLP:journals/corr/Banerjee0L16} designed approximation algorithms to find the optimal allocation. Recently, \citet{ma2018spatio} also considered spatio-temporal pricing, while \citet{afeche2018ride} provide new insights on the interplay between admission control and drivers' strategic repositioning decisions. 

% Such a strategic behavior often improves individual payoff but jeopardizes the performance of the platform. \citet{scheiber2017uber,lu2018surge,fang2018loyalty,banerjee2015pricing} look at methods that the platform could leverage on to ensure that drivers actively participate in only one platform. 

\subsubsection*{Discriminatory Access Platforms.}

Another possible way to improve upon open access platforms is through discriminatory access. This is studied in \citet{banerjee2017segmenting,kanoria2017facilitating,akbarpour2017thickness}, where the platform restricts the set of markets that producers are allowed to bid in to improve social welfare. 
%\sam{\textbf{Sam:} what is the connection between algorithmic pricing and discriminatory access?}
A typical example of discriminatory access platforms is Amazon's Buybox studied in \citet{chen2016empirical}, where Amazon highlights one seller for each item. Another example of discriminatory access is Airbnb's Superhost program, which highlights certain hosts through badges. \sam{In \citet{liang2017superhost}, it was shown that the Superhost program vastly increases Airbnb's revenue.}
% A significant amount of effort has been placed into what is known in the literature, e.g., \citet{chawla2007algorithmic,chawla2010multi,chen2017observing}, as \emph{algorithmic pricing}, a tool that aims to improve the chances to be a highlighted producer for a single product, a form of discriminatory access. 
\sam{The majority of prior work on discriminatory access platforms, e.g., \citet{chawla2007algorithmic,chawla2010multi,chen2017observing}, has focused on the effect of algorithmic pricing on the efficiency of the platform. In this paper, we instead examine the reduction in worst-csae efficiency loss (relative to open access designs) that can be attained through discriminatory access.}


%One of the starting objectives of online marketplaces or platforms as stated in \citet{bakos1997reducing} was to reduce search costs --- that is, to reduce the amount of effort to acquire information on sellers and the quality of their goods. \citet{diehl2003smart} showed that lower search costs leads to an increase in price sensitivity. However, it has also been shown in \citet{branco2015too} that too much information revealed in online platforms can instead result in increasing search costs from the consumers' point of view. \citet{nishida2018lowering} showed that reducing search costs can lead to higher prices and profit while \citet{gamp2016guided} showed that a monopolist may impede information acquisition to improve her profits. In a more recent work, \citet{dinerstein2018consumer} studies the tradeoff between guiding consumers to their most desired product while also strengthening seller incentives to offer low prices.

\subsubsection*{Alternative Design Factors.} Besides access and allocation control, work in this area has also covered a variety of possible design factors, including pricing \citep{weyl2010price}, competition  \citep{armstrong2006competition}, reputation \citep{nosko2015limits,tadelis2016reputation,luca2017designing}, and thickness or volume \citep{ashlagi2018matching}. % also dynamic models for kidney exchange in \citet{agarwal2018market}. 
%\sam{\textbf{Sam:} on a quick inspection it seems that market thickness refers to the number of buyers offering the same product. Am I correct in saying this? Also, what is meant by ``dynamic models for kidney exchange"?}
Recent empirical studies in \citet{einav2015assessing} and \citet{bimpikis2016spatial} also reveal significant price dispersion in online e-commerce and ridesharing marketplaces, 
%\sam{\textbf{Sam:} what is meant by spatial marketplace here?} 
causing platforms to differentiate products in order to create distinct consumer markets as in \citet{dinerstein2018consumer}. In particular, these results highlight the need to study platforms in using models of \emph{networked competition}.

\subsection*{Networked Competition}
Models of networked competition aim to capture the effects of network constraints on strategic interactions between firms. They are prevalent in industries which have distinct geographical markets with significant price differentiation. 
%
\sam{Depending on the model's assumption on the decision variables of the producers, these models can be classified into the networked Bertrand model \citep{chawla2008bertrand, guzman2011price, anshelevich2015price}, the networked Cournot model \citep{ilkilic2009cournot, bimpikis2014cournot, abolhassani2014network,  xu2017efficiency,le2018efficiency}, the networked supply function model 
\citep{berry1999understanding, hobbs2000strategic, liu2007impacts, wilson2008supply, holmberg2014supply, lin2019structural}, and other networked bargaining games where agents can trade via bilateral contracts over a network that determines the set of feasible trades (cf.  \citet{AbreuManea2012, Elliott2015, Nava2015, nguyen2015coalitional}).}
% These models include 
% networked Bertrand models studied in \citet{guzman2011price, anshelevich2015price, chawla2008bertrand}, networked Cournot models in \citet{bimpikis2014cournot, abolhassani2014network, ilkilic2009cournot}, networked Stackelberg competition in \citet{xu2017efficiency,le2018efficiency}, and other networked bargaining games where agents can trade via bilateral contracts over a network that determines the set of feasible trades, e.g., \citet{Elliott2015, Nava2015, AbreuManea2012, nguyen2015coalitional}. 
These networked competition models have applications in many areas, e.g., electricity markets in \citet{bose2014role} and demand-side management in smart grids in \citet{motalleb2017game}.


% \sam{In this paper, we rely on a networked Cournot competition model to describe the strategic interactions between producers in online platforms. The advantage of using the networked Cournot model primarily lies in its good balance between the tractability of analysis and the theoretical insights that the model reveals. }


Our work relies on a  model of networked Cournot competition. 
\sam{Compared with other models of networked competition, the advantage of the networked Cournot model is its  balance between explanatory power and tractability of analysis. Specifically, Cournot models are able to capture the potential exercise of market power from producers via the withholding of production. The Bertrand model, in contrast, assumes that each producer is willing to produce any amount of good at its offered price, and might overestimate the intensity of competition between producers (cf. \citet{yao2008modeling}). On the other hand, although one might obtain additional flexibility in describing the price-quantity pair that each firm offers via the use of supply function models, the equilibrium analysis of such models are, in general, intractable if a firm has access to multiple markets with heterogeneous demand functions (cf. \citet{wilson2008supply}).  }

The vast majority of the literature on networked Cournot competition, e.g., \citet{bimpikis2014cournot, abolhassani2014network, ilkilic2009cournot}, focuses on characterizing and computing Nash equilibria in the absence of capacity constraints. Recent work from \citet{alsabahcapacity} focuses on a scenario with capacity constraints. This paper is most closely related to \citet{johari2005efficiency}, which provide bounds on the worst case efficiency loss of Cournot games. \citet{cai2017role} shows how the mechanism of market clearing (which is determined via the choice of the system operator's objective function) might affect the efficiency of the platform under network constraints. Our work focuses on platform design through access and allocation control under the networked competition model. We extend some key results from \citet{johari2005efficiency} on worst case efficiency loss while presenting new results on how a platform might reduce the worst-case efficiency loss at Nash equilibrium via appropriate access control. 

% \adam{The following seems out of place to me here...maybe we can do it in the related work section instead?}
% \subsection{Comparison of Competition Models.}




%  \textcolor{blue}{The networked competition models mentioned above each have their own strengths and drawbacks. Cournot competition studies quantity competition and has been used to describe competition in a variety of industries where products are difficult to transport, either due to sheer weight in the case of cement markets or due to the effect the transportation network in the case of power markets. While Cournot models typically do not include some important features, such as capacity constraints or dynamics, the analysis of these models has had significant practical impact. Further, models with capacity constraints, such as that of \citet{kreps1983quantity}, or those that considered dynamics, such as \citet{daughety1985reconsidering}, have often resulted in Cournot-like results. }
 
% Before moving forward, we first provide context for how the networked Cournot competition model can differ from Bertrand and Supply Function models, which are other common models of networked competition.}

% \rone{In contrast, Bertrand models capture price competition in networks rather than quantity competition, e.g., \citet{chawla2008bertrand}.  They have typically been used to model applications such as competition between internet service providers.  However, they tend to overestimate the intensity of competition between firms; thereby under-predicting price markups due to the exercise of market power. For example, when firms have identical production costs, the unique Bertrand equilibrium when there are at least two firms corresponds to the competitive equilibrium. On the other hand, Cournot models have proven useful in studying the potential exercise of market power from producers that withhold supply. 
% %Additionally, although producers do not directly specify their production quantities in e-Commerce, Cournot models are still potentially useful in helping predict the production capacity that each firm builds out in the long run. Specifically, as is pointed out in the classical paper by \citet{kreps1983quantity}, the price and production levels at the unique Cournot equilibrium are identical to the price and production levels at the unique subgame perfect equilibrium of a two-stage game, in which firms first choose their capacities in stage 1 (\'{a} la Cournot), followed by a choice of prices (\'{a} la Bertrand) in stage 2, where production levels are set according to the capacity levels chosen in stage 1.
% }

% \rone{Finally, studying supply function models, first introduced by \citet{klemperer1989supply}, in the networked setting gives additional flexibility for describing the price-quantity pair that each firm offers.  This is particularly of interest in the case of electricity markets, where firms often bid using supply functions.  However, the equilibrium analysis of such models are, in general, intractable if a firm has access to multiple markets with heterogeneous demand functions. In many cases the equilibrium of supply function models aligns with that of Cournot models, though this is not always the case, as shown in \citet{willems2009cournot}. }


==> 2020_ OR_ Net Cournot and Platforms/macros.tex <==
% Colors:
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
\def\black{\textcolor{black}}
\def\yellow{\textcolor{yellow}}
\def\green{\textcolor{green}}
\def\tcbg{\textcolor{bgrd}}
\def\magenta{\textcolor{magenta}}
\def\white{\textcolor{white}}
\def\gray{\textcolor{gray}}

==> 2020_ OR_ Net Cournot and Platforms/notation.tex <==
%% General machinery
\newcommand{\AutoAdjust}[3]{\mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}% {\left[{#1}\right]}
\newcommand{\Ex}[2][]{\operatorname{\mathbf E}_{#1}\InBrackets{#2}}
\newcommand{\Prx}[2][]{\operatorname{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\def\prob{\Prx}
\def\expect{\Ex}
\newcommand{\probq}[2]{x_{#1}\AutoAdjust{(}{#2}{)}}
\newcommand{\cumprobq}[2]{X_{#1}\AutoAdjust{(}{#2}{)}}
\newcommand{\super}[1]{^{(#1)}}
\newcommand{\dd}{\mathrm{d}}  % for integrals
\newcommand{\given}{\;\mid\;}
\newcommand{\eps}{\epsilon}

\newcommand{\noaccents}[1]{#1}

\newcommand{\newagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

\newcommand{\profit}{\pi}
\newcommand{\price}{p}
\newcommand{\demlim}{\alpha}
\newcommand{\demrate}{\beta}
\newcommand{\supply}{s}
\newcommand{\demand}{d}
\newcommand{\production}{q}
\newcommand{\cost}{C}
\newcommand{\realloc}{z}
\newcommand{\thrmarket}{j^{\mathrm{thr}}}
\DeclareMathOperator{\SW}{SW}
\DeclareMathOperator{\REV}{REV}
\DeclareMathOperator{\CS}{CS}
\newcommand{\util}{U}
\DeclareMathOperator{\SWCL}{SWCL}
\DeclareMathOperator{\SWOA}{SWOA}


% CALLIGRAPHIC AND BOLD SYMBOLS
\newcommand{\Bset}{\mathbb{B}}
\newcommand{\Cset}{\mathbb{C}}
\newcommand{\Fset}{\mathbb{F}}
\newcommand{\Mset}{\mathbb{M}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\Qset}{\mathbb{Q}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Sset}{\mathbb{S}}
\newcommand{\Tset}{\mathbb{T}}
\newcommand{\Uset}{\mathbb{U}}
\newcommand{\Vset}{\mathbb{V}}
\newcommand{\Wset}{\mathbb{W}}
\newcommand{\Zset}{\mathbb{Z}}

\newcommand{\Ical}{{\cal I}}
\newcommand{\Acal}{{\cal A}}
\newcommand{\Bcal}{{\cal B}}
\newcommand{\Ccal}{{\cal C}}
\newcommand{\Dcal}{{\cal D}}
\newcommand{\Ecal}{{\cal E}}
\newcommand{\Fcal}{{\cal F}}
\newcommand{\Gcal}{{\cal G}}
\newcommand{\Hcal}{{\cal H}}
\newcommand{\Kcal}{{\cal K}}
\newcommand{\Lcal}{{\cal L}}
\newcommand{\Mcal}{{\cal M}}
\newcommand{\Ncal}{{\cal N}}
\newcommand{\Ocal}{{\cal O}}
\newcommand{\Pcal}{{\cal P}}
\newcommand{\Qcal}{{\cal Q}}
\newcommand{\Rcal}{{\cal R}}
\newcommand{\Scal}{{\cal S}}
\newcommand{\Tcal}{{\cal T}}
\newcommand{\Wcal}{{\cal W}}
\newcommand{\Ucal}{{\cal U}}
\newcommand{\Vcal}{{\cal V}}
\newcommand{\Xcal}{{\cal X}}
\newcommand{\Zcal}{{\cal Z}}

\makeatletter
\newcommand{\hufu}[1]{\textcolor{red}{[Hu\@ifnotempty{#1}{: #1}]}}
\makeatother

==> 2020_ OR_ Net Cournot and Platforms/openaccess.tex <==
%openaccess


Open access platforms, such as eBay and Etsy, provide all customers access to all active sellers.
% thrive on transparency and offer buyers/consumers access to all possible sellers. 
Such platforms are typically accompanied by lower barriers to entry, which has the potential to increase market competitiveness and efficiency.
% This platform design is usually accompanied by lower entry costs that enables increased competition between producers, and thereby boost transaction volume, and oftentimes lead to socially efficient markets by fairly presenting similar opportunities to every participant. 
%
In this section, we  provide tight bounds on the worst case efficiency loss in  open access platforms under a variety of assumptions on supply and demand-side characteristics.


% The main theorem in this section provides a (tight) efficiency loss bound of a networked Cournot game governed by an open access platform with respect to the number of firms $n$.

\begin{theorem} \label{thm:PoA_asym}
	%Let Assumption \ref{ass:cost} hold. 
	The worst case efficiency loss associated with a cost function profile $C$ and the corresponding open access networked Cournot game $(F, \mathcal{Q}(F \times M), \pi)$ is upper bounded by
	\begin{align*}
	\rho (F \times M,C) \leq \frac{3}{2} \left( 1 - \frac{1}{3n+6} \right).
	\end{align*}
 	The bound is tight if all markets are identical in terms of their maximal willingness to pay. That is, if  $\alpha_1 = \alpha_2 =  \cdots = \alpha_m$, then there exists a cost function profile $\overline{C}$ such that
\begin{align*}
	\rho (F \times M,\overline{C}) =  \frac{3}{2} \left( 1 - \frac{1}{3n+6} \right).
\end{align*}
\end{theorem}



\noindent \eb{Letting the number of firms $n \rightarrow \infty$, we have the following result as an immediate corollary to Theorem \ref{thm:PoA_asym}. }

\begin{corollary}
	\label{cor:poabound} The price of anarchy of open access platforms is at most 3/2.
\end{corollary}
\eb{The price of anarchy bound in \autoref{cor:poabound} is valid for open access platform with any number of firms and markets. It, therefore, recovers the 3/2 price of anarchy bound first established by \citet{johari2005efficiency} in the context of single-market Cournot games as a special case.}

\eb{In addition to having bounded efficiency loss,  open access platforms are also guaranteed to limit the extent to which firms withhold their production (relative to socially optimal levels) at  Nash equilibrium.} \sam{We formally state this property in Proposition \ref{lem:prodpres}.}

\begin{proposition}
    \label{lem:prodpres}
    \rone{
	  At each Nash \eb{equilibrium}, the demand fulfilled in each  market $j\in M$ is at least half of the demand fulfilled at the socially efficient production profile.} % \rone{Alternative: Producers, on aggregate under the open access platform, withhold at most half of the demand fulfilled in each market $j\in M$. }
\end{proposition}  


\sam{In other words, the amount of production that is withheld in each market at Nash equilibrium is no greater than half of the socially efficient production quantity.  This ensures that aggregate consumer utility at Nash equilibrium is at least $3/4$ of the aggregate consumer utility at the efficient production profile---a result that is critical to the low efficiency loss of open access platforms. }


\subsection{Excess Entry in Open Access Platforms }
\eb{Theorem \ref{thm:PoA_asym} reveals that increased competition in the supply-side of the platform does not necessarily translate to increased market efficiency.
We shed  light on what drives this seemingly counterintuitive behavior, where the entry of a ``new'' firm to the platform can result in a reduction of social welfare at Nash equilibrium. 
While the entry of a new firm is guaranteed to increase the aggregate quantity supplied to each market at equilibrium, the entry of an additional firm will also result in a reduction in the  quantities produced by each of the existing firms at equilibrium. Thus, if the new entrant's marginal cost to produce is large relative to existing firms, then its entry will result in an increase in the aggregate production cost at equilibrium. And, under certain conditions on the firms' cost structure, this increase in the aggregate production cost will exceed the corresponding increase in aggregate consumer utility driven by the new entrant---resulting in an overall reduction in social welfare at equilibrium.} \sam{This behavior is closely related to the  ``excess entry theorem'' in the economics literature  \citep{suzumura1987entry, mankiw1986free, lahiri1988helping}.
}


We investigate this behavior more deeply in Sections \ref{sec:worst_case_cost}-\ref{sec:efflossOAP}, where we provide a refinement of the price of anarchy bound in Theorem \ref{thm:PoA_asym} that sheds light on the role played by asymmetry in the cost structure across firms. As part of these analyses, we  also establish a technical lemma in Section \ref{sec:worst_case_cost}, which characterizes the functional form of the cost function profile that maximizes the efficiency loss in networked Cournot games.



% \sam{
% This seemingly counterintuitive result indeed occurs if the increase in competition is a consequence of the entry of an expensive producer.
% Specifically, the entry of a new producer is guaranteed to lead to an increase in aggregate supply in each market at Nash equilibrium, which subsequently leads to an increase in consumer utility.
% However, it is also guaranteed to result in a reduction in the production quantity of each of the existing producers.
% As a result, there exists a range of linear cost functions of the new producer, under which the entry of the new producer will lead to an increase in production cost that is greater than the increase in consumer utility---thereby resulting in a reduction in social welfare.
% %
% % First, note that  the entry of this new firm  results in an increase in aggregate supply at Nash equilibrium, because of increased `competition' in the market.
% % However, its entry takes away production from its (cheap) competitors. 
% % This manifests in a reduction in social welfare if the increase in production cost exceeds the increase in consumer utility. 
% %Such a counterintuitive behavior of Nash equilibrium was first analyzed in \citet{lahiri1988helping}, which shows that the removal of expensive firms might lead to an increase in social welfare in Cournot competitions with asymmetric cost. 
% Such a phenomenon is known as the ``excess entry theorem'' in the economics literature, e.g., \citet{suzumura1987entry, mankiw1986free, lahiri1988helping}, and reveals the possibility that a new firm's entry can lead to a reduction in social welfare.
% }




% \sam{For the remainder of this section, we examine the  provide a deeper investigation into the potential increase in efficiency loss that occurs after the introduction of a new producer.
% As is discussed after Theorem \ref{thm:PoA_asym}, such an increase in efficiency loss will occur if the entry of the new producer leads to an increase in production cost that is higher than the increase in consumer utility---a phenomenon that is closely related to the asymmetry in production cost.
% % Finally, recall that Theorem \ref{thm:PoA_asym} shows that the increase in competition---as is reflected by the increase in the number of producers---might result in a reduction in social welfare. 
% % As is discussed earlier, such a reduction in social welfare will occur only if the difference between the entrant's production cost and the cost of the cheapest producer is large enough. In other words, the potential increase in efficiency loss is closely related to the asymmetry in producers' cost functions. 
% In what follows, we provide a refinement to Theorem \ref{thm:PoA_asym}, which establishes a price of anarchy bound for open access platforms that reflects the role played by asymmetry in the cost structure across firms.
% %
% To do this, we first establish a technical lemma in Section \ref{sec:worst_case_cost}, which characterizes the functional form of the cost function profile that maximizes the efficiency loss in networked Cournot games.}

% \rone{In other words, open access platforms encourage production (at least half), with allocations to the markets somewhat aligned. The efficient allocation would require the right amount of production, and an efficient allocation to the various markets. In the following sections, we will explore in Section \ref{sec:dap} a platform that limits the access between firms and markets, and a platform that controls allocations in Section \ref{sec:cap}, which are two different mechanisms to potentially improve allocations. }

% In the remainder of this section, we prove Theorem \ref{thm:PoA_asym} first by proving a critical result in Lemma \ref{Lem:WorstCaseLinear} that the cost functions maximizing the worst case efficiency loss are linear ones, a result presented in \citet{johari2005efficiency} for the case without a network. That means that given any set of convex cost functions, we can find a corresponding set of linear cost functions that increase the worst case efficiency loss. Applying Lemma \ref{Lem:WorstCaseLinear}, bounds on efficiency loss are developed for both the symmetric and asymmetric costs setting in Proposition \ref{prop:PoA_symm} (Section \ref{subsec:symm}) and Theorem \ref{thm:PoA_asym} (Section \ref{subsec:asymm}) respectively. 

% The result in Theorem \ref{thm:PoA_asym} (for firms with asymmetric costs) is potentially counter-intuitive since an increase in the number of firms $n$ (presumably increasing competition) results instead in a larger worst case efficiency loss. To shed more light on this, we further develop worst case efficiency loss bounds on networked Cournot games under open access platforms with linear cost functions and bounds on asymmetry, presented later in Proposition \ref{prop:linearcostspoa}. Additionally, in the symmetric cost case, in Proposition \ref{prop:PoA_symm} we see that it is indeed that as the number of perfectly competing firms increase, the worst case efficiency loss decreases.  



% \sout{We present a generalized result from \citet{pang2017efficiency} in the following lemma that demand fulfilled at the Nash equilibrium of the networked Cournot game for any market is at least half of the fulfilled demand under a socially efficient allocation. }

%This result shows that the production rates and demand fulfillment rates at the equilibrium under an open access platform are preserved, suggesting that efficiency loss is driven by misaligned allocations by anarchistic firms, motivating the controlled allocation platforms studied in the next section, where the platform control allocations to optimize social welfare (and possibly other objectives). 

%Here we present an extension of Lemma 5 from \citet{pang2017efficiency}. Following notation, we have sets $S_N$ and $S_*$ denoting the sets of active markets under the equilibrium and optimal setting respectively. 

% \begin{proposition}
%     \label{lem:prodpres}
% 	  At Nash \eb{equilibrium}, the demand fulfilled in each  market $j\in M$ is at least half of the demand fulfilled at the socially efficient outcome. \rone{Alternative: Producers, on aggregate under the open access platform, withhold at most half of the demand fulfilled in each market $j\in M$. }
% \end{proposition}  
%\proof{Proof:} Proof included in the Appendix. \endproof



% \sout{This proposition underlines one of the critical reasons open access platforms perform well---that open access platform designs preserve a large proportion of production. }


% \sout{However, open access platforms still suffer from selfish behavior that manifest in the misalignment between efficient allocations and Nash allocations. Contrasting to this, in \rone{Section \ref{sec:cap}}, we explore a platform targeted at \rone{enforcing an efficient} allocation.  }

% \ebc{(Eilyan says: What is a ``perfect allocation''? Also, it may not be clear to the reader which section ``next section'' is referring to.)} \johnp{John: Sorry about that. I mean to say efficient allocations. I have also changed next section to refer directly to Section 4. }

%We provide tight bounds on the price of anarchy of the networked Cournot game in an open access platform, under a variety of assumptions on firms' cost functions. 
%In particular, our tight price of anarchy bounds depend on the number of firms and also on the degree of asymmetry between firms' cost functions. These results improve upon the bounds presented in \citet{pang2017efficiency} and generalize those in \citet{johari2005efficiency} to the networked setting. Critical to these results is a property that the cost functions that maximize price of anarchy are linear ones, as in \citet{johari2005efficiency} for the non-networked case. 

\subsection{Worst-Case Cost  Profiles} \label{sec:worst_case_cost}

\eb{The following result reveals that, among all convex production cost functions satisfying Assumption \ref{ass:cost}, \emph{piecewise linear cost functions maximize the worst-case efficiency loss in networked Cournot games.} The result is also constructive in nature. That is, given a particular game and  cost profile satisfying Assumption \ref{ass:cost}, Lemma \ref{Lem:WorstCaseLinear} provides an explicit characterization of a piecewise linear cost profile that gives rise to a new game whose price of anarchy is no less than that of the original game. Thus, in constructing bounds on the price of anarchy associated with a particular game, it suffices to consider piecewise linear cost functions of the form specified in Lemma \ref{Lem:WorstCaseLinear}.}

% the worst case efficiency loss of networked Cournot games \eb{is} maximized at a cost function profile consisting of cost functions that are linear over the non-negative real numbers, demonstrating that any cost function profile $C$ as specified in Section \ref{sec:producer} can be correspondingly re-designed to construct a piecewise linear cost function profile $\overline{C}$, resulting in an increased worst case efficiency loss. In light of this result, in designing efficiency loss bounds guaranteed to hold for all cost functions belonging to the family specified in Section \ref{sec:producer}, it suffices to consider cost functions that are linear on $(0, \infty)$. 

%-------------------------------- Up to here! --------------------------------

%Such result are useful in facilitating the derivation of tight bounds on the price of anarchy for networked Cournot games in an open access platform. 

%The following lemma establishes piecewise linearity of the worst-case cost function profile. 
%Its proof is deferred to the Appendix.
%Its proof can be found in the extended version of this paper  \citet{linpangbitarwierman2017}.



\begin{lemma} \label{Lem:WorstCaseLinear}
	Let  $C = (C_1, \dots, C_n)$ be a cost function profile satisfying Assumption \ref{ass:cost}. Let $q^{\rm NE}( F \times M)$ denote the unique Nash equilibrium of the corresponding  networked Cournot game, and define the piecewise linear cost function profile $\overline{C} = (\overline{C}_1, \dots, \overline{C}_n)$ according to
	%$$\overline{C}_i (s_i) = \left( C_i' \left( \sum_{j=1}^m q_{ij}^{\rm NE} (\Kcal_{F. M}) \right) s_i \right)^+$$
	$$\overline{C}_i (s_i) := \left( \partial^+ C_i \left( \sum_{j=1}^m q_{ij}^{\rm NE} ( F \times M ) \right) \cdot s_i \right)^+$$
	for $i=1,\dots,n$, where $\partial^+ C_i$ denotes the right-derivative of the function $C_i$. It holds that  $$\rho (F \times M , C) \, \leq \,  \rho (F \times M, \overline{C} ).$$
\end{lemma}
We provide a complete proof of Lemma \ref{Lem:WorstCaseLinear} in the Appendix to this paper. The characterization of the worst-case cost  profile in Lemma \ref{Lem:WorstCaseLinear} will prove crucial to the derivation of tight upper bounds on the price of anarchy for the class of networked Cournot games considered in this paper. \eb{Specifically, 
under linear cost profiles, a networked Cournot game can be decoupled into $m$ single-market Cournot games,  each  corresponding to a distinct market in the original networked game.}




% One example of this simplification is that under linear cost function profiles, the networked Cournot game can essentially be decoupled into $m$ many different Cournot games with a single market since the marginal cost of each firm remain constant. In what follows, we examine the role played by \emph{(a)symmetry} in linear cost functions in determining platform efficiency. 



% We provide some intuition behind some of it's key arguments here.The social welfare achieved at a Nash equilibrium depends on the underlying cost function profile only through the firms' marginal costs at Nash equilibrium. This  follows from the fact that each firm's payoff function is concave in  its supply profile. Thus, by replacing the given cost profile with a  linear cost profile whose marginal costs are identical those of the original game at equilibrium, it can be shown that the Nash equilibrium of the new game
% has identical production quantities and a worse-off social welfare compared to the original one. A careful reader may notice here that the efficient social welfare may also decrease, but one can show that the decrease in the efficient social welfare is guaranteed to be no larger than that of the social welfare at Nash equilibrium.



\subsection{Efficiency Loss in Open Access Platforms}

\label{sec:efflossOAP}
\eb{Theorem \ref{thm:PoA_asym} reveals the possibility that increased competition in open access platforms may not always lead to increases in  platform efficiency. In what follows, we this investigate this behavior in more depth by examining the impact that producer  \emph{cost asymmetry}  has on  platform efficiency.}
%To facilitate our analysis, we restrict our attention to  production cost functions that linear over $(0, \infty)$.

% Before proving Theorem \ref{thm:PoA_asym}, we prove a result for the case where firms have symmetric costs. This help us show that the intuition that increased competition does indeed lead to less efficiency loss is indeed correct given the right assumptions.

% In proving Theorem \ref{thm:PoA_asym}, we devise worst case asymmetric cost functions compared to the one cost function utilized in the optimal case. Intuitively, since the optimal would only be utilizing the firm with the smallest marginal cost, the worst case family of cost functions should consist of one firm with a low cost and the remaining with high costs. As we increase the number of firms in this scenario, the set with high costs increase, leading to a slight increase in competition which however is inefficient. Another way to approach the counter-intuitive result is that the additional firm can always be designed to have arbitrarily large marginal cost, such that it does not participate, and therefore maintains the efficiency loss without its participation.  

% The worst case efficiency loss bounds under these two families of cost functions exhibit distinct behaviors in terms of their monotonicity in the number of firms $n$. We thus further explore the question as to how the degree of asymmetry between firms' cost functions might affect the efficiency loss in open access platforms. In doing so, we characterize tight worst case efficiency loss bounds when the underlying cost functions are restricted to be linear over $(0, \infty)$, and whose slope lies within a bounded interval  $[c_{\min}, c_{\max }] \subseteq \Rset_+$.




%We develop such bounds for cases in which firms have symmetric cost functions, or arbitrarily asymmetric cost functions, in which case we devise worst case asymmetric cost functions compared to the single cost function used in the optimal case (another benefit of linear cost functions in that marginal cost remains constant regardless of quantity produced). The price of anarchy bounds under these two families of cost functions, however, exhibit distinct behaviors in terms of their monotonicity in the number of firms $n$. We thus further explore the question as to how the degree of asymmetry between firms' cost functions might affect the efficiency loss in open access platforms. In doing so, we characterize tight price of anarchy bounds when the underlying cost functions are restricted to be linear over $(0, \infty)$, whose slope lies within a bounded interval  $[c_{\min}, c_{\max }] \subseteq \Rset_+$.


\subsubsection{Symmetric Cost Profiles}\label{subsec:symm}
We first consider the symmetric setting, where firms are assumed to have identical cost functions. 
%representing equally competitive producers. 
\eb{In Proposition \ref{prop:PoA_symm}, we establish a tight upper bound on the price of anarchy in this setting. The upper bound that we construct \emph{decreases monotonically} in the number of firms, and converges to one as the number of firms grows large---a behavior that is consistent with  classical competitive limit theorems for markets with symmetric firms \citep{mas1995microeconomic}.}



% conforms with the intuition that increasing (symmetric/perfectly competitive) suppliers strictly increases competition, and thereby reduce the extent to which any one producer might exert market power, improving the efficiency of platforms as selfish behavior becomes restricted. 

%We first 
%consider a special case of the Cournot game, where we
%assume that all firms are symmetric, i.e., have identical cost functions. Under this assumption, we characterize a tight price of anarchy bound for any number of firms $n$. As one might expect, the price of anarchy is decreasing in $n$, and converges to 1 as $n \to \infty$. 


\begin{proposition} \label{prop:PoA_symm}
	%Let Assumption \ref{ass:cost} hold. 
	Assume that $C_1 = C_2 = \cdots = C_n$.  The price of anarchy associated with the corresponding networked Cournot game $(F, \mathcal{Q}(F \times M), \pi)$ is upper bounded by
	\begin{align*}
	\rho (F \times M,C) \, \leq \, 1 + \frac{1}{(n  + 1)^2 - 1}.
	\end{align*}
	Additionally, this bound is tight. That is, there exists a symmetric cost  profile under which the upper bound is achieved.
	%$\overline{C}$ satisfying $\overline{C}_1 = \overline{C}_2 = \cdots = \overline{C}_n$, such that
	%\begin{align*}
	%\rho (\Kcal_{F, M}, \overline{C}) = 1 + \frac{1}{(n  + 1)^2 - 1}.
	%\end{align*}
\end{proposition}
%The proof of Proposition \ref{prop:PoA_symm} is provided in the Appendix.
%A detailed proof of Proposition \ref{prop:PoA_symm} is provided in the extended version of this paper \citet{linpangbitarwierman2017}. 


% \begin{proof}
% The proof is deferred to the Appendix.
% \end{proof}

We apply  \autoref{Lem:WorstCaseLinear} in proving Proposition \ref{prop:PoA_symm}, which reveals that the worst-case symmetric cost  profile is comprised  of $n$ identical cost functions that are linear on $(0, \infty)$. The complete proof of  \autoref{Lem:WorstCaseLinear} can be found in the  Appendix.

%A key step in proving \cref{prop:PoA_symm} is the application of  \cref{Lem:WorstCaseLinear}, revealing that the worst-case symmetric cost function profile consists of $n$ identical cost functions that are linear on $(0, \infty)$. The other details of the proof are deferred to the Appendix.

%The key step of the proof of \autoref{prop:PoA_symm} amounts to showing that the worst-case symmetric cost function profile consists of $n$ identical cost functions that are linear on $(0, \infty)$. \john{Isn't this just an application of Lemma 2? } \sam{That's true.}



% \subsubsection{Asymmetric Linear Cost Profiles}\label{subsec:asymm}
% We now consider the more general setting in which firms have arbitrary asymmetric cost functions satisfying the assumptions in Section \ref{sec:producer}, summarized in Theorem \ref{thm:PoA_asym}, where we establish a tight upper bound on the efficiency loss that is \emph{monotonically increasing} in the number of firms. In this case, it may seem counterintuitive that a perceived increased competition instead lead to efficiency loss. %It is important to note that in this case, the firms are under imperfect competition, and therefore the same intuition does not hold. 
% %the number of firms.  
% Its proof is provided in the Appendix. 


% %We now consider a more general setting of the networked Cournot game, where the cost functions of firms can be arbitrarily asymmetric. In the following theorem, we establish a tight price of anarchy bound that increases with the number of firms $n$. %Such a result reveals that the efficiency loss at Nash equilibrium can be increasing in the number of firms in the worst case.

% % \begin{theorem} \label{thm:PoA_asym2}
% % 	%Let Assumption \ref{ass:cost} hold. 
% % 	The price of anarchy associated with a cost function profile $C$ and the corresponding open access networked Cournot game $(F, \mathcal{Q}(F \times M), \pi)$ is upper bounded by
% % 	\begin{align*}
% % 	\rho (F \times M,C) \leq \frac{3}{2} \left( 1 - \frac{1}{3n+6} \right).
% % 	\end{align*}
% % 	The bound is tight if $\alpha_1 = \alpha_2 =  \cdots = \alpha_m$. %Namely, for any choice of $n$, there exists a cost function profile $\overline{C}$, such that
% % 	% \begin{align*}
% % 	% \rho (\overline{C}) =  \frac{3}{2} \left( 1 - \frac{1}{3n+6} \right).
% % 	% \end{align*}
% % \end{theorem}

% %The proof of Theorem \ref{thm:PoA_asym} relies on an explicit characterization of the cost function profile that maximizes the price of anarchy of the open access networked Cournot game.

% This seemingly counterintuitive result can occur if an expensive firm enters the market.
% First, note that  the entry of this new firm  results in an increase in aggregate supply at Nash equilibrium, because of increased `competition' in the market.
% However, its entry takes away production from its (cheap) competitors. 
% This manifests in a reduction in social welfare if the increase in production cost exceeds the increase in consumer utility. 
% %Such a counterintuitive behavior of Nash equilibrium was first analyzed in \citet{lahiri1988helping}, which shows that the removal of expensive firms might lead to an increase in social welfare in Cournot competitions with asymmetric cost. 
% Such a phenomenon is known as the ``excess entry theorem'' in the economics literature, e.g., \citet{suzumura1987entry, mankiw1986free, lahiri1988helping}, and reveals the possibility that a new firm's entry can lead to a reduction in social welfare.

% %\john{Such a phenomenon is known as the ``excess entry theorem'' in the Economics literature, which reveals the possibility that the entry of a new firm reducing social welfare \citet{suzumura1987entry, mankiw1986free, lahiri1988helping}.``I think possibility and can lead to are essentially saying the same thing, and so it is kinda repetitive..."}


% %This phenomenon is known in the Economics literature as the ``excess entry theorem'' \citet{suzumura1987entry, mankiw1986free, lahiri1988helping}, which reveals the possibility that the entry of a new firm can lead to a reduction in social welfare, largely attributed by the negative effect the entry has on the current participation. 



% %Consider the case in which the set of firms consist of one cheap firm and $n-1$ expensive firms. An increase in $n$ manifests in both an increase in the aggregate supply and a reduction in supply from the cheap firm. If the resulting increase in consumer welfare is less than the increase in production cost, an increase in the number of firms $n$ will manifest in a reduction in social welfare, and consequently, an increase in the price of anarchy.

% % Additionally, taking the number of firms $n \to \infty$ yields a worst case efficiency loss bound that is valid for any number of firms, and any number of markets, presented in Corollary \ref{cor:poabound}. This recovers the $3/2$ worst case efficiency loss or price of anarchy bound first established by \citet{johari2005efficiency} for a single market. % We have the following corollary.
% % % \begin{corollary}
% % % 	\label{cor:poabound}
% % % 	Open access platforms have a price of anarchy that is at most 3/2.
% % % \end{corollary}
% % %\sam{Perhaps we can present a comparison against the infocom PoA bound here?}
% %  In fact, under this generalized characterization, one can obtain both the previous result in their work, and for a networked market of any size with open access.


\subsubsection{Asymmetric Linear Cost Profiles}\label{subsec:asymm}
\eb{At first glance, the efficiency loss bounds established  in Proposition \ref{prop:PoA_symm} and Theorem \ref{thm:PoA_asym} may appear to stand in conflict.
If firms are symmetric, then the efficiency loss bound that we construct \emph{decreases} monotonically in the number of firms, approaching one asymptotically. If there is asymmetry in the cost structure across firms, however, then the corresponding efficiency loss bound that we establish \emph{increases} monotonically in the number of firms, approaching 3/2 as the number of firms grows large.
In what follows, we resolve this seeming discrepancy  by refining the structure of our efficiency loss bounds to reflect an explicit measure of cost asymmetry between firms. To facilitate our analysis, we restrict our attention to cost functions} that are linear on $(0, \infty)$, and whose slopes lie within  $[c_{\min}, c_{\max}] \subseteq \mathbb{R}_+$. We denote the space of all such cost functions by
% explore how the efficiency loss depends on the asymmetry between firms' cost functions, providing more intuition towards this counter-intuitive result, by restricting ourselves to cost functions that are linear on $(0, \infty)$, and whose slopes lie within  $[c_{\min}, c_{\max}] \subseteq \mathbb{R}_+$.
% That is, the efficiency loss bound is decreasing in $n$ if producers have symmetric cost functions but it is increasing in $n$ if producers are allowed to have asymmetric cost functions. In what follows, we explore how the efficiency loss depends on the asymmetry between firms' cost functions, providing more intuition towards this counter-intuitive result, by restricting ourselves to cost functions that are linear on $(0, \infty)$, and whose slopes lie within  $[c_{\min}, c_{\max}] \subseteq \mathbb{R}_+$.
% \begin{align*}
% \mathcal{L} (c_{\min}, c_{\max}) := \left\{C_0(x) = \left( cx\right)^+, ~  c \in [c_{\min}, c_{\max}] \subseteq \mathbb{R}_+ \right\}.
% \end{align*}
\begin{align*}
\mathcal{L} (c_{\min}, c_{\max}) := \left\{C_0: \Rset \to \Rset_+ \;  \Big| \; C_0(x) = \left( cx\right)^+, \right. 
~  c \in [c_{\min}, c_{\max}] \Big\}&.
\end{align*}
We write $C \in \mathcal{L}^n (c_{\min}, c_{\max})$ if the cost function profile $C$ satisfies $C_i \in \mathcal{L} (c_{\min}, c_{\max})$ for each  firm $i \in F$. 
%Clearly, the cost parameters $c_{\min}$ and $c_{\max}$ control the degree of asymmetry between firms' cost functions. 
\eb{We define a non-dimensional measure of cost asymmetry that is normalized according the maximum willingness to pay in each  market $j \in M$ according to}
% asymmetry between firms for each market $j \in M$. Specifically, for each market $j \in M$, define 
\begin{align}
\gamma_j :=  1 - \frac{ c_{\max} - c_{\min}}{\alpha_j - c_{\min}}.
\end{align}
It holds that $\gamma_j \in (-\infty, 1]$ if $c_{\min} < \alpha_j$. 
Clearly, $\gamma_j$ is increasing in consumers' maximum willingness to pay $\alpha_j$, and decreasing in the maximum marginal cost $c_{\max}$.  A value of $\gamma_j$ close to one implies a small degree of asymmetry between firms' cost functions relative to consumers' maximum willingness to pay in market $j$.

%A large value of $\gamma_j$ implies a small degree of asymmetry between firms' cost functions relative to consumers' maximum willingness to pay $\alpha_j$ in market $j$. 



%For this setting, we have the following proposition, which provides a tight price of anarchy bound for the networked Cournot game in an open access platforms, when firms have linear cost functions with bounded degrees of asymmetry. 

The following result provides a tight bound on the price of anarchy in open access platforms when firms have linear cost functions with a bounded degree of asymmetry. 
%Its proof is deferred to the Appendix.
\begin{proposition}
	\label{prop:linearcostspoa} Let $C \in \mathcal{L}^n (c_{\min},  c_{\max})$, and assume that 
	$c_{\min} < \max_{j\in M} \,  \{\alpha_j\}$. 
	%(that at least one firm would be willing to produce to one market). 
	The price of anarchy of  the corresponding networked Cournot game $(F, \mathcal{Q}(F \times M), \pi)$  satisfies
	\begin{align*}
	\rho (F \times M , C) \leq \dfrac{\displaystyle\sum_{j=1}^m  \frac{\left( (\alpha_j - c_{\min} )^+ \right) ^2}{\beta_j}}{\displaystyle\sum_{j=1}^m \left( \frac{2n+4}{3n+5}  + \delta (\gamma_j, n) \right) \frac{ \left( (\alpha_j - c_{\min} )^+ \right)^2}{\beta_j}},
	\end{align*}
	where 
% 	\begin{align*}
% 	\delta (\gamma, n): = \begin{cases}
% 	0, & \text{if } \displaystyle\gamma < \frac{2n+3}{3n+5}, \\
% 	\displaystyle\frac{(n-1) (3n+5)}{(n+1)^2} \left(  \gamma - \frac{2n+3}{3n+5} \right)^2,  & \text{otherwise } .
% 	\end{cases}
% 	\end{align*}
		\begin{align*}
	\delta (\gamma, n): = \begin{cases}
		\displaystyle\frac{(n-1) (3n+5)}{(n+1)^2} \left(  \gamma - \frac{2n+3}{3n+5} \right)^2, & \text{if } \displaystyle\gamma \geq \frac{2n+3}{3n+5}, \\
0,  & \text{otherwise } .
	\end{cases}
	\end{align*}
	The bound is tight if $\alpha_1 = \alpha_2 = \cdots = \alpha_m$.
	\label{prop:PoA_cmin_cmax}
\end{proposition}



%\red{
%\begin{align*}
%\rho (\Kcal_{F, M}, C) \leq \dfrac{\sum_{j=1}^m  \dfrac{\left( (\alpha_j - c_{\min} )^+ \right) ^2}{\beta_j}}{\sum_{j=1}^m  \dfrac{ r (\gamma_j, n) \left( (\alpha_j - c_{\min} )^+ \right)^2}{\beta_j}},
%\end{align*}
%where the function $r (\gamma, n)$ is defined according to
%\begin{align*}
%r (\gamma, n) = \begin{cases}
%\frac{2n+4}{3n+5}   & \text{if } \gamma < \frac{2n+3}{3n+5}, \\
%\frac{2n+4}{3n+5}  + \frac{(n-1) (3n+5)}{(n+1)^2} \left(  \gamma - \frac{2n+3}{3n+5} \right)^2  & \text{otherwise } .
%\end{cases}
%\end{align*}
%}



The price of anarchy bound established in Proposition \ref{prop:PoA_cmin_cmax} captures the impact that cost asymmetry has on efficiency loss through the 
market-dependent quantities $\delta (\gamma_j, n)$  for $j =1, \dots, m$. Crucially, each term  $\delta (\gamma_i, n)$ is nondecreasing in $\gamma_j$, revealing that a reduction in the degree of asymmetry in the cost structure across  firms translates to a reduction in the corresponding price of anarchy bound. \eb{As a corollary to this result, the price of anarchy bound in Proposition \ref{prop:PoA_cmin_cmax} reduces that of Proposition \ref{prop:PoA_symm} in the symmetric limit where $\gamma_j =1$ for all markets $j \in M$.} 

% The worst case efficiency loss bound specified in Proposition \ref{prop:PoA_cmin_cmax} depends on the degree of (a)symmetry between firms' cost functions only through the terms $\delta (\gamma_j, n)$  for $j =1, \dots, m$. In particular, as $\delta (\gamma, n)$ is non-decreasing in $\gamma$, a reduction in the degree of asymmetry between firms' cost functions manifests in a reduction in the worst case efficiency loss bound. 

%\subsection{Production Preservation of Open Access Platforms}


% Finally, we remark that the price of anarchy bound in  \cref{prop:PoA_cmin_cmax} may exhibit non-monotonic behavior in the number of firms $n$.
% More specifically,  consider the case in which the maximum willingness to pay $\alpha_j$ is identical across all markets $j \in M$.
% When $\gamma \leq 17/22$, this price of anarchy bound is monotonically increasing in $n$. On the other hand, when $17/22 < \gamma  < 1$, said price of anarchy bound decreases in $n$ for $1 \leq n \leq \left\lfloor  \frac{3\gamma - 2}{1 - \gamma} \right\rfloor$, and increases in $n$ for $n \geq \left\lfloor \frac{3\gamma - 2}{1 - \gamma} \right\rfloor + 1 $.



%The dimensionless parameter $\gamma$ can be best understood from a single market game. It serves as a measure of the degree of asymmetry between firms' cost functions relative to customers' maximum willingness to pay $\alpha$. 
%When $\gamma$ is small enough i.e. $\gamma <\frac{2n+3}{3n+5}$, the worst case occurs when the cost of the other firms are set to $c_i^*=c_{\textrm{max}}$, while if $\gamma$ is large, the optimal worst cost is feasible and is $c_i^*=\alpha_1 - \frac{2n+3}{3n+5} (\alpha_1 - c_{\textrm{min}})$. %In the second regime, as $\gamma$ increases towards $1$, the  
%In particular, when $c_{\min} < \alpha_1$, $\gamma \in (-\infty, 1]$, and a larger value of $\gamma$ implies a larger "degree of symmetry" between firms' cost functions relative to customers' maximum willingness to pay. To see this, first note that $\gamma \to 1$ as $c_{\max} \to c_{min}$, in which case all firms' cost functions becomes perfectly symmetric, and $\gamma \to -\infty$ as $c_{\max} \to \infty$, in which case all firms' cost functions can become arbitrarily asymmetric. Moreover, $\gamma \to 1$ as $\alpha_1 \to \infty$. In this case, as customers' maximum willingness to pay increases, customers become indifferent between different firms, and firms appear to be symmetric from customers' viewpoint.
%\red{We also make the following remark on the monotonicity of the worst case PoA in the number of firms $n$, depending on $\gamma$:}
% %In particular, if
% %$c_{\max} \to c_{\min}$, then all firms' cost functions becomes symmetric, and $\gamma \to 1$. On the other hand, if $c_{\max} \to \infty$, then firms' cost functions can be arbitrarily asymmetric, and $\gamma \to -\infty$.
%\john{Do note that this remark is for one market...}
%  \begin{remark}[Monotonicity of the Worst-case Price of Anarchy]
% A calculation on the worst-case price of anarchy in Proposition \ref{prop:PoA_cmin_cmax} reveals that when $\gamma \leq \tfrac{17}{22}$, the worst-case price of anarchy is monotonically increasing in $n$. On the other hand, if $\tfrac{17}{22} < \gamma  < 1$, then the worst-case price of anarchy decreases in $n$ for $1 \leq n \leq \left\lfloor \frac{3\gamma - 2}{1 - \gamma} \right\rfloor$, and increases in $n$ for $n \geq \left\lfloor \frac{3\gamma - 2}{1 - \gamma} \right\rfloor + 1 $.
% \end{remark}

% With the positive worst case efficiency loss results from open access platform designs, together with the result in Lemma \ref{lem:prodpres} that open access platform designs preserve a good proportion of demand fulfilled, we explore in the next section the platform design that controls allocations on behalf of the participating firms, allowing them to only decide their production quantity. 



==> 2020_ OR_ Net Cournot and Platforms/prelims.tex <==
%prelims
\label{sec:prelims}

\eb{In this paper, we adopt a model of platform competition in which firms compete  \'{a} la Cournot to produce a homogeneous product in multiple markets, where the platform serves to mediate the interactions between firms and markets.  Within this framework, we examine three distinct approaches to platform control: \emph{open access}, \emph{discriminatory access}, and \emph{controlled allocation} designs, as illustrated in Fig. \ref{fig:platforms}. In open access platforms, all firms are given access to all markets. In discriminatory access designs, the platform  explicitly controls (restricts) the set of markets that each firm is given access to. In controlled allocation designs, the platform determines the allocation of supply across the different markets given quantity offers from the different firms.} 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{platformdesigns2.pdf}
    \caption{\eb{From left: (a) open access platforms allow all firms access to all markets, (b) discriminatory access platforms restrict the set of markets that each firm has access to, and (c) controlled allocation platforms determine the allocation of supply to markets given quantity offers from the firms. All edges are directed from firms (circular nodes) to markets (square nodes), and removed for clarity.} }
    \label{fig:platforms}
\end{figure}



\eb{At the heart of our models for open and discriminatory access platforms is a directed bipartite graph $(F, M, \mathcal{E})$ that specifies the set of markets that each firm is given access to.}
Here, $F := \{1, \dots, n\}$ denotes the set  of $n$ firms,   $M := \{1, \dots, m\}$ denotes the set  of $m$ markets, and 
$\mathcal{E} \subseteq F \times M$ denotes the set of  directed edges connecting firms to markets. That is to say, $(i,j)\in \mathcal{E}$ if and only if  firm $i \in F$ has access to market $j \in M$. In what follows, we develop mathematical models for each of these three classes of platform designs.


%In general, the efficiency of such marketplaces depends on the structure of the underlying graph, which restricts the set of markets to which each firm has access. A crucial role that the platform might play in this setting is, therefore, the selection of markets that are made available to each firm. Potentially, connections can be allowed through open access or a carefully selected through discriminatory access. \textcolor{blue}{This may mean that only a sub-graph of the original complete bipartite graph is retained. }Additionally, in a controlled allocation platform, an alternative way for a platform to moderate the system is to direct each firm's production to various markets; that is, given the quantity of production decided by the firms, the platform dictates its allocation to the markets.
%The goal of this paper is to contrast and optimize different approaches for platform design.  As such, 
%In what follows, we examine these three classes of platform designs: \emph{open access} platforms, \emph{controlled allocation} platforms and \emph{discriminatory access} platforms.  



%In this paper, we aim to  \sam{quantify the effect of access and allocation control on the worst-case efficiency loss in online platforms.}  In doing so, \sam{we adopt a model of networked competition}, where the platform allows multiple producers to have access to multiple markets. 
% 
%Specifically, we describe the competition in online platforms according to the \textit{networked Cournot competition} model introduced in  \citet{abolhassani2014network} and \citet{bimpikis2014cournot}. As a generalization of the classical model of Cournot competition, the networked Cournot model captures settings in which firms compete to produce a homogeneous good in \emph{multiple markets}, where each market is potentially only accessible by a subset of the firms.  %The existence of a platform allows firms to participate in a broader set of markets than they could independently. Firms' decisions are connected across markets through an aggregate production cost while decisions across firms are connected via a single price from each market. 
%\sam{In spite of its simplicity, the networked Cournot model has proved useful in studying the strategic interactions between producers in networked environments---see, for example, \citet{jing1999spatial} and \citet{hobbs2001linear}.}




% The core of the model is a network specifying the connections between firms and markets. It is described by a directed bipartite graph $(F, M, \mathcal{E})$.
% %which describes  connecting firms to markets. This graph determines which firms participate in which markets. We represent the graph as follows.  
% Here, we denote by $F := \{1, \dots, n\}$ the set  of $n$ firms,   $M := \{1, \dots, m\}$ the set  of $m$ markets, and 
% $\mathcal{E} \subseteq F \times M$ the set of  directed edges connecting firms to markets where $(i,j)\in \mathcal{E}$ if and only if  firm $i$ has access to market~$j$. 

% \rone{To illustrate the model, let us consider a few examples.  In the case of ridesharing, each producer (or consumer) represents the set of drivers (or riders) in a particular neighborhood.  The edges represent neighboring neighborhoods where drivers may be assigned to riders by the platform.  Thus, the production level is a function of how many drivers  choose to drop offline rather than be assigned a new ride, e.g., drivers that are ``chasing the surge.'' Similarly, when considering an e-commerce scenario, each producer represents a firm selling a particular good and each consumer represents demand from a geographical region (e.g. country or state).  The edges represent which firms can ship products to which regions. Since the demand of the consumers are geographically separate, price differentiation across consumer regions is possible.}

%\sam{\textbf{Sam:} I removed the paragraph on ``illustrative examples" here, as Section \ref{sec:applications} talks about such examples in details.}

%\sam{We specify the set of markets that each firm has access to according to a directed bipartite graph $(F, M, \mathcal{E})$. Here, we denote by $F := \{1, \dots, n\}$ the set  of $n$ firms,   $M := \{1, \dots, m\}$ the set  of $m$ markets, and $\mathcal{E} \subseteq F \times M$ the set of  directed edges connecting firms to markets. That is to say, $(i,j)\in \mathcal{E}$ if and only if  firm $i$ has access to market~$j$.}

% The networked Cournot competition model may not capture some important aspects of platform designs, such as the possibility for platforms to set prices or dynamically match agents. However, endogenous price formation allows us to focus on access and allocation control. In fact, the Cournot model has been prominent in many applications, such as analyzing the efficiency loss in electricity markets, e.g., \citet{jing1999spatial,hobbs2001linear}. 

%We consider two types of platform designs in this work: one corresponds to platforms that perform access control, and the other corresponds to platforms that directly control the allocation of supply between different markets. In access control platforms, we specify the set of markets that each firm has access to according to a directed bipartite graph $(F, M, \mathcal{E})$. Here, we denote by $F := \{1, \dots, n\}$ the set  of $n$ firms,   $M := \{1, \dots, m\}$ the set  of $m$ markets, and  $\mathcal{E} \subseteq F \times M$ the set of  directed edges connecting firms to markets. That is to say, $(i,j)\in \mathcal{E}$ if and only if  firm $i$ has access to market~$j$.
 

\subsection{Open Access Platforms}
\eb{In open access platforms, all firms are given access to all markets. Examples of such platforms 
include eBay and Etsy, where every customer is shown every retailer that sells the item she desires.
Mathematically, open access platforms can be described according to networks  $(F, M, \mathcal{E})$ with a complete set of directed edges from firms to markets given by $\Ecal = F \times M$.} 


\eb{We now  introduce the various components that form the basis for our model of networked Cournot competition in open access platforms.} We discuss how to adapt this model to accommodate controlled allocation and discriminatory access platform designs in the following sections.






%An open access platform allows all firms to freely access all markets. This corresponds to the complete set of directed edges from firms to markets,  i.e., $\Ecal = F \times M$..  Examples of open access platforms  include eBay and Etsy, where every customer is shown every retailer that sells the item she desires.  These platforms thrive on fairness, transparency, and increased production and competition.



 %need to define the producer model, market model, and our main objective, social welfare. We introduce them for open access designs and then discuss how they change for controlled allocation and discriminatory access designs in the subsequent sections. 

\emph{Producer model:} \label{sec:producer}
In open access platforms, each firm determines how much it will produce in each market. Accordingly, we let $\production_{ij} \in \Rset_+$  denote the quantity produced by firm $i$ in market $j$, and let $\production_i :=  ( \production_{i1}, \dots, \production_{im} ) \in \mathbb{R}_+^m$ denote the supply profile associated with firm $i$. We define the set of feasible supply profiles from firm $i$ as
$$\Qcal_i (F \times M) := \left\{ x \in \mathbb{R}_+^m \, \left| \, x_j = 0, \ \forall \ (i, j ) \notin F \times M \right.  \right\}.$$ 
We  denote the supply profile across all producers by $q:=(q_1, \dots, q_n)$, and define the corresponding set of feasible supply profiles from all firms  by $\mathcal{Q} (F \times M) := \prod_{i = 1}^n \mathcal{Q}_i (F \times M)$. We let $\supply_i \in \mathbb{R}_+$ denote the aggregate quantity produced by each firm $i \in F$. It is given by
\begin{equation}
\supply_i := \sum_{j=1}^m \production_{ij}. 
\end{equation}
\eb{The cost incurred by each firm $i$ to produce an aggregate quantity $s_i$ is defined according to $\cost_i (\supply_i)$, where   $\cost_i: \mathbb{R} \rightarrow \mathbb{R}_+$ denotes each firm's  production cost function.}  We let $C := (C_1, \dots, C_n)$ denote the cost function profile across all firms, \eb{which is treated as common knowledge.} \eb{The cost functions considered in this paper are assumed to satisfy the following assumption.
\begin{assumption}  \label{ass:cost}
Each firm's  cost function $\cost_i$ is assumed to be convex, differentiable on $(0,\infty)$, and satisfy $\cost_i(x)=0$ for all $x\le 0$. 
\end{assumption}}







\emph{Demand model:}
As is standard in Cournot models of competition, we model price formation in each market according to a commonly known inverse demand function.
%Since we consider Cournot competition, given the production quantities, the price in a market is determined by the total supply to the market through an inverse demand function.  
Similar to \citet{bimpikis2014cournot}, we restrict our attention to affine inverse demand functions throughout this paper. Specifically, the price in each market $j \in M$ is determined according to 
$$\price_j(\demand_j):=\demlim_j - \demrate_j \demand_j,$$
where $\demand_j :=  \sum_{i=1}^n \production_{ij}$  denotes the aggregate quantity supplied to market $j$. The parameters $(\alpha_j, \beta_j)$ are  assumed to be strictly positive  for all $j \in M$.


%Here, $\demlim_j > 0$ measures consumers' maximum willingness to pay, and $\beta_j > 0$ measures the price elasticity of demand. We describe the price formation here and describe the competition model and equilibrium analysis in Section \ref{subsec:ncm}.


%for each market $j \in M$, its total supply $\demand_j$ is given by
%\begin{align}
%\demand_j := \sum_{i=1}^n \production_{ij},  \label{eq:dj}
%\end{align}
%and then the price $\price_j$ at market~$j$ is given by 
%$$\price_j(\demand_j):=\demlim_j - \demrate_j \demand_j,$$
%where $\demlim_j > 0$ measures consumers' maximum willingness to pay, and $\beta_j > 0$ measures the price elasticity of demand.
%$\demlim_j$ and $\demrate_j$ are market specific parameters.  The \emph{demand curve} of market~$j$ characterizes the price $\price_j$ as a function of demand $\demand_j$.  

%\sam{I think we may need to inline $p_j (d_j)$. This function is used in the definition of $SW(q, C)$.}\john{good now?}

%\sam{I presented the definition of SW prior to the game, as Lemma 1 uses the definition of SW.}

\emph{Social welfare:}
We measure the performance of a platform according to the \textit{social welfare} that it generates at equilibrium. The maximization of social welfare benefits both buyers and sellers,  promoting  platform growth in the long run. 
%Amazon, in its Buy Box design, believes that welfare measures such as availability, fulfillment, and customer service ultimately lead to increased customer satisfaction, and thereby, promote its growth in the long run, as observed in \citet{chen2017observing}. 
Social welfare is defined as aggregate consumer utility 
minus the aggregate production cost. Specifically, the social welfare induced by a particular supply profile $\production$  is given by
	\begin{align}
	\label{eq:welfare-def}
	\SW(\production,\cost) := \sum_{j=1}^m \int_0^{\demand_j}\price_j(z) \: \dd z - \sum_{i=1}^n \cost_i(\supply_i),
	\end{align}
where $\supply_i :=  \sum_{j =1}^m q_{ij}$ denotes the aggregate supply of firm $i \in F$  and $\demand_j := \sum_{i=1}^n q_{ij}$ denotes the aggregate demand in market $j \in M$. \eb{We have made explicit the dependence of social welfare on the cost profile $\cost$  to facilitate later discussions and proofs, where we quantify the dependence of social welfare on the underlying cost profile.} The \emph{efficient social welfare} associated with a cost  profile $\cost$ and the edge set $F\times M$ is defined as:
\begin{equation}
\SW^*(F\times M,\cost) := \sup_{\production \in \mathcal{Q}(F\times M)}~ \SW(q,\cost).
\end{equation}
%\hufu{Is the notation $\mathcal{Q (F \times M)}$ defined?}
Under the the paper's standing assumptions, it is straightforward to show that the above supremum is achieved, and that the set of efficient supply profiles is non-empty. In Section \ref{sec:disc_acc}, we adapt the definition of efficient social welfare to the setting of discriminatory access platforms.

\subsection{Controlled Allocation Platforms}
\eb{In the family of controlled allocation platform designs that we consider, firms choose their individual production levels, while the platform determines the allocation of the resulting aggregate supply across the different markets to maximize a combination of aggregate consumer surplus and  producer revenues.}
%The controlled allocation platform design is an attempt to pursue the socially optimal supply profile by controlling the allocation of the firms' aggregate supply to each market.
%  In an ideal world, if the firms produce at optimal levels, then the optimal social welfare can be attained. 
%\sam{In controlled allocation platforms}, firms continue to retain control over their production level. %
In ridesharing platforms, for example, drivers typically determine the number of hours that they work, \eb{while the platform determines the specific rides that they're matched to, and, as a result, the geographic regions (markets) that they are routed to.} \rone{In reality, drivers can also influence (in part) the market that they serve by choosing to go offline and reroute to different regions.}\ebc{[Eilyan says: This is not a perfect example of controlled allocation platforms, as I would not necessarily equate the matching of drivers to riders with  ``market allocation''. Rather, drivers can influence (in part) the market that they serve by choosing to go offline and reroute to different regions.]} %\johnp{( John: I agree this is not a perfect example. We can either provide some caveats around this example which is a nice motivating example, or let's try to think of a better example.)} \adam{I think sticking with this should be fine.}
%and which \sam{area they want to start in}, but largely not the riders they serve, i.e., the market in which they produce. %This also implies that the price formation, i.e., market model, under the controlled allocation platform design are not as simple as open access designs.   \hufu{The last sentence wasn't quite clear to me when I first read it.}
 
%  \rone{Ridesharing platforms have revolutionize transportation in cities and change the ways users today view car ownership. Behind the success of ridesharing are platforms who carefully set prices for rides and match riders to drivers, which (i) sufficiently provides an incentive for driver participation, (ii) ensure reasonable waiting time for riders, and (iii) careful subsidies that further improve participation on both sides, to thrive on \textit{network effects} in these networked marketplaces.}

More formally, in a controlled allocation platform, 
%is again specified by production cost functions $C_1, \cdots, C_n$ and inverse demand functions $p_1, \ldots, p_m$.  
each firm $i \in F$ chooses its aggregate production quantity $s_i \in \mathbb{R}_+$, incurring a production cost $C_i(s_i)$. \eb{The platform determines the aggregate quantity $d_j \in \mathbb{R}_+$ supplied to each market $j \in M$, subject to the constraint $\sum_{j=1}^m d_j \leq Q$, \sam{where $Q := \sum_{i=1}^n s_i$.}
We consider a family of market clearing mechanisms where the platform determines the allocation of supply to maximize a convex combination of consumer surplus and producer revenue, given by
\begin{align*}
    \textrm{OBJ}(d; \lambda) := \lambda \cdot \CS(d) + (1- \lambda) \cdot \REV(d),
\end{align*}
where $\textrm{CS}: \Rset_+^m \rightarrow \Rset$ and $\textrm{REV}: \Rset_+^m \rightarrow \Rset$ 
denote the  aggregate consumer surplus and aggregate producer revenue functions, respectively. They are given by}
\rone{
\begin{align*}
    \CS(d) &:= \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)\textrm{dz} - \demand_j\price_j(\demand_j),\\
    \REV(d) &:= \sum_{j=1}^m  \demand_j\price_j(\demand_j).
\end{align*}} 
\eb{The parameter $\lambda \in [0,1]$ can be specified by the platform to tradeoff the competing interests of  consumers and  producers. For example, setting $\lambda = 1/2$ results in a platform objective function $\textrm{OBJ}(d; 1/2)$ that corresponds to aggregate consumer utility.} 
% \ebc{[Eilyan says: We originally said that maximizing $\textrm{OBJ}(d; 1/2)$  corresponds to maximizing social welfare -- but I find this to be misleading, as the platform's decisions cannot directly affect producer costs. Rather, the platform is explicitly maximizing total consumer utility in this case. Let's make sure to fix this discussion if it appears in other places as well.]} \johnp{(John: that's right, this is the only point that cites $\lambda = 1/2$. It is true that technically $\lambda =1/2$ corresponds to consumer utility and I should have been precise)}
%\rone{
%We consider a \ market clearing mechanism in which the platform allocates the aggregate production from firms to different markets to maximize an objective function $\textrm{OBJ}(d; \lambda)$, a convex combination of consumer surplus and revenue determined by $\lambda$, defined as 
%\begin{align*}
    %\textrm{OBJ}(d; \lambda) = \lambda \cdot \CS(d) + %(1- \lambda) \cdot \REV(d).
%\end{align*}
%In $\textrm{OBJ}(d; \lambda)$, the parameter $\lambda$ allows the platform to balance the interests of the consumers (in maximizing consumer surplus CS) and producers (in maximizing revenue REV), defined as: 
%\begin{align*}
    %\CS(d) &:= \sum_{j=1}^m %\int_0^{\demand_j}\price_j(z)\textrm{dz} - %\demand_j\price_j(\demand_j),\\
    %\REV(d) &:= \sum_{j=1}^m  %\demand_j\price_j(\demand_j)
%\end{align*}
%This family of objective functions covers a range of popular objective functions. For example, one can show that the controlled allocation platform maximizing $\textrm{OBJ}(d,1/2)$ is a social welfare maximizing platform (since the choice over $d$ does not affect production cost $C_i(s_i)$). 
\rone{Given a particular choice of $\lambda \in [0,1]$, the controlled allocation platform performs the following optimization to determine the allocation of supply to each market:}
\eb{
\begin{align}
\label{opt:cont} \textrm{maximize} ~&~ \textrm{OBJ}(d;\lambda)\\
\nonumber \textrm{subject to}   ~&~ \sum_{j=1}^m d_j =  Q,
\end{align}
where $Q \in \mathbb{R}_+$ is determined by the firms, and $d \in \mathbb{R}_+^m$ is the platform's decision variable.} \eb{Given an efficient allocation $d$, we  assumed that firms are remunerated according to a \emph{uniform pricing mechanism} that is also \emph{budget balanced}. The unique pricing mechanism $p: \mathbb{R}_+^m \rightarrow \mathbb{R}$ that satisfies these criteria is given by  
\begin{equation}\label{eq:capprice}
p\left(  d\right) := \frac{\sum_{j=1}^m d_j p_j(d_j)}{\sum_{j=1}^m d_j}.
\end{equation}
Controlled allocation platforms, being defined in this manner, can be interpreted as giving rise to a multi-leader, single-follower Stackelberg game, where  firms choose their production quantities simultaneously, in anticipation that price will be determined according to \eqref{opt:cont}-\eqref{eq:capprice}. In specifying the firms' payoff functions in Section \ref{sec:cap}, it will be convenient to express the optimal solution to the platform's optimization problem \eqref{opt:cont} in the form of an \emph{allocation function} $A_\lambda:\mathbb{R}_+ \rightarrow \mathbb{R}^m_+$, which maps the aggregate production quantity $Q = \sum_{i\in F} s_i$  to an allocation $d$. We have parameterized the allocation function in terms of $\lambda$ to emphasize its dependence on the specific  objection function being optimized by the platform.}

% \johnp{(John: I wanted to make clear that while the allocation function can typically be more general, in this paper we just need it to correspond to a particular platform objective function which we parameterize by $\lambda$.)}


\eb{Given a supply profile $s \in \Rset_+^n$, one can express the \emph{social welfare} derived under the controlled allocation platform according to
\begin{align}
\label{eq:welfare-def-stack}
\SW(\supply, \lambda) := \sum_{j=1}^m \int_0^{d_j} \price_j(z) \: \dd z - \sum_{i=1}^n \cost_i(\supply_i),
\end{align}
where $d = A_\lambda \big(\sum_{i \in F} \supply_i \big)$.
}
\rone{Here, we have made explicit the dependence of social welfare on the platform objective parameter $\lambda$ to facilitate the presentation of our results in the sequel.} \eb{We also note that, while we have reused the notation $\SW(\cdot, \cdot)$  in  defining  the  social welfare function associated with each platform design, the specific platform being considered when examining social welfare will always be clear from the surrounding context.}


% \rone{Under this setting, given $\lambda$ and the corresponding allocation function $A_\lambda$, we simplify and overload the definition of social welfare $\SW$, expressing it as a function of the supply vector $s$:
% \begin{align}
% \label{eq:welfare-def-stack}
% \SW(\supply, \lambda) := \sum_{j=1}^m \int_0^{A_\lambda(\sum_{i \in F} \supply_i)_j}\price_j(z) \: \dd z - \sum_{i=1}^n \cost_i(\supply_i),
% \end{align}
% where $A_\lambda(\sum_{i \in F} \supply_i)_j$ is the platform allocation of aggregate supply $\sum_{i \in F} \supply_i$ to market $j$ when the platform objective is parameterized by $\lambda$. Here, we make the explicit dependence of social welfare on the platform objective parameter $\lambda$ to facilitate the presentation of results later, where we quantify the dependence of social welfare of a networked Stackelberg game on the platform objective. }




% \ebc{[Eilyan says: Is there a specific reason why the inequality $\sum_{j=1}^m d_j\leq Q$ in the platform's optimization problem \eqref{opt:cont} isn't stated as an equality constraint. I ask, because this may lead to some confusion in how the market clearing mechanism is interpreted. If an allocation $d$ is such that the inequality is not binding, then the question of  how production levels are determined needs to be addressed explicitly. Since (based on Eq (8)), each firm still assumed to produce $s_i$, it should be stated explicitly that the excess supply is spilled or lost.] -- (JP: Indeed, that is a typo. I have changed that in the main text. Having the potential inequality actually breaks some of our arguments. )} 


% social welfare.
% From each firm's perspective, this gives rise to an ``aggregate inverse demand'' function: given the production levels of the other firms, a firm~$i$, when producing quantity~$\sum_i s_i$, 
%which results in equal prices across active markets.
% Given that the inverse demand function in each market is affine, the resulting ``aggregate" inverse demand function is piecewise linear. %This platform turns out to be equivalent to the networked Stackelberg game defined in \citet{xu2017efficiency}. 
%\hufu{It wasn't clear to me what the ``aggregate inverse demand'' is: whether it refers to the market as a whole, or the inverse demand faced by one firm when the other firms' production is fixed.  The rest of the subsection doesn't seem to answer that, so I just removed the sentence for now.}
% To see this, we analyze the platform's allocation that 
% % first define the platform's action, assuming it 
% aims to maximize social welfare. 
% The platform takes the aggregate production $Q=\sum_{i=1}^ns_i$ (a quantity it has no control over), and performs the following optimization to decide the allocation $d_j$ to market~$j$:
% % perform the social welfare maximizing allocation to the different markets: 
% \begin{align*}
% \max_{d_1,d_2,\dots,d_m}~&~ \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)\: \dd z - \sum_{i=1}^n \cost_i(\supply_i)\\
% s.t. ~&~ \sum_{j=1}^m d_j\leq Q
% \end{align*}
% In Section \ref{sec:cap}, we consider a larger family of market clearing mechanisms, in which the platform is allowed to use objective functions that differ from the social welfare. 
% \begin{align*}
% \max_{d_1,d_2,\dots,d_m}~&~ \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)dz \\
% s.t. ~&~ \sum_{j=1}^m d_j\leq Q
% \end{align*}
% In general, allocations are equivalent for all objective functions that are equivalent modulo functions of the firms' productions, e.g., cost. %One such example from above is that controlled allocation platforms maximizing social welfare and consumer welfare are essentially the same platform and make the same allocations. 
% \rone{Given $Q$, the controlled allocation platform maximizes its objective function $\text{OBJ}(d; \lambda)$, a convex combination of consumer surplus and revenue determined by $\lambda$, defined as 
% \begin{align*}
%     \text{OBJ}(d; \lambda) = \lambda \cdot \text{CS}(d) + (1- \lambda) \cdot \text{REV}(d).
% \end{align*}


% \sam{\textbf{TODO:} describe the family of objective functions under consideration here. This will make the exposition a lot cleaner.}

% Given the platform's objective, % e.g., maximizing social welfare, 
% or the corresponding choice of $\lambda$, the firms fully understand how their aggregate productions are to be allocated across the markets, and act together as joint leaders in a Stackelberg game. %The formal definition of the Stackelberg game will be presented in Section \ref{subsec:ncm}. 
% %As an example of 
% To illustrate such an allocation process, a social welfare maximizing controlled allocation platform ($\lambda$ = 1/2) will start allocating from the market with the highest willingness to pay and, as that market's price decreases with fulfilled demand, transition into markets with decreasing willingness to pay, keeping prices constant across the set of markets receiving positive supplies.  In general, an \emph{allocation function} $A:\mathbb{R}_+ \rightarrow \mathbb{R}^m_+$ 
% %can then be defined that 
% takes as input the aggregate production $Q = \sum_{i\in F} s_i$ and outputs the corresponding allocations to the markets $d=(d_1,d_2, \dots, d_m)$. 

% For objectives other than the social welfare, prices may not be the same among markets that receive supplies.  We will assume that the platform still pays the same per-unit price~$p$ to all firms that produce, where $p$ 
% % For concreteness, we assume also that in optimizing other objective functions where prices may not be equal in active markets that the per-unit price $p$ paid to the firms is universal and 
% is the average price over the demand fulfilled, or more formally defined by: 
% \begin{equation}\label{eq:capprice}
% p\left(  d\right) = \frac{\sum_{j=1}^m d_j (\alpha_j - \beta_j d_j)}{\sum_{j=1}^m d_j}.
% \end{equation}



\subsection{Discriminatory access platforms} \label{sec:disc_acc}
A discriminatory access platform restricts the set of markets that can be accessed by each firm in the form of an edge set $\Ecal\subseteq F \times M$. This restriction may be designed to improve producer surplus, consumer surplus, or social welfare. An example of a discriminatory access platform design is Amazon's Buy Box, where Amazon chooses a default seller based on a score that is based on product pricing, availability, fulfillment capabilities, and customer service records. Operationally, these restrictions prevent certain firms from accessing certain markets. We encode these restrictions in form of sparsity constraints on the supply profile of each firm. Formally, each firm~$i$ determines the quantity~$\production_{ij}$ that it supplies to each market~$j$, subject to the restriction 
% In particular, we require 
that $\production_{ij} = 0$ for all $(i, j) \notin \Ecal$. We denote the set of feasible supply profiles associated with each firm $i \in F$ by
$$\Qcal_i (\Ecal) := \left\{ x \in \mathbb{R}_+^m \, \left| \, x_j = 0, \ \forall \ (i, j ) \notin \Ecal \right.  \right\}.$$
We denote the set of feasible supply profiles across all firms by $\mathcal{Q} (\Ecal) := \prod_{i = 1}^n \mathcal{Q}_i (\Ecal)$. In studying  discriminatory access platform designs, we assume that the supplier cost functions and  demand functions are identical to those considered in the context of open access platform designs. 

%and its competition model is described in Section \ref{subsec:ncm}. 
% \subsection{Producer Model} \label{sec:producer}
% Under both the open and discriminatory access platform models, each firm decides its producing quantity to each market. We let $\production_{ij} \in \Rset_+$  denote the quantity produced by firm $i$ in market $j$, and let $\production_i :=  ( \production_{i1}, \dots, \production_{im} ) \in \mathbb{R}_+^m$ denote the supply profile from firm $i$. In the controlled allocation platform model, the firm would not be able to decide its allocations and only control its aggregate supply, i.e., in that case, $\production_i = \sum_{j=1}^m \production_{ij}$ and the platform decide each $\production_{ij}$ such that $ \sum_{j=1}^m \production_{ij}=\production_i$. In the access platform models, we require that $\production_{ij} = 0$ for all $(i, j) \notin \Ecal$, and define the set of feasible supply profiles from firm $i$ as:
% $$\Qcal_i (\Ecal) := \left\{ x \in \mathbb{R}_+^m \, \left| \, x_j = 0, \ \forall \ (i, j ) \notin \Ecal \right.  \right\}.$$ 
% Trivially, the feasible supply profiles from firm $i$ under the controlled allocation platform model is just $\Qcal_i := \{x \in \mathbb{R}_+\}$. 
% We denote the supply profile from all firms by $\production:= (\production_1, \dots, \production_n) \in \Rset_+^{mn}$ ($\Rset_+^{n}$ for the controlled allocation platform model). Accordingly, the set of feasible supply profiles from all firms is given by $\mathcal{Q} (\Ecal) := \prod_{i = 1}^n \mathcal{Q}_i (\Ecal)$. In the controlled allocation platform model, the set $\Ecal$ correspond to the full bipartite graph, as in open access, since this would allow the platform most room and flexibility for optimization. 
%The production cost of each firm $i \in F$ depends on its supply profile only through its aggregate production quantity, which is given by  %More specifically, the aggregate production quantity of firm $i$ is given by 
% We let $\supply_i$ be the aggregate production quantity of firm $i \in F$. It is given by
% \begin{equation}
% \supply_i := \sum_{j=1}^m \production_{ij}. 
% \end{equation}
% The resulting production cost of firm $i$ is defined by $\cost_i (\supply_i)$ or $\cost_i(q_i)$ in the controlled allocation case. We assume that the cost function $\cost_i$ is convex, differentiable on $(0,\infty)$, and satisfies $\cost_i(x)=0$ for all $x\le 0$. (This family of cost functions represents a generalization of previous work \citet{pang2017efficiency}, which assumed that all firms have quadratic cost functions.) Finally, we define $C := (C_1, \dots, C_n)$ as the cost function profile.
% \subsection{Market Model}
% As is standard in Cournot models of competition, we model price formation according to an inverse demand function in each market.  
% %Since we consider Cournot competition, given the production quantities, the price in a market is determined by the total supply to the market through an inverse demand function.  
% Similar to \citet{bimpikis2014cournot}, we restrict our attention to affine inverse demand functions throughout this paper. Specifically, the price in each  market $j \in M$ is determined according to 
% $\price_j(\demand_j):=\demlim_j - \demrate_j \demand_j,$
% where $\demand_j$  denotes the aggregate quantity supplied to market $j$,  given by
% \begin{align}
% \demand_j := \sum_{i=1}^n \production_{ij}.  
% \end{align}
% Here, $\demlim_j > 0$ measures consumers' maximum willingness to pay, and $\beta_j > 0$ measures the price elasticity of demand.
% %for each market $j \in M$, its total supply $\demand_j$ is given by
% %\begin{align}
% %\demand_j := \sum_{i=1}^n \production_{ij},  \label{eq:dj}
% %\end{align}
% %and then the price $\price_j$ at market~$j$ is given by 
% %$$\price_j(\demand_j):=\demlim_j - \demrate_j \demand_j,$$
% %where $\demlim_j > 0$ measures consumers' maximum willingness to pay, and $\beta_j > 0$ measures the price elasticity of demand.
% %$\demlim_j$ and $\demrate_j$ are market specific parameters.  The \emph{demand curve} of market~$j$ characterizes the price $\price_j$ as a function of demand $\demand_j$.  
% \subsection{Social Welfare}
% In this paper, we measure the performance (or efficiency) of a platform according to \textit{social welfare}. For platforms, the pursuit of social welfare benefits both buyers and sellers, and in the long run, promotes their expansion.
% For example, 
% Amazon (in its Buy Box design) believes that welfare measures such as availability, fulfillment, and customer service  ultimately lead to increased customer satisfaction, and thereby, promote its growth in the long run \citet{chen2017observing}. 
% We adopt the standard notion of social welfare defined as aggregate consumer utility less total production cost.
% \begin{definition}
% 	Specifically, the social welfare associated with a supply profile $\production$ and a cost function profile $\cost$ is defined according to
% 	\begin{align}
% 	\label{eq:welfare-def}
% 	\SW(\production,\cost) := \sum_{j=1}^m \int_0^{\demand_j}\price_j(z)dz - \sum_{i=1}^n \cost_i(\supply_i),
% 	\end{align}
% 	where $\supply_i$ and $\demand_j$ are defined in Eqs. (1) and (2), respectively.
% \end{definition}


We define the \emph{efficient social welfare} 
% \ebc{[Eilyan says: We use the term optimal social welfare in the open access section. Let's stick with one terminology throughout the paper. While I prefer efficient to optimal, I'm fine with either.]} \johnp{(John: I did a search over all occurences and changed all "optimal social" to "efficient social".)} \ebc{[Eilyan says: There may be other occurrences related to ``optimal supply profile'', etc.]} \johnp{(John: Checked through one more time for all the other stray ones. Feel free to do a quick scan too! )} 
associated with an edge set $\Ecal$ and a cost function profile $\cost$ as
\begin{equation}
\SW^*(\Ecal, \cost) := \sup_{\production \in \Qcal(\Ecal)}~ \SW(q,\cost).
\end{equation}
A supply profile $\production \in \Qcal(\Ecal)$ is said to be efficient with respect to a given edge set $\mathcal{E}$ if it satisfies $\SW(\production,\cost) = \SW^*(\Ecal,\cost)$. It is straightforward to verify that the above supremum is  attained, and that the set of efficient supply profiles is non-empty. 

%Having now described the economic models for all the platforms, we are ready to present the networked Cournot competition for access control designs and the networked Stackelberg competition for allocation control designs. 

\subsection{Networked Competition Model}\label{subsec:ncm}
We now introduce the game theoretic models that we use to characterize market equilibrium in each of the  three platform designs considered in this paper.

\subsubsection{Competition under open access and discriminatory access platforms:} 
%We describe the network Cournot competition for the open and discriminatory access platforms according to Nash, where no producers can deviate to obtain a better outcome.  
%Given the models above, our focus is on the Nash equilibrium of the resulting game.  
We consider profit maximizing firms, where the payoff function $\pi_i$ for each firm $i \in F$ is defined as
\begin{equation}
\profit_i(\production_i,\production_{-i})  := \sum_{j=1}^m \production_{ij}\price_j(\demand_j)
- \cost_i (\supply_i).
\end{equation}
Here, $q_i$ denotes the supply profile of firm $i$, and $\production_{-i}=(q_1, .., q_{i-1}, q_{i+1}, .., q_n) $ denotes the supply profiles of all firms not including firm $i$, and $d_j := \sum_{i=1}^n q_{ij}$ denotes the aggregate quantity consumed in each market  $j \in M$.

%\adam{introduce the $-i$ notation} \sam{This was done in the notations part in intro. Would it be easier for the reader if we put it here?}  \adam{I think so. This is the first place we use it right? } \sam{That's true. And I believe that it's probably the only place we use such a notation.}
% where $p_j$ is a price formed based on the total demand $\demand_j$ in market $j$. We denote by $\profit :=(\profit_1,\dots,\profit_n)$ the collection of payoff functions of all firms. 

\eb{Given an edge set $\Ecal \subseteq F \times M$,} the triple $(F,\Qcal(\Ecal),\profit)$ defines a normal-form game, which we refer to as a \emph{networked Cournot game}. \eb{Depending the particular choice of edge set, the \emph{networked Cournot game} can be used to describe competition in either open access platform designs ($\Ecal = F \times M$), or discriminatory access platform designs ($\Ecal \subset F \times M$).}
% that we employ to study both open access and discriminatory access platform designs. We refer to the resulting game as the \emph{networked Cournot game} associated with the edge set $\Ecal$. 
%
We describe the \eb{family of  stable outcomes} associated with each  networked Cournot game using the concept of Nash equilibrium.

\begin{definition}[Nash Equilibrium]
	\emph{A supply profile $\production \in \mathcal{Q}(\Ecal)$ constitutes a \emph{pure strategy Nash equilibrium} of the game $(F,\mathcal{Q}(\Ecal),\profit)$ if for every firm $i\in F$, it holds that $\profit_i(\production_i,\production_{-i}) \ge \profit_i(\overline{\production}_i,\production_{-i})$ for all  $\overline{\production}_i \in \mathcal{Q}_i (\Ecal)$.} 
\end{definition}

Under the assumptions of convex cost functions and affine inverse demand functions, \citet{abolhassani2014network} have previously shown that the networked Cournot game is an ordinal potential game. Additionally, it admits a unique Nash equilibrium, which can be characterized as the unique optimal solution to a particular convex program.
%and the Nash equilibrium is the unique optimal solution to a convex program. Consequently, the networked Cournot game associated with any edge set $\Ecal \subseteq F \times M$ admits a unique Nash equilibrium. }
We summarize the results of \citet{abolhassani2014network} in the following lemma.

\begin{lemma}\label{lem:NE} \citep{abolhassani2014network}
	The game $(F, \Qcal(\Ecal), \pi)$ admits a unique Nash equilibrium $q^{\rm{NE}}(\Ecal) \in \Qcal(\Ecal)$ that is the unique optimal solution to the following convex program:
	\begin{equation}
	\begin{alignedat}{8}
	&\underset{q \in \Qcal(\Ecal)}{\text{\rm maximize}} \quad && \SW (q, C) - \sum_{i=1}^n \sum_{j=1}^m \frac{\beta_j q_{ij}^2}{2}  .
	\end{alignedat} \label{opt:NE}
	\end{equation} 
\end{lemma}


In general, the supply profile at the unique Nash equilibrium 
%of the networked Cournot game 
may not coincide with the  efficient supply profile. The potential loss of efficiency is can be measured according to the \emph{price of anarchy} of the underlying game \citep{KP99}. %Implicit in Definition \ref{def:PoA} is the fact that the networked Cournot game admits a unique Nash equilibrium. 
In the remainder of the paper, we use the terms \emph{worst-case efficiency loss} and \emph{price of anarchy} interchangeably. 
\begin{definition}[Price of Anarchy] \label{def:PoA} \emph{Given an edge set $\Ecal$ and cost function profile $C$, we define the \emph{price of anarchy (PoA)} associated with the corresponding networked Cournot game $(F, \mathcal{Q}(\Ecal), \profit)$  as
	\begin{align*}
	\rho (\Ecal, C) :=  \frac{\SW^* (F\times M, C)}{\SW \left( q^{\textrm NE} (\Ecal), C \right) }.
	\end{align*}
	 We define $\rho (\Ecal, C) := 1$ if both $\SW^* (F \times M, \cost)  = 0$ and $\SW (\production^{\rm NE} (\Ecal), \cost)=0$.} 
	%for all $q \in \mathcal{Q}_{\rm{NE}}$, and $\rho (C) = \infty$ if $\mathcal{Q}_{\rm{NE}} = \emptyset$.
\end{definition}

It is worth noting that, in games that may exhibit a multiplicity of Nash equilibria, the price of anarchy is typically defined as the ratio of the efficient social welfare over that of the Nash equilibrium with the \emph{lowest} social welfare. 
%and is no less than $1$. 
Since each of the networked Cournot games considered in this paper admits a unique Nash equilibrium, \eb{this more general definition of price of anarchy reduces to the one specified in Definition \ref{def:PoA}.}
%we do not explicitly define price of anarchy or the worst case efficiency loss over all possible equilibrium. 
It's also worth mentioning that, in our definition of price of anarchy, the social welfare at Nash equilibrium is always measured against the efficient social welfare, which is defined  in terms of the complete edge set $F \times M$.



%We first formally define the networked Stackelberg game, %first introduced in \citet{xu2017efficiency}. We 
% and extend their results and show that the equivalent networked Stackelberg game can possibly have no equilibria, a unique equilibria or even multiple equilibria. We will then prove Theorem \ref{thm:ineff}, before giving results for controlled allocation platforms optimizing a myriad of objectives that are convex combinations of consumer surplus and aggregate profit in Theorem \ref{thm:generalcap}. 

\subsubsection{Competition under controlled allocation platforms:}
We model competition in controlled allocation platforms according to a multi-leader, single-follower Stackelberg game. 
% A Stackelberg competition model includes a leader, who moves first, and a follower, who moves sequentially after. The leader is assumed to know the best response of the follower (dependent on the move it makes), and solves by backward induction the optimal choice to make, i.e., the quantity to produce. 
\eb{In this context,  firms lead by determining their aggregate production quantities simultaneously, in anticipation of the  platform's allocation of the resulting aggregate supply across the different markets according to \eqref{opt:cont}, and the subsequent determination of price according to \eqref{eq:capprice}.}
% the platform best responds by allocating the aggregate production to maximize an objective function made known beforehand to the firms, e.g., social welfare. Having defined the allocation function $A$ and the price $p$ in Eq. \eqref{eq:capprice},
\eb{Letting $s_i \in \Rset_+$ denote the aggregate quantity supplied by each firm $i\in F$, the payoff derived by each firm under the controlled allocation \eqref{opt:cont}, pricing mechanism \eqref{eq:capprice}, the platform objective defined by $\lambda$, and its corresponding allocation function $A_\lambda$, can be explicitly defined as 
\begin{equation}
\pi_i(s_i, s_{-i}; \lambda) := s_i p\left(A_\lambda\left(\sum_{i=1}^n s_i\right)\right) -C_i(s_i).
\end{equation}}
\rone{We overload the use of the notation $\pi_i$ in the setting here in a slight abuse of notation, but the operating definition will be clear from the context. Based on this, we introduce the definition of a Stackelberg equilibrium in the networked Stackelberg game. }
% \ebc{[Eilyan says: Do you need to make $A$ an explicit argument to $\pi$? If so, make sure that this is reflected throughout the paper. For example, the payoffs used in teh definition below are inconsistent with this notation. Also, you should mention that the overloaded use of the notation $\pi_i$ for payoff in the two different setting is a slight abuse of notation, but that the operating definition will always be clear from the context....]} \johnp{(John: Together with the POA part, I think that having $A$ being mapped in a 1-1 fashion to a $\lambda$ is the best option in my head, and I will try to update it to be consistent. I do hope it reads better and clearer this way. I have noted on the overloaded notation too. )}
%We adopt this model from the work of \citet{xu2017efficiency} where they also consider a networked Stackelberg model with constrained capacity.
% \sam{\textbf{Sam:} I removed the qualitative description of the standard Stackelberg model, as this is a basic microecon concept.}
\rone{\begin{definition}[Stackelberg Equilibrium]
\emph{The supply profile $s \in \Rset_+^n$ constitutes a \emph{Stackelberg equilibrium} of the networked Stackelberg game with platform objective parameterized by $\lambda$ if $\pi_i(s_i,s_{-i}; \lambda) \ \geq \ \pi_i(\overline{s}_i,s_{-i}; \lambda)$ for all $\overline{s}_i \in \Rset_+$ and  every firm $i \in F$. When multiple equilibria exists, we let $\rm{SE} \subset \Rset_+^n$ denote the \emph{set of Stackelberg equilibria} associated with the networked Stackelberg game.} 
\end{definition}}
% Given the allocation function $A$, a Stackelberg equilibrium $s^{SE}$ is defined : 
% $$
% \pi(s_i^{SE},s_{-i}^{SE}) \geq \pi(s_i,s_{-i}^{SE}), ~\forall s_i\geq 0
% $$
%Unlike the networked Cournot competition for the access control designs, Lemma \ref{lem:NE} above does not hold since the networked Stackelberg game for the controlled allocation design is significantly different in that firms do not control their allocations and that there can be multiple equilibria instead. %Additionally, the worst case efficiency loss or price of anarchy in that case is defined similarly, but is taken as the maximum multiplicative factor $\rho$ over all Stackelberg equilibria. 


\eb{We note that the family of  networked Stackelberg games studied in this paper is similar in spirit to the class of games  considered in \citet{cai2017role, xu2017efficiency}.}  In this earlier work, it is shown that networked Stackelberg games may possess (i) no Stackelberg equilibrium, (ii) a unique Stackelberg equilibrium, or (iii) multiple Stackelberg equilibria.
\eb{Taking these different possibilities into account, we define the price of anarchy associated with the networked Stackelberg game as follows. }
% whereby the platform first commits to allocations based on its objective and the firms act first by selecting their production, privy to how the platform distributes production. Under the networked Stackelberg competition, there exists systems with (i) no Stackelberg equilibrium, (ii) a unique Stackelberg equilibrium, and (iii) multiple Stackelberg equilibria.
\rone{\begin{definition}
	\emph{The \emph{price of anarchy} $\rho(\lambda, M)$ associated with the networked Stackelberg game with platform objective function determined by $\lambda$ and a set of markets $M$ is defined as 
    % $$
    % \rho(C,M) = \argmin_{s \in \textrm{SE}}\frac{\SW^*(F\times M,C)}{\SW(s)},
    % $$
    \eb{$$
    \rho(\lambda, M) := \sup_{s \in \rm{SE}} \ \frac{\SW^*(F\times M,C)}{\SW(s, \lambda)},
    $$}
    with set of firms $F$ having the corresponding set of cost functions $C$ . We define $\rho(\lambda, M) := \infty$ if $\rm{SE} = \emptyset$, and $\rho (\lambda, M) := 1$ if both $\SW^* (F \times M, \cost)  = 0$ and $\SW(s, \lambda)$ = 0.}
\end{definition}
In this context, we have to chosen to make explicit the dependence of the price of anarchy on the platform parameter $\lambda$ and the set of markets $M$ to facilitate the presentation of our main results. We also note that, while we have reused the notation $\rho(\cdot, \cdot)$  in  defining  the  price of anarchy function associated with each platform design, the specific platform being considered will always be clear from the surrounding context.}
% \ebc{Eilyan says:
% \begin{itemize}
%     \item Again,  the fact that the notation $\rho$ is being overloaded needs to be mentioned. Also, it would be nice to try to maintain some symmetry in the arguments across the two definitions for $\rho$, e.g., $\rho(M,C)$ matches $\rho(\Ecal, C)$ in the second argument. 
%     \item Notice that I've replaced the $\argmin$ operator with $\sup$. Make sure to fix this error if it appears elsewhere. 
%     \item $SW(s)$ does not appear to be defined anywhere.
%     \item You also need to deal with the case $\rho = 0/0$ when defining the PoA.
%     \item You should explain why you have made the dependence on C and M explicit in defining $\rho$.
%     \item In the paper, some definitions are italicized, some are not. Please be consistent throughout the paper.
% \end{itemize}}
% \johnp{John says: Thanks for the comments! 
% \begin{itemize}
%     \item (For point 5 as well) After some thought, I have decided to have $\rho$ here as a function of the operator objective parameter $\lambda$ and the set of markets $M$. This is because the results around price of anarchy of this part revolves around these. I have tried to maintain symmetry in the sense that $\lambda$ is controllable by the platform. 
%     \item Sorry about that. Must have been a typo when we defined price of anarchy in the opposite manner for the infocom paper! Thanks for noticing. 
%     \item $SW(s)$ is now defined and also defined as $\SW(s,\lambda)$ for completeness. 
%     \item I have ensured that the $0/0$ case is now answered for, 
%     \item and fixed the consistency for definitions to be all italicized. 
% \end{itemize}}
%An example where an equilibrium does not exist can be found in \citet{xu2017efficiency}, while the single market case always leads to a unique equilibrium, and our result for unbounded price of anarchy for a social welfare maximizing controlled allocation platform will include an example for a system with multiple equilibria. For controlled allocation platforms maximizing objectives other than social welfare, the equilibrium under a networked setting is much harder to attain and the examples we have usually have only one firm, and often have zero production cost. 
\rone{\subsection{Illustrative applications}} \label{sec:applications}

\rone{In what follows, we discuss connections of our platform models to ridesharing and e-commerce.  
Note that we are not seeking to model all details of these applications. Rather, our objective is to illustrate the relevance and limitations of applying our networked Cournot model to these practical settings. 
}

\rone{\emph{Ridesharing.} \sam{Ridesharing platforms can be modeled as a controlled allocation platform. Specifically, collection of drivers located in a common geographical region can be approximately modeled as a single firm,} \sam{where the number of rides provided by drivers in that regions can be modeled 
as the firm's production quantity.
Importantly, a supply-side model of this type can capture the strategic withholding of supply (rides) from the drivers.
% A market, on the other hand, corresponds to the aggregation of customers in a geographical region whose destinations are in a ride requests have mileage that falls in a specific range.
A market, on the other hand, corresponds to a collection of customers whose current locations and ride destinations correspond to a specific pair of geographical regions.
%
In practice, the platform matches each ride request to an available driver nearby according to the solution of an online matching problem. In the context of controlled allocation platforms, we provide a simplified description of this matching mechanism according to the market clearing mechanism specified in \eqref{opt:cont}.}
% Similarly, a market is an aggregation of consumers in a geographical region. Drivers can choose to turn off their applications to drive to other regions, thereby withholding production. Additionally, they can  communicate with one another and turn off their applications, withholding production in an aggregate sense.  Both of these behaviors are quite common and are impacted significantly by the platform pricing and matching policies.
} 

\sam{Modeling ridesharing platforms in this manner enables the analysis of the efficiency loss in ridesharing platforms that is associated with the supply withholding from the driver side. In Section \ref{sec:cap}, we show that such efficiency loss might be infinitely large for a range of market clearing mechanisms. The limitation of this model, however, is that it does not enable the description of the dynamic evolution of the supply and the demand side that is driven by the spatial movements of the drivers and the riders.}

% \begin{itemize}
%     \item What are the producers and suppliers
%     \item What is the market clearing mechanism
%     \item What insights could we glean from the model
% \end{itemize}

% \sam{Sam: I rewrote the discussion on ridesharing platforms in a simpler way in order to more clearly reflect the insights we could glean from the model.}

% Corresponds to ride originating in their current zone 

% Not able to capture the dynamics of the model

% \rone{To model the behavior of an individual, it is natural to break down the driver's cost into two parts: (i) fuel and other vehicular costs such as maintenance, and (ii) opportunity cost such as other sources of income or limitations on the hours of ridesharing. The first part of this cost is linear in the amount of ``production'', while the latter is usually convex in production (consider health concerns, fatigue, working hours, etc.). On the consumer side, consumers within a geographical region have different ``willingness to pay", which results in a decreasing inverse demand function in aggregate.  Thus, our assumptions on the supply and demand sides of the market are satisfied.  However, the model is only useful at a macro-level, and does not capture dynamics around demand and driver positioning, etc. }

% \sam{I think the specific discussions on what the cost functions and inverse demand functions should be removed. Delving into such details seems like opening a Pandora's box for attacks from the reviewers.}

% \rone{In terms of the behavior of the platform, to a first-order level, it is natural to think of the ridesharing platform as a controlled allocation platform that assigns drivers to riders to optimize a particular objective, e.g., profit or social welfare. Of course, other factors also play a role in assignment too.  However, since our analysis focuses on the production incentives created by the assignment of the platform, the crucial factor is how the matching is determined.  In particular, using the model, we can effectively illustrate the underlying factors pushing drivers to withhold production and the inefficiency this creates. }

% \rone{In a more direct fashion, the analysis from this work can also be used to study brokers that play the roles of a ``platform in a platform", such as what SMart did for deliveroo in 2016, see \citet{vandaele2019algorithm}. Under these settings, the broker typically employs these gig economy workers and has control over where and how they work. Similar brokers exist in ridesharing markets such as for Didi premium vehicle drivers in China.}

\rone{\emph{E-commerce.}} \sam{Depending on its method of access control, e-commerce platforms like Ebay, Amazon, or Alibaba can be described as open access or discriminatory access platforms.}
\rone{For example, Amazon can be viewed as a discriminatory access platform, where the Buybox is used to identify and highlight a single seller based on performance measures such as pricing, reviews and shipping. In contrast, eBay and Etsy can be viewed as open access platforms. Alibaba serves similarly as a platform between manufacturers, suppliers/exporters, and importers. }
\sam{In this paper, we quantify the worst-case efficiency loss in open access and discriminatory access platforms. Our results reveal insights on the efficiency gain that can be attained by access control in e-commerce platforms.}


\sam{
Specifically, we use the networked Cournot model to describe the interaction between the sellers of a single product in e-commerce platforms.
A market corresponds to the aggregation of consumers in a particular geographical region.  A producer, on the other hand, corresponds to one seller of the single product under consideration. 
The set of markets that each producer has access to depends on the method of access control in the platform.
The decision variable of each producer is assumed to be his production quantity at each market he has access to.
Note that although producers do not directly specify their production quantities in e-commerce platforms, this Cournot model is still potentially useful in helping predict the production capacity that each firm builds out in the long run.
Specifically, as is pointed out in \citet{kreps1983quantity}, the price and production levels at the unique Cournot equilibrium are identical to the price and production levels at the unique subgame perfect equilibrium of a two-stage game, in which firms first choose their capacities (\`a la Cournot) in Stage 1, followed by a choice of prices (\`a la Bertrand) in Stage 2, where production levels are set according to the capacity levels chosen in Stage 1.
}

% To use the networked Cournot model in the context of e-commerce platforms, we focuse on a particular item.
% A producer corresponds to one seller of the said product, 
% while a market is an aggregation of consumers in a particular geographical region. 
% When supply is scarce, sellers can withhold production to manipulate prices, as was observed for masks and other protective equipment during the recent 2019 Coronavirus pandemic. 

%

% \sam{
% The main insight we obtain through the analysis of such networked Cournot models is the role of access control in e-commerce platforms.
% Specifically, in Section \ref{sec:oap} and \ref{sec:dap}, we quantify the worst-case efficiency loss in open access and discriminatory access platforms, and establish conditions on producers' cost functions under which the efficiency gain from allocation control is large.
% % Specifically, in open access platforms, each producer has access to all markets; in discriminatory access platforms, however, the set of markets that each producer has access to is determined by the platform.
% % , and highlight the potential efficiency gain that can be attained through access control.
% }

% \sam{TODO: add a discussion on how Cournot model is aligned with the Bertrand-Edgeworth model.}

% \rone{An individual seller's cost in this case is mostly linear, representing the cost she may incur in procuring the item in the first place. As her sales grow, the tax and fees from the platform may grow, resulting in costs that may grow in a convex fashion. Consumers within a geographical region have different ``willingness to pay", resulting in a decreasing inverse demand function. Thus, our assumptions on the supply and demand sides of this market hold once again. }

% \rone{Existing e-commerce platforms are largely either open access or discriminatory access, and function primarily as a platform to connect consumers and sellers. For example, Amazon can be viewed as a discriminatory access platform, where the Buybox is used to identify and highlight a single seller based on performance measures such as pricing, reviews and shipping. In contrast, E-bay can be viewed as an open access platform. More broadly, there are a wide variety of platforms, e.g., Alibaba, that connect manufacturers, suppliers, exporters and importers for large quantities of goods in similar ways.  As in the case of ridesharing, the model should be used only at the macro-level, and does not capture the dynamics of inventory, etc.  However, the model can effectively highlight the inefficiency resulting from the production incentives created by the platform design.  }

% \sam{Sam: I removed the discussion on supply withholding during COVID-19, as this}

% [[rewrite this to mimic the ridesharing structure.  1st paragraph describe what producer/consumers are, second describe why our assumptions are satisfied, third describe the platform design and why the model is useful]] In this case of e-commerce, we consider each producer as a seller who perhaps engages in algorithmic pricing, or the automatic setting of prices based on inventory levels, e.g., as the inventory decreases, price rise. On the other hand, consumers on the platform are aggregated over different consumer regions or demographic classes, which each have different inverse demand functions. Unlike \citet{cai2018ranking} who studies ranking for price setting agents, we view open access more generally, i.e., as long as the platform does not highlight a particular seller for any one product. Applied to e-Commerce, discriminatory access platforms may be likened to Amazon, where a particular seller holds access to the Buybox, which is the default seller of the item. 



% \subsection{\textcolor{blue}{Discussion on the applicability of networked Cournot models}}

% \textcolor{blue}{In this part, , how it can be applied to different applications, and the limitations and explanatory power of our proposed model. }

% \subsection*{\textcolor{blue}{Comparison with Bertrand and Supply Function Models}}


% \textcolor{blue}{Our comparisons between Cournot, Bertrand and Supply Function models will }

% \textcolor{blue}{}


% \subsection*{\textcolor{blue}{The Ridesharing Market Example}}




% \subsection*{\textcolor{blue}{The Electricity Market Example}}

% \textcolor{blue}{The electricity grid relies on an electricity market governed by independent system operators (ISO), who ensures that the \textit{right prices} are set across the grid such that (i) supply meets demand, and that (ii) social welfare is maximized. To do this, the ISO usually receives quantity bids from producers and estimates demand over the grid, and optimizes flow in the network, resulting in prices that serves as \textit{optimal incentives} for the producers at those nodes to generate the right amount of power. The quantity bid that producers submit is in the form of a cost function, where producers agree to produce a certain amount for each cost. }

% \textcolor{blue}{When applied to electricity markets, each consumer in the networked Cournot model best models the entire set of consumers in a geographical location. }

% \subsection*{\textcolor{blue}{Model Limitations}}



% \subsection*{\textcolor{blue}{Model Explanatory Power}}




%Passing electricity from one node to another is not as trivial and straightforward as it seems. When these flow physics and constraints are not sufficiently considered, then flows may not be as calculated, and even if supply meets demand and social welfare is maximized, there are still supply-demand mismatch in individual nodes. These supply-demand mismatch means that some local generators need to work beyond their set-points to make up for this mismatch. Sustained supply-demand mismatch can lead to generator shutdowns, which can then cause blackouts, which further leads to cascading failures across the grid. 


==> 2020_ OR_ Net Cournot and Platforms/searchcosts.tex <==
% The model and analysis presented thus far considers production costs but not other costs which can also be on the consumer side, and may be monetary, e.g., transportation and communication, or non-monetary, e.g., search costs. Platform designs center around lowering entry costs for producers, oftentimes leading to increased production and competition, and lowering search costs for consumers. In this section, we present a simple search cost model which highlights the ability of the discriminatory access design to also consider search costs, and the distinction between open access and discriminatory access designs. 

% As we are working in the networked Cournot setting where demand is aggregated, we must use a simple model for search costs. We define a search cost for each consumer market $j$, $r_j$, on the consumers as a product of their consumer surplus (taking care of the simple assuring assumption that markets are rational and that search costs can never be more than their surplus) and a discount factor $f(n)$ which monotonically increases with the number of firms $n$, and lastly, a market-specific parameter $\theta$ highlighting potentially different market segments with differing search costs, defined as follows: 
% $$
% r_j = \theta f(n) CS_j, ~ 0\le \theta \le 1,
% $$
% where function $f$ has the following properties:
% $$
% f(1) = 0, \lim_{n\rightarrow \infty} f(n) = 1, f ~\text{monotonically increasing}
% $$


% %To further understand and motivate shifts towards controlled allocation and discriminatory access platforms, a model including search costs is introduced in this section. As mentioned, these costs, often not monetary, have various effects on different groups of people. Additionally, it also further motivate controlled allocation (and respectively discriminatory access) platforms in that search costs for buyers are minimal (respectively controlled) as compared to open access platforms which connects every possible firm. 

% % The search cost model for consumers in the networked Cournot setting for each market $j$ is defined below: 
% % $$
% % p_j = \theta f(n) CS_j, ~ 0\le \theta \le 1,
% % $$
% % where $\theta$ is a search cost parameter for the population, $CS_j$ refers to the consumer surplus at that market, and the function $f$ can be inferred from data, with the following properties: 
% % $$
% % f(1) = 0, \lim_{n\rightarrow \infty} f(n) = 1, f ~\text{monotonically increasing}
% % $$
% This search cost model ensures that (i) search cost penalties can never exceed consumer surplus---an assumption that search cost can never cause the market to receive negative utility, (ii) differentiation can be made through $\theta$ for low and high search cost participants, and that (iii) search cost increases in the number of firms exposed to - the effort or cost has to increase as the number of choices increase. 

% \begin{remark}
% Since controlled allocation platforms essentially make all decisions on allocation, the search cost is $0$ for consumers but continue to maintain its previous negative result from Section 4, implying that search costs has no effect on controlled allocation platforms.  
% \end{remark}

% In light of the difficulty to analyze without a further parametric form of $f(n)$, we assume hereafter that $f(n)$ assumes the form of $f(n) = \frac{n-1}{n+1}$, fulfilling the preceding properties we listed.

% Open access designs, by definition, presents all possible choices to consumers, allowing them to make production and allocation decisions, but also thereby incurring large search costs. In the following theorem, we highlight the impact of search costs on open access platforms. 

% \begin{theorem}\label{thm:openaccess-search}
% 	Open Access Platforms with search costs defined with $f(n)=\frac{n-1}{n+1}$ have worst case efficiency loss $\Omega(n)$. 
% \end{theorem}
% % \proof{Proof:} The proof is included in the Appendix. 
% % \endproof

% On the other hand, referring to Corollary \ref{cor:nine}, where the price of anarchy is $\frac{4}{3}$ at $n=1$ (which coincidentally incurs zero search cost) for discriminatory access platform designs, they maintain its worst case constant bound price of anarchy under linear cost functions and search costs. %In fact, this is true for any function $f$ that satisfies the above properties and is not restricted to the parametric form $f(n)=\frac{n-1}{n+1}$.

% %\begin{proposition}
% %	In a similar fashion, we can find that the price of anarchy in the asymmetric cost case can be written as follow: 
% %	$$
% %	\rho(K_{F,M},\overline{C}) \le \frac{1}{\frac{2n+4}{3n+5} + \delta(\gamma,n) -\theta f(n) \eta(\gamma,n)}
% %	$$
% %\end{proposition}

% %
% %
% % We consider a special example showing that misclassifying two market segments with different search costs as one can lead to inefficiency. In the simple example, we consider two market segments, one with high search costs $(\theta=1)$ and one with low ones $(\theta = 0)$. The key point is that to show that open access would result in a penalized price of anarchy, we show that finding an optimal set of firms for both segments would result still in inefficiency as compared to viewing the two market segments separately, similar to a discriminatory access platform would. 
% %
% %\begin{example}
% %	Under the setting where $f(n)$ is defined as $\frac{n-1}{n+1}$, the Price of Anarchy(PoA) can be written in the following simplified form (Note that when $n=1$, $PoA = \frac{3}{4}=0.75$.): 
% %	$$
% %	PoA(\theta) = \frac{2n+4}{3n+5} + \frac{(n-1)(3n+5)(\gamma - \frac{2n+3}{3n+5})^2}{(n+1)^2} - \theta \left(\frac{n-1}{n+1}\right)\left(\frac{\gamma(n-1) +1}{n+1}\right)^2 
% %	$$
% %	
% %	We first show that collectively considering the two different market segments with the same elasticity (We are comparing between two market segments that are typically mistaken to be one. Under the most general assumptions, they should behave almost identically and so we assume same elasticity. ) results in looking at one market with averaged search cost, essentially comparing $P_S = \frac{1}{2}(PoA(\theta_H)+PoA(\theta_L))$ against $P_J = PoA((\theta_H+\theta_L)/2)$, relying on the fact that optimal social welfare irregardless of $\theta$ since only one firm is needed there. 
% %	%Summarizing the simulation results, we have the following points to make: 
% %	%\begin{enumerate}
% %	%\item For $\theta_H$, the optimal number of firms remain as $1$ regardless of the value of $\gamma$. 
% %	%\item For $\theta_M$, the optimal number of firms remain as $1$ for $\gamma \leq 0.907 $ and $2$ otherwise.
% %	%\item For $\theta_L$, the optimal number of firms grow ``exponentially" in the value of $\gamma$. 
% %	%\item Consequently, $P_S$ grows immediately while $P_J$ only grows after $\gamma = 0.907$.
% %	%\end{enumerate}
% %	The metric of performance we are interested in can be written and defined as the following: 
% %	$$
% %	\tau = \min_\gamma \frac{1-P_S}{1-P_J}
% %	$$
% %	and can be understood as the ratio between the worst case losses in performances in the two cases. In both cases, the Price of Anarchy (PoA) is at least $0.75$ and therefore a direct comparison between the two PoA will lead to a multiplicative factor difference of at most $\frac{4}{3}$.
% %	
% %	\begin{proposition}
% %		For our similar two market segment example, the worst case $\tau$ factor is $\frac{27}{40}$. 
% %	\end{proposition}
% %	
% %	\proof{Proof: } To prove the above proposition, we will enumerate a list of lemmata, each of which will be proven in the appendix. 
% %	
% %	%Some obvious questions to ask are the following: 
% %	%\begin{enumerate}
% %	%\item Why is the transition at $0.907$? 
% %	%\item Why is $P_S$ increasing?
% %	%\item Why does $P_J$ stagnate at first and then increases after $0.907$? 
% %	%\item What is the worst case ratio $\tau$? 
% %	%\item Finally, a more difficult question is, what if market segments have different price elasticity? 
% %	%\end{enumerate}
% %	
% %	%\newpage
% %	\begin{lemma}\label{lem:agnostic-search}
% %		For the platform agnostic to the market segments with different search costs, the optimal strategy is to only show one firm for $\gamma < \frac{43}{65}+\frac{\sqrt[3]{\frac{114}{130}}}{130}\approx 0.9079$, and to show two firms otherwise. 
% %	\end{lemma}
% %
% %	This lemma highlights the two choices that the agnostic platform should make. It ends up always choosing only one or two firms depending on the symmetry of costs of the producing firms. This is clearly undesirable for the market segment with low search costs. 
% %	
% %	\begin{lemma}\label{lem:agnostic-search2}
% %		For the platform selecting firms for the market segments with high search costs, the optimal strategy is to always only show one firm. On the other hand, for the market segment with low search costs, the optimal number of firms increases as a function of $\gamma$, and in fact, transitions from $n$ to $n+1$ at $\gamma = 1-\frac{2n+3}{2n^2+10n+10} $. 
% %	\end{lemma}
% %	
% %	The optimal number of markets then for the three different search cost settings are $1$, either $1$ or $2$ and growing in $\gamma$ for the high, medium and low search cost platforms respectively. This characterization demonstrates the differing strategies and sheds light on the difference in performances we can expect. We next show the following lemma: 
% %	
% %	\begin{lemma}\label{lem:worstcase}
% %		The worse case $\gamma$ is exactly $\gamma = 1$, which yields an infinitely large optimal number of firms for the low search cost segment. The price of anarchy in the separate and joint optimization are $7/8$ and $22/27$ respectively. 
% %	\end{lemma}
% %	
% %	The result is easily obtained by computing our ratio of performance. This concludes our proof and example. \Halmos \endproof
% %	
% %\end{example}
% %$-------------------$Old Version Below$-------------------$

% Prior to this section, it seems that the performance guarantees attained by open access and discriminatory access platform designs are similar. This section presents a preliminary look at the impact of search cost on platform design, in particular highlighting the potentially post-search unbounded worst case efficiency loss result for open access platforms, and the flexibility of the discriminatory access platform design to consider search costs. It remains important to study this further, e.g., to find out how to optimize network design with search costs, or how computation or other costs involved may affect the performance of discriminatory access designs too.

%our aim was to highlight the trend towards discriminatory access despite its marginal improvement from a price of anarchy point of view in the previous sections in the absence of search costs. A simple search cost model shows that discriminatory access platforms have much more potential as compared to an open access one, and maintains its advantage over the controlled allocation platform. 

% Samples of sectioning (and labeling) in MOOR.
% NOTE: (1) all section levels end with a period,
%       (2) capitalization is as shown (sentence style, not title style).
%
%\section{Introduction.}\label{intro} %%1.
%\subsection{Duality and the classical EOQ problem.}\label{class-EOQ} %% 1.1.
%\subsection{Outline.}\label{outline1} %% 1.2.
%\subsubsection{Cyclic schedules for the general deterministic SMDP.}
%  \label{cyclic-schedules} %% 1.2.1
%\section{Problem description.}\label{problemdescription} %% 2.

% Text of your paper here

% Appendix here
% Options are (1) APPENDIX (with or without general title) or 
%             (2) APPENDICES (if it has more than one unrelated sections)
% Outcomment the appropriate case if necessary
%
% \begin{APPENDIX}{<Title of the Appendix>}
% \end{APPENDIX}
%
%   or 
%


==> DMAmacros.tex <==
% Theorem, Lemma, Propositions, etc

 %Classifies font styles of different math environments into 2 categories: definition and remark
\theoremstyle{plain} % plain, {definition}, remark (bold title, regular text)
%\newtheorem{theorem}{Theorem}[section]		% Option in [] specifies the name of the section level to use in numbering the theorem
\newtheorem{theore}{Theorem}
\newtheorem{corollar}{Corollary}
\newtheorem{lemm}[theore]{Lemma}
\newtheorem{definitio}{Definition}
\newtheorem{proble}{Problem}
\newtheorem{assumptio}{Assumption}
\newtheorem{propert}{Property}
\newtheorem{propositio}{Proposition}
\newtheorem{conjectur}{Conjecture}
\newtheorem{exampl}{Example}
\newtheorem{rul}{Rule}

%\theoremstyle{remark} % plain, definition, {remark} (title in italics, regular text)
\newtheorem{remar}{Remark}
\newtheorem{fac}{Fact}
\newtheorem{clai}{Claim}


\newcommand{\theorem}[1]{\begin{theore} {\rm #1} \hfill $\Box$ \end{theore}}
\newcommand{\corollary}[1]{\begin{corollar} {\rm #1} \end{corollar}}
\newcommand{\lemma}[1]{\begin{lemm} {\rm #1}  \hfill $\Box$ \end{lemm}}
%\newcommand{\definition}[1]{\begin{definitio} {\rm #1 } \hfill $\Box$ \end{definitio}}
\newcommand{\definition}[1]{\begin{definitio} {\rm #1 } \end{definitio}}
\newcommand{\problem}[1]{\begin{proble} {\rm #1 } \end{proble}}
\newcommand{\assumption}[1]{\begin{assumptio} {\rm #1 } \end{assumptio}}
\newcommand{\property}[1]{\begin{propert} {\rm #1 } \end{propert}}
%\newcommand{\proposition}[1]{\begin{propositio} {\rm #1} \hfill $\Box$ \end{propositio}}
\newcommand{\proposition}[1]{\begin{propositio} {\rm #1} \end{propositio}}
\newcommand{\conjecture}[1]{\begin{conjectur} #1 \end{conjectur}}
\newcommand{\example}[1]{\begin{exampl} {\rm #1} \end{exampl}}
%\newcommand{\proof}[1]{{\em Proof:} \, #1 \hfill $\Box$}
\newcommand{\remark}[1]{\begin{remar} {\rm #1} \hfill \hfill $\blacksquare$ \end{remar}}
\newcommand{\fact}[1]{\begin{fac} {\rm #1} \end{fac}}
\newcommand{\mrule}[1]{\begin{rul} {\rm #1}  \end{rul}}


%\newcommand{\assumption}[2]{\noindent {\bf A#1.} \, #2 \\}
%\newcommand{\assumption}[2]{\noindent {\bf A#1.}#2 \\}


% Beginnings and ends, equations
\def\nn{\nonumber}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqs{\begin{equation*}}
\def\eeqs{\end{equation*}}
\def\balign{\begin{align}}
\def\ealign{\end{align}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ba{\begin{array}}
\def\ea{\end{array}}
\def\bcenter{\begin{center}}
\def\ecenter{\end{center}}
\def\bitem{\begin{itemize}}
\def\eitem{\end{itemize}}
\def\benum{\begin{enumerate}}
\def\eenum{\end{enumerate}}
\def\bdoc{\begin{document}}
\def\edoc{\end{document}}
\def\defeq{{\stackrel{\Delta}{=}}}
\def\nn{\nonumber}


% Lattins
\def\eg{{e.g., \/}}
\def\etal{{\it et al. \/}}
\def\viz{{\iet viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\etc{{\it etc.,\ \/}}
\def\cf{{cf.,\ \/}}

% Colors:
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

%\def\red{\textcolor{red}}
%\def\blue{\textcolor{blue}}
\def\black{\textcolor{black}}
\def\yellow{\textcolor{yellow}}
\def\green{\textcolor{green}}
\def\tcbg{\textcolor{bgrd}}
\def\magenta{\textcolor{magenta}}
\def\white{\textcolor{white}}
\def\gray{\textcolor{gray}}

% User-specified command definitions/redefinitions
\newcommand\Quote[1]{\lq\textsl{#1}\rq}
\newcommand\fr[2]{{\textstyle\frac{#1}{#2}}}

%% Mathbb
\newcommand{\Ambb}{\mathbb{A}}
\newcommand{\Bmbb}{\mathbb{B}}
\newcommand{\Cmbb}{\mathbb{C}}
\newcommand{\Dmbb}{\mathbb{D}}
\newcommand{\Embb}{\mathbb{E}}
\newcommand{\Fmbb}{\mathbb{F}}
\newcommand{\Gmbb}{\mathbb{G}}
\newcommand{\Hmbb}{\mathbb{H}}
\newcommand{\Imbb}{\mathbb{I}}
\newcommand{\Jmbb}{\mathbb{J}}
\newcommand{\Kmbb}{\mathbb{K}}
\newcommand{\Lmbb}{\mathbb{L}}
\newcommand{\Mmbb}{\mathbb{M}}
\newcommand{\Nmbb}{\mathbb{N}}
\newcommand{\Ombb}{\mathbb{O}}
\newcommand{\Pmbb}{\mathbb{P}}
\newcommand{\Qmbb}{\mathbb{Q}}
\newcommand{\Rmbb}{\mathbb{R}}
\newcommand{\Smbb}{\mathbb{S}}
\newcommand{\Tmbb}{\mathbb{T}}
\newcommand{\Umbb}{\mathbb{U}}
\newcommand{\Vmbb}{\mathbb{V}}
\newcommand{\Wmbb}{\mathbb{W}}
\newcommand{\Xmbb}{\mathbb{X}}
\newcommand{\Ymbb}{\mathbb{Y}}
\newcommand{\Zmbb}{\mathbb{Z}}

%
%% MSC Letters
\newcommand{\Amsc}{\mathcal{A}}
\newcommand{\Bmsc}{\mathcal{B}}
\newcommand{\Cmsc}{\mathcal{C}}
\newcommand{\Dmsc}{\mathcal{D}}
\newcommand{\Emsc}{\mathcal{E}}
\newcommand{\Fmsc}{\mathcal{F}}
\newcommand{\Gmsc}{\mathcal{G}}
\newcommand{\Hmsc}{\mathcal{H}}
\newcommand{\Imsc}{\mathcal{I}}
\newcommand{\Jmsc}{\mathcal{J}}
\newcommand{\Kmsc}{\mathcal{K}}
\newcommand{\Lmsc}{\mathcal{L}}
\newcommand{\Mmsc}{\mathcal{M}}
\newcommand{\Nmsc}{\mathcal{N}}
\newcommand{\Omsc}{\mathcal{O}}
\newcommand{\Pmsc}{\mathcal{P}}
\newcommand{\Qmsc}{\mathcal{Q}}
\newcommand{\Rmsc}{\mathcal{R}}
\newcommand{\Smsc}{\mathcal{S}}
\newcommand{\Tmsc}{\mathcal{T}}
\newcommand{\Umsc}{\mathcal{U}}
\newcommand{\Vmsc}{\mathcal{V}}
\newcommand{\Wmsc}{\mathcal{W}}
\newcommand{\Xmsc}{\mathcal{X}}
\newcommand{\Ymsc}{\mathcal{Y}}
\newcommand{\Zmsc}{\mathcal{Z}}


%% Script Letters
\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}


% Tiny capital letters sub-super scripts
\def\Atiny{\mbox{\tiny{A}}}
\def\Btiny{\mbox{\tiny{B}}}
\def\Ctiny{\mbox{\tiny{C}}}
\def\Dtiny{\mbox{\tiny{D}}}
\def\Etiny{\mbox{\tiny{E}}}
\def\Ctiny{\mbox{\tiny{C}}}
\def\Ftiny{\mbox{\tiny{F}}}
\def\Gtiny{\mbox{\tiny{G}}}
\def\Htiny{\mbox{\tiny{H}}}
\def\Itiny{\mbox{\tiny{I}}}
\def\Jtiny{\mbox{\tiny{J}}}
\def\Ktiny{\mbox{\tiny{K}}}
\def\Ltiny{\mbox{\tiny{L}}}
\def\Mtiny{\mbox{\tiny{M}}}
\def\Ntiny{\mbox{\tiny{N}}}
\def\Otiny{\mbox{\tiny{O}}}
\def\Ptiny{\mbox{\tiny{P}}}
\def\Qtiny{\mbox{\tiny{Q}}}
\def\Rtiny{\mbox{\tiny{R}}}
\def\Stiny{\mbox{\tiny{S}}}
\def\Ttiny{\mbox{\tiny{T}}}
\def\Utiny{\mbox{\tiny{U}}}
\def\Vtiny{\mbox{\tiny{V}}}
\def\Wtiny{\mbox{\tiny{W}}}
\def\Xtiny{\mbox{\tiny{X}}}
\def\Ytiny{\mbox{\tiny{Y}}}
\def\Ztiny{\mbox{\tiny{Z}}}


%
%
%% Greeks Boldface
\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
%\def\Pibf{{\bf$\Pi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}

%
% BF letters
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\pbf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

\def\0bf{\mathbf{0}}
\def\1bf{\mathbf{1}}

\def\lambdabf{\boldsymbol{\lambda}}
\def\mubf{\boldsymbol{\mu}}
\def\gammabf{\boldsymbol{\gamma}}
\def\xibf{\boldsymbol{\xi}}
\def\sigmabf{\boldsymbol{\sigma}}
\def\zetabf{\boldsymbol{\zeta}}

\def\Lambdabf{\boldsymbol{\Lambda}}
\def\Mubf{\boldsymbol{\Mu}}
\def\Gammabf{\boldsymbol{\Gamma}}
\def\Xibf{\boldsymbol{\Xi}}
\def\Sigmabf{\boldsymbol{\Sigma}}
\def\Zetabf{\boldsymbol{\Zeta}}




==> searchcosts.tex <==
% The model and analysis presented thus far considers production costs but not other costs which can also be on the consumer side, and may be monetary, e.g., transportation and communication, or non-monetary, e.g., search costs. Platform designs center around lowering entry costs for producers, oftentimes leading to increased production and competition, and lowering search costs for consumers. In this section, we present a simple search cost model which highlights the ability of the discriminatory access design to also consider search costs, and the distinction between open access and discriminatory access designs. 

% As we are working in the networked Cournot setting where demand is aggregated, we must use a simple model for search costs. We define a search cost for each consumer market $j$, $r_j$, on the consumers as a product of their consumer surplus (taking care of the simple assuring assumption that markets are rational and that search costs can never be more than their surplus) and a discount factor $f(n)$ which monotonically increases with the number of firms $n$, and lastly, a market-specific parameter $\theta$ highlighting potentially different market segments with differing search costs, defined as follows: 
% $$
% r_j = \theta f(n) CS_j, ~ 0\le \theta \le 1,
% $$
% where function $f$ has the following properties:
% $$
% f(1) = 0, \lim_{n\rightarrow \infty} f(n) = 1, f ~\text{monotonically increasing}
% $$


% %To further understand and motivate shifts towards controlled allocation and discriminatory access platforms, a model including search costs is introduced in this section. As mentioned, these costs, often not monetary, have various effects on different groups of people. Additionally, it also further motivate controlled allocation (and respectively discriminatory access) platforms in that search costs for buyers are minimal (respectively controlled) as compared to open access platforms which connects every possible firm. 

% % The search cost model for consumers in the networked Cournot setting for each market $j$ is defined below: 
% % $$
% % p_j = \theta f(n) CS_j, ~ 0\le \theta \le 1,
% % $$
% % where $\theta$ is a search cost parameter for the population, $CS_j$ refers to the consumer surplus at that market, and the function $f$ can be inferred from data, with the following properties: 
% % $$
% % f(1) = 0, \lim_{n\rightarrow \infty} f(n) = 1, f ~\text{monotonically increasing}
% % $$
% This search cost model ensures that (i) search cost penalties can never exceed consumer surplus---an assumption that search cost can never cause the market to receive negative utility, (ii) differentiation can be made through $\theta$ for low and high search cost participants, and that (iii) search cost increases in the number of firms exposed to - the effort or cost has to increase as the number of choices increase. 

% \begin{remark}
% Since controlled allocation platforms essentially make all decisions on allocation, the search cost is $0$ for consumers but continue to maintain its previous negative result from Section 4, implying that search costs has no effect on controlled allocation platforms.  
% \end{remark}

% In light of the difficulty to analyze without a further parametric form of $f(n)$, we assume hereafter that $f(n)$ assumes the form of $f(n) = \frac{n-1}{n+1}$, fulfilling the preceding properties we listed.

% Open access designs, by definition, presents all possible choices to consumers, allowing them to make production and allocation decisions, but also thereby incurring large search costs. In the following theorem, we highlight the impact of search costs on open access platforms. 

% \begin{theorem}\label{thm:openaccess-search}
% 	Open Access Platforms with search costs defined with $f(n)=\frac{n-1}{n+1}$ have worst case efficiency loss $\Omega(n)$. 
% \end{theorem}
% % \proof{Proof:} The proof is included in the Appendix. 
% % \endproof

% On the other hand, referring to Corollary \ref{cor:nine}, where the price of anarchy is $\frac{4}{3}$ at $n=1$ (which coincidentally incurs zero search cost) for discriminatory access platform designs, they maintain its worst case constant bound price of anarchy under linear cost functions and search costs. %In fact, this is true for any function $f$ that satisfies the above properties and is not restricted to the parametric form $f(n)=\frac{n-1}{n+1}$.

% %\begin{proposition}
% %	In a similar fashion, we can find that the price of anarchy in the asymmetric cost case can be written as follow: 
% %	$$
% %	\rho(K_{F,M},\overline{C}) \le \frac{1}{\frac{2n+4}{3n+5} + \delta(\gamma,n) -\theta f(n) \eta(\gamma,n)}
% %	$$
% %\end{proposition}

% %
% %
% % We consider a special example showing that misclassifying two market segments with different search costs as one can lead to inefficiency. In the simple example, we consider two market segments, one with high search costs $(\theta=1)$ and one with low ones $(\theta = 0)$. The key point is that to show that open access would result in a penalized price of anarchy, we show that finding an optimal set of firms for both segments would result still in inefficiency as compared to viewing the two market segments separately, similar to a discriminatory access platform would. 
% %
% %\begin{example}
% %	Under the setting where $f(n)$ is defined as $\frac{n-1}{n+1}$, the Price of Anarchy(PoA) can be written in the following simplified form (Note that when $n=1$, $PoA = \frac{3}{4}=0.75$.): 
% %	$$
% %	PoA(\theta) = \frac{2n+4}{3n+5} + \frac{(n-1)(3n+5)(\gamma - \frac{2n+3}{3n+5})^2}{(n+1)^2} - \theta \left(\frac{n-1}{n+1}\right)\left(\frac{\gamma(n-1) +1}{n+1}\right)^2 
% %	$$
% %	
% %	We first show that collectively considering the two different market segments with the same elasticity (We are comparing between two market segments that are typically mistaken to be one. Under the most general assumptions, they should behave almost identically and so we assume same elasticity. ) results in looking at one market with averaged search cost, essentially comparing $P_S = \frac{1}{2}(PoA(\theta_H)+PoA(\theta_L))$ against $P_J = PoA((\theta_H+\theta_L)/2)$, relying on the fact that optimal social welfare irregardless of $\theta$ since only one firm is needed there. 
% %	%Summarizing the simulation results, we have the following points to make: 
% %	%\begin{enumerate}
% %	%\item For $\theta_H$, the optimal number of firms remain as $1$ regardless of the value of $\gamma$. 
% %	%\item For $\theta_M$, the optimal number of firms remain as $1$ for $\gamma \leq 0.907 $ and $2$ otherwise.
% %	%\item For $\theta_L$, the optimal number of firms grow ``exponentially" in the value of $\gamma$. 
% %	%\item Consequently, $P_S$ grows immediately while $P_J$ only grows after $\gamma = 0.907$.
% %	%\end{enumerate}
% %	The metric of performance we are interested in can be written and defined as the following: 
% %	$$
% %	\tau = \min_\gamma \frac{1-P_S}{1-P_J}
% %	$$
% %	and can be understood as the ratio between the worst case losses in performances in the two cases. In both cases, the Price of Anarchy (PoA) is at least $0.75$ and therefore a direct comparison between the two PoA will lead to a multiplicative factor difference of at most $\frac{4}{3}$.
% %	
% %	\begin{proposition}
% %		For our similar two market segment example, the worst case $\tau$ factor is $\frac{27}{40}$. 
% %	\end{proposition}
% %	
% %	\proof{Proof: } To prove the above proposition, we will enumerate a list of lemmata, each of which will be proven in the appendix. 
% %	
% %	%Some obvious questions to ask are the following: 
% %	%\begin{enumerate}
% %	%\item Why is the transition at $0.907$? 
% %	%\item Why is $P_S$ increasing?
% %	%\item Why does $P_J$ stagnate at first and then increases after $0.907$? 
% %	%\item What is the worst case ratio $\tau$? 
% %	%\item Finally, a more difficult question is, what if market segments have different price elasticity? 
% %	%\end{enumerate}
% %	
% %	%\newpage
% %	\begin{lemma}\label{lem:agnostic-search}
% %		For the platform agnostic to the market segments with different search costs, the optimal strategy is to only show one firm for $\gamma < \frac{43}{65}+\frac{\sqrt[3]{\frac{114}{130}}}{130}\approx 0.9079$, and to show two firms otherwise. 
% %	\end{lemma}
% %
% %	This lemma highlights the two choices that the agnostic platform should make. It ends up always choosing only one or two firms depending on the symmetry of costs of the producing firms. This is clearly undesirable for the market segment with low search costs. 
% %	
% %	\begin{lemma}\label{lem:agnostic-search2}
% %		For the platform selecting firms for the market segments with high search costs, the optimal strategy is to always only show one firm. On the other hand, for the market segment with low search costs, the optimal number of firms increases as a function of $\gamma$, and in fact, transitions from $n$ to $n+1$ at $\gamma = 1-\frac{2n+3}{2n^2+10n+10} $. 
% %	\end{lemma}
% %	
% %	The optimal number of markets then for the three different search cost settings are $1$, either $1$ or $2$ and growing in $\gamma$ for the high, medium and low search cost platforms respectively. This characterization demonstrates the differing strategies and sheds light on the difference in performances we can expect. We next show the following lemma: 
% %	
% %	\begin{lemma}\label{lem:worstcase}
% %		The worse case $\gamma$ is exactly $\gamma = 1$, which yields an infinitely large optimal number of firms for the low search cost segment. The price of anarchy in the separate and joint optimization are $7/8$ and $22/27$ respectively. 
% %	\end{lemma}
% %	
% %	The result is easily obtained by computing our ratio of performance. This concludes our proof and example. \Halmos \endproof
% %	
% %\end{example}
% %$-------------------$Old Version Below$-------------------$

% Prior to this section, it seems that the performance guarantees attained by open access and discriminatory access platform designs are similar. This section presents a preliminary look at the impact of search cost on platform design, in particular highlighting the potentially post-search unbounded worst case efficiency loss result for open access platforms, and the flexibility of the discriminatory access platform design to consider search costs. It remains important to study this further, e.g., to find out how to optimize network design with search costs, or how computation or other costs involved may affect the performance of discriminatory access designs too.

%our aim was to highlight the trend towards discriminatory access despite its marginal improvement from a price of anarchy point of view in the previous sections in the absence of search costs. A simple search cost model shows that discriminatory access platforms have much more potential as compared to an open access one, and maintains its advantage over the controlled allocation platform. 

% Samples of sectioning (and labeling) in MOOR.
% NOTE: (1) all section levels end with a period,
%       (2) capitalization is as shown (sentence style, not title style).
%
%\section{Introduction.}\label{intro} %%1.
%\subsection{Duality and the classical EOQ problem.}\label{class-EOQ} %% 1.1.
%\subsection{Outline.}\label{outline1} %% 1.2.
%\subsubsection{Cyclic schedules for the general deterministic SMDP.}
%  \label{cyclic-schedules} %% 1.2.1
%\section{Problem description.}\label{problemdescription} %% 2.

% Text of your paper here

% Appendix here
% Options are (1) APPENDIX (with or without general title) or 
%             (2) APPENDICES (if it has more than one unrelated sections)
% Outcomment the appropriate case if necessary
%
% \begin{APPENDIX}{<Title of the Appendix>}
% \end{APPENDIX}
%
%   or 
%

